Normed \Omega-Group

Since sum which is not necessarily commutative is defined in \Omega-algebra A, then \Omega-algebra A is called \Omega-group. I also considered representation of \Omega-group. Norm defined in \Omega-group allows us to consider continuity of operations and continuity of representation.

==> Biblio.Russian.tex <==
%auto-ignore
\OpenBiblio

\BiblioItem{Einstein: Electrodynamics of Moving Bodies}
{
Альберт Эйнштейн,
К электродинамике движущихся тел, 1905,
Собрание научных трудов, I, 7 - 35,
М., Наука, 1965
\\
Zur Elektrodynamik der bewegter K\"orper. Ann. Phys., 1905, 17, 891-921. 
}%

\BiblioItem{Einstein: On the Relativity Principle}
{
Альберт Эйнштейн,
О принципе относительности и его следствиях, 1907,
Собрание научных трудов, I, 65 - 114,
М., Наука, 1965
\\
\"Uber das Relativit\"atsprinzip und die aus demselben gezogenen Folgerungen. 
Jahrb. d. Radioaktivit\"at u. Elektronik, 1907, 4, 411-462. 
}%

\BiblioItem{Einstein: Foundations of general relativity}
{
Альберт Эйнштейн,
Основы общей теории относительности, 1916,
Собрание научных трудов, I, 452 - 504,
М., Наука, 1965
}%

\BiblioItem{Einstein: Geometry and Experience}
{
Альберт Эйнштейн,
Геометрия и опыт, (1921)
Собрание научных трудов, II, 83 - 84,
М., Наука, 1966
}%

\BiblioItem{Einstein: Main problems of general relativity}
{
Альберт Эйнштейн,
Основные идеи и проблемы теории относительности, (1923)
Собрание научных трудов, II, 120 - 129,
М., Наука, 1966
}%

\BiblioItem{Einstein: Noneuclidean Geometry and Physics}
{
Альберт Эйнштейн,
Неэвклидова геометрия и физика, (1926)
Собрание научных трудов, II, 178 - 182,
М., Наука, 1966
}%

\BiblioItem{Einstein: Isaak Newton}
{
Альберт Эйнштейн,
Исаак Ньютон, 1927,
Собрание научных трудов, IV, 78 - 81,
М., Наука, 1967
}%

\BiblioItem{Einstein: On Science}
{
Альберт Эйнштейн,
О науке, 1931,
Собрание научных трудов, IV, 142 - 146,
М., Наука, 1967
}%

\BiblioItem{Einstein: Autobiographical Notes}
{
Альберт Эйнштейн,
Автобиографические заметки, 1949,
Собрание научных трудов, IV, 259 - 293,
М., Наука, 1967
}%

\BiblioItem{Feynman 3}
{
Фейнман Р., Лейтон Р., Сэндс М..
Фейнмановские лекции по физике (том 3). Излучение. Волны. Кванты.
М., Мир, 1976
}%

\BiblioItem{0538731877}
{
James Shipman, Jerry D. Wilson and Aaron Todd.
Introduction to Physical Science.
Cengage Learning, 2009; ISBN 0538731877.
}%

\BiblioItem{Cite: 104}
{
Ссылка 104, Источник неизвестен
}%

\BiblioItem{Ghez}
{
Ghez et al.,
The First Measurement of Spectral Lines in a Short-Period Star Bound to the Galaxy's Central Black Hole: A Paradox of Youth,
\href{http://www.journals.uchicago.edu/ApJ/journal/issues/ApJL/v586n2/16990/brief/16990.abstract.html}{ApJL, 586, L127} (2003),
eprint \href{http://arxiv.org/abs/astro-ph/0302299}{arXiv:astro-ph/0302299} (2003)
}%

\BiblioItem{Schodel}
{
R. Sch\"odel et al.,
A star in a 15.2-year orbit around the supermassive black hole at the centre of the Milky Way,
\href{http://www.nature.com/cgi-taf/DynaPage.taf?file=/nature/journal/v419/n6908/abs/nature01121_fs.html}{Nature 419, 694} (2002)
}%

\BiblioItem{Mielke}
{
Eckehard W. Mielke, Affine generalization of the Komar complex of general relativity,
\href{http://prola.aps.org/searchabstract/PRD/v63/i4/e044018}{Phys. Rev. D 63, 044018} (2001)
}%

\BiblioItem{Obukhov}
{
Yu. N. Obukhov and J. G. Pereira, Metric\hyph affine approach to teleparallel gravity,
\href{http://scitation.aip.org/getabs/servlet/GetabsServlet?prog=normal&id=PRVDAQ000067000004044016000001&idtype=cvips&gifs=Yes}
{Phys. Rev. D 67, 044016} (2003),
eprint \href{http://arxiv.org/abs/gr-qc/0212080}{arXiv:gr-qc/0212080} (2002)
}%

\BiblioItem{Sardanashvily}
{
Giovanni Giachetta, Gennadi Sardanashvily, Dirac Equation in Gauge and Affine-Metric Gravitation Theories,
eprint \href{http://arxiv.org/abs/gr-qc/9511035}{arXiv:gr-qc/9511035} (1995)
}%

\BiblioItem{Gauge}
{
Frank Gronwald and Friedrich W. Hehl, On the Gauge Aspects of Gravity, eprint
\href{http://arxiv.org/abs/gr-qc/9602013}{arXiv:gr-qc/9602013} (1996)
}%

\begin{otherlanguage}{english}
\BiblioItem{Neeman}
{
Yuval Neeman, Friedrich W. Hehl, Test Matter in a Spacetime with Nonmetricity, eprint
\href{http://arxiv.org/abs/gr-qc/9604047}{arXiv:gr-qc/9604047} (1996)
}%
\end{otherlanguage}

\BiblioItem{torsion}
{
F. W. Hehl, P. von der Heyde, G. D. Kerlick, and J. M. Nester,
General relativity with spin and torsion: Foundations and prospects,\\
\href{http://prola.aps.org/abstract/RMP/v48/i3/p393_1}{Rev. Mod. Phys. 48, 393} (1976)
}%

\BiblioItem{Megged}
{
O. Megged, Post-Riemannian Merger of Yang-Mills Interactions with Gravity,
eprint \href{http://arxiv.org/abs/hep-th/0008135}{arXiv:hep-th/0008135} (2001)
}%

%\BiblioItem{Hehl}
%{
%Friedrich W. Hehl, Uwe Muench,
%eprint \href{http://arxiv.org/abs/gr-qc/9708007}{arXiv:gr-qc/9708007} (1997)
%}%

\BiblioItem{gr-qc-9604027}
{
Yu.N. Obukhov, E.J. Vlachynsky, W. Esser, R. Tresguerres and F.W. Hehl,
An exact solution of the metric\hyph affine gauge theory with dilation, shear, and spin charges,
eprint \href{http://arxiv.org/abs/gr-qc/9604027}{arXiv:gr-qc/9604027} (1996)
}%

\BiblioItem{4419-7514}
{
Mari\'an Fabian, Petr Habala, Petr H\'ajek, Vicente Montesinos, V\'aclav Zizler.
Banach Space Theory: The Basis for Linear and Nonlinear Analysis.
\\
Springer; New York, 2010; ISBN-13: 978-1441975140
}%

\BiblioItem{Weinberg I}
{
Стивен Вайнберг.
Квантовая теория полей. Том 1. Основы.
\\
Перевод на русский язык А. В. Беркова под редакцией Б. Л. Воронова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Weinberg II}
{
Стивен Вайнберг.
Квантовая теория полей. Том 2. Современные приложения.
\\
Перевод на русский язык А. В. Беркова,
М., Физико-математическая литература, 2001
}%

\BiblioItem{Reinhardt}
{
Walter Greiner, Joachim Reinhardt. Field Quantization. Springer.
}%

\BiblioItem{978-3540875604}
{
Walter Greiner, Joachim Reinhardt. Quantum Electrodynamics. Springer, 2009.
}%

\BiblioItem{978-1898563020}
{
H. Robert Mills. Practical Astronomy. Woodhead Publishing, 1994. ISBN-13: 978-1898563020.v
}%

\BiblioItem{Landau}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, теория поля,
М., Наука, 1988
}%

\BiblioItem{Landau III}
{
Л. Д. Ландау, Е. М. Лифшич,
Теоретическая физика, том III, квантовая механика,
нерелятивистская теория,
М., Наука, 1989
}%

\BiblioItem{Wheeler}
{
Ignazio Ciufolini, John Wheeler. Gravitation and Inertia.
Princeton university press.
}%

\BiblioItem{Gravitation MTW 1}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $1$.
\\
Перевод с английского М. М. Баско
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Gravitation MTW 2}
{
Ч. Мизнер, К. Торн, Дж. Уилер.
Гравитация, том $2$.
\\
Перевод с английского A. А. Рузмайкина 
под редакцией В. Б. Брагинского и И. Д. Новикова.
\\
М. Мир, 1977.
}%

\BiblioItem{Anderson98}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Indication, from Pioneer 10/11, Galileo, and Ulysses Data, of an Apparent Anomalous, Weak, Long-Range Acceleration,
\href{http://prola.aps.org/abstract/PRL/v81/i14/p2858_1}{Phys. Rev. Lett. 81, 2858}, (1998),
eprint \href{http://arxiv.org/abs/gr-qc/9808081}{arXiv:gr-qc/9808081} (1998)
}%

\BiblioItem{Anderson02}
{
J. D. Anderson, P. A. Laing, E. L. Lau, A. S. Liu, M. M. Nieto, and S. G. Turyshev,
Study of the anomalous acceleration of Pioneer 10 and 11,
\href{http://prola.aps.org/searchabstract/PRD/v65/i8/e082004}{Phys. Rev. D 65, 082004, 50 pp.}, (2002),
eprint \href{http://arxiv.org/abs/gr-qc/0104064}{arXiv:gr-qc/0104064} (2001)
}%

%\BiblioItem{Havas} Peter Havas, The Classical Equations of Motion of Point Particles, I,
%{
%\href{http://prola.aps.org/abstract/PR/v87/i2/p309_1}{Phys. Rev. 87, 309} (1952)
%}%

\BiblioItem{H. Aslaksen}
{
H. Aslaksen.  Quaternionic determinants \textit{Math.
Intelligencer} {\bf 18}(3), pp.57-65, (1996).
}%

\BiblioItem{L. Chen: Definition of determinant}
{
L. Chen, Definition of determinant and Cramer solutions over
quaternion field, \textit{Acta Math. Sinica (N.S.)} {\bf 7},
pp.171-180, (1991).
}%

\BiblioItem{L. Chen: Inverse matrix}
{
L. Chen,
Inverse matrix and properties of double determinant over quaternion
field, \textit{Sci. China, Ser. A} {\bf 34}, pp.528-540, (1991).
}%

\BiblioItem{N. Cohen S. De Leo}
{
N. Cohen, S. De Leo, The quaternionic determinant, \textit{The Electronic Journal Linear
Algebra} {\bf 7}, pp.100-111, (2000).
}%

\BiblioItem{Dyson: Quaternion determinants}
{
F. J. Dyson, Quaternion determinants, \textit{Helvetica Phys.
Acta} {\bf 45}, pp. 289-302, (1972).
}%

\BiblioItem{Melvin Hausner}
{
Melvin Hausner,
A Vector Space Approach to Geometry,
Dover Publications, 1998
}%

\BiblioItem{Serge Lang}
{
Серж Ленг,
Алгебра, М. Мир, 1968
}%

\BiblioItem{9780534423230}
{
Charles Lanski.
Concepts In Abstract Algebra.
American Mathematical Soc., 2005, ISBN 978-0534423230
}%

\BiblioItem{Burris Sankappanavar}
{
S. Burris, H.P. Sankappanavar,
A Course in Universal Algebra, Springer-Verlag (March, 1982),
\\eprint
\href{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
{http://www.math.uwaterloo.ca/~snburris/htdocs/ualg.html}
\\(The Millennium Edition)
}%

\BiblioItem{Shilov single 12}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, части 1 - 2,
М., Наука, 1969
}%

\BiblioItem{Shilov single 3}
{
Г. Е. Шилов. Математический анализ,
Функции одного переменного, часть 3,
М., Наука, 1970
}%

\BiblioItem{Shilov}
{
Г. Е. Шилов. Математический анализ,
Функции нескольких вещественных переменных, части 1 - 2,
М., Наука, 1972
}%

\BiblioItem{Kolmogorov Fomin}
{
А. Н. Колмогоров, С. В. Фомин.
Элементы теории функций и функционального анализа.
М., Наука, 1976
}%

\BiblioItem{Lebedev Vorovich}
{
И. И. Ворович, Л. П. Лебедев,
Функциональный анализ и его приложения в механике сплошной среды,
М., Вузовская книга, 2000
}%

\BiblioItem
{Rashevsky}
{
П. К. Рашевский,
Риманова геометрия и тензорный анализ,\\
М., Наука, 1967
}%

\BiblioItem
{Kurosh: High Algebra}
{
А. Г. Курош,
Курс высшей алгебры,
М., Наука, 1968
}%

\BiblioItem
{Kurosh: General Algebra}
{
А. Г. Курош,
Общая алгебра, (лекции 1969 - 70 учебного года),
М., МГУ, 1970
}%

\BiblioItem
{Sabinin: Smooth Quasigroups}
{
Lev V. Sabinin, Smooth Quasigroups and Loops,
Kluwer Academic Publisher, 1999 
}%

\BiblioItem{Dubrovin Fomenko Novikov part 1}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том I, Геометрия поверхностей, групп преобразований и полей,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Dubrovin Fomenko Novikov part 2}
{
Б. А. Дубровин, С. П. Новиков, А. Т. Фоменко,
Современная геометрия, Методы и приложения,\\
Том II, Геометрия и топология многообразий,\\
Эдиториал УРСС, М. 1998
}%

\BiblioItem{Kobayashi Nomizu vol 1}
{
Ш. Кобаяси, К. Номидзу,
Основы дифференциальной геометрии, Том I,
перевод с английского Л. В. Сабинина,
М., Наука, 1981
}%

\BiblioItem{Lichnerowicz}
{
Андрэ Лихнерович,
Теория связностей в целом и группы голономий,
перевод с французкого С. П. Финикова под редакцией В. В. Рыжкова,
М., Иностранная литература, 1960
}%

\BiblioItem{Korn}
{
Г. Корн, Т. Корн,
Справочник по математике для научных работников и инженеров,
М., Наука, 1974
}%

\BiblioItem{Hocking Young Topology}
{
John G. Hocking, Gail S. Young,
Topology,\\
Courier Dover Publications, 1988
}%

\BiblioItem{Olver: Lie groups to differential equations}
{
П. Олвер,
Приложения групп Ли к дифференциальным уравнениям,\\
М. Мир, 1989
}%

\BiblioItem{Tartaglia}
{
Angelo Tartaglia and Matteo Luca Ruggiero,
Angular Momentum Effects in Michelson\Hyph Morley Type Experiments,
Gen.Rel.Grav. 34, 1371-1382 (2002),\\
eprint \href{http://arxiv.org/abs/gr-qc/0110015}{arXiv:gr-qc/0110015} (2001)
}%

\BiblioItem{Tomozawa}
{
Yukio Tomozawa, Speed of Light in Gravitational Fields, eprint
\href{http://arxiv.org/abs/astro-ph/0303047}{arXiv:astro-ph/0303047} (2004)
}%

\BiblioItem{Magueijo}
{
Joao Magueijo,
Covariant and locally Lorentz-invariant varying speed of light theories,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103521}{Phys. Rev. D 62, 103521} (2000),
eprint \href{http://arxiv.org/abs/gr-qc/0007036}{arXiv:gr-qc/0007036} (2000)
}%

\BiblioItem{Bassett}
{
Bruce A. Bassett, Stefano Liberati, Carmen Molina-Paris, and Matt Visser,
Geometrodynamics of variable-speed-of-light cosmologies,
\href{http://prola.aps.org/abstract/PRD/v62/i10/e103518}{Phys. Rev. D 62}, 103518 (2000),
eprint \href{http://arxiv.org/abs/astro-ph/0001441}{arXiv:astro-ph/0001441} (2000)
}%

\BiblioItem{C.A. Deavours The Quaternion Calculus}
{
C.A. Deavours, The Quaternion Calculus, 
American Mathematical Monthly, {\bf 80} (1973), pp. 995 - 1008
}%

\BiblioItem{Straumann}
{
Lochlainn O'Raifeartaigh and Norbert Straumann,
Gauge theory: Historical origins and some modern developments,
\href{http://prola.aps.org/abstract/RMP/v72/i1/p1_1}{Rev. Mod. Phys. 72, 1} (2000)
}%

\begin{otherlanguage}{english}
\BiblioItem{Lammerzahl}
{
Claus L\"ammerzahl, Mark P. Haugan,
On the interpretation of Michelson\Hyph Morley experiments,
%\href{http://www.sciencedirect.comyph /science?_ob=ArticleURL&_udi=B6TVM-42WP7CR-1&_user=10&_handle=W-WA-A-A-AZ-MsSAYZW-UUW-AUDDYZYZAU-WZCBYCEDW-AZ-U&_fmt=summary&_coverDate=04%2F23%2F2001&_rdoc=1&_orig=browse&_srch=%23toc%235538%232001%23997179995%23246657!&_cdi=5538&view=c&_acct=C000050221&_version=1&_urlVersion=0&_userid=10&md5=385478cda8c5568dea1aeaf0c43669da}
{Phys. Lett. A282 223-229} (2001),\\
eprint \href{http://arxiv.org/abs/gr-qc/0103052}{arXiv:gr-qc/0103052} (2001)
}%
\end{otherlanguage}

\begin{otherlanguage}{english}
\BiblioItem{0305117}
{
Holger Mueller, Sven Herrmann, Claus Braxmaier, Stephan Schiller, Achim Peters.
Modern Michelson-Morley Experiment using Cryogenic Optical Resonators.
eprint \href{http://arxiv.org/abs/physics/0305117}{arXiv:physics/0305117} (2003)
\\
Phys. Rev. Lett. 91:020401, 2003
}%
\end{otherlanguage}

\BiblioItem{0706.2031}
{
Holger Mueller, Paul Louis Stanwix, Michael Edmund Tobar,
Eugene Ivanov, Peter Wolf, Sven Herrmann, Alexander Senger,
Evgeny Kovalchuk, Achim Peters.
Relativity tests by complementary rotating Michelson-Morley experiments.
eprint \href{http://arxiv.org/abs/0706.2031}{arXiv:0706.2031 [physics.class-ph]} (2006)
\\
Phys. Rev. Lett. 99:050401, 2007
}%

\BiblioItem{1008.1205}
{
M. Nagel, K. M\"ohle, K. D\"oringshoff, S. Herrmann, A. Senger, E.V. Kovalchuk, A. Peters.
Testing Lorentz Invariance by Comparing Light Propagation in Vacuum and Matter.
eprint \href{http://arxiv.org/abs/1008.1205}{arXiv:1008.1205 [physics.ins-det]} (2010)
}%

\BiblioItem{1109.4897}
{
The OPERA Collaboration.
Measurement of the neutrino velocity with the OPERA detector in the CNGS beam.
eprint \href{http://arxiv.org/abs/1109.4897}{arXiv:1109.4897 [hep-ex]} (2011)
}%

\begin{otherlanguage}{english}
\BiblioItem{Ranada}
{
Antonio F. Ranada,
Pioneer acceleration and variation of light speed: experimental situation,
eprint \href{http://arxiv.org/abs/gr-qc/0402120}{arXiv:gr-qc/0402120} (2004)
}%
\end{otherlanguage}

\BiblioItem{Gelfand Minlos: rotation and Lorentz groups}
{
И. М. Гельфанд, Р. А. Минлос, З. Я. Шапиро,
Представления группы вращений и группы Лоренца, их применения,\\
М., Наука, 1958
}%

\BiblioItem{math.QA-0208146}
{
I. Gelfand, S. Gelfand, V. Retakh, R. Wilson,
Quasideterminants,\\
eprint \href{http://arxiv.org/abs/math.QA/0208146}{arXiv:math.QA/0208146} (2002)
}%

\BiblioItem{q-alg-9705026}
{
I. Gelfand, V. Retakh,
Quasideterminants, I,\\
eprint \href{http://arxiv.org/abs/q-alg/9705026}{arXiv:q-alg/9705026} (1997)
}%

\BiblioItem{Gelfand Retakh 1991}
{
И. М. Гельфанд, В. С. Ретах,  Детерминанты матриц над некоммутативными кольцами,
\textit{Функциональный анализ и его приложения} {\bf 25}(2), c. 13-35, (1991).
}%

\BiblioItem{Gelfand Retakh 1992}
{
И. М. Гельфанд, В. С. Ретах,  Теория некоммутативных
детерминантов и характеристические функции графов,\\
\textit{Функциональный анализ и его приложения} {\bf 26} (4), c.
33-45, (1992).
}%

\BiblioItem{hep-th-9407124}
{
I. M. Gelfand, D. Krob, A. Lascoux, B. Leclerc, V.S. Retakh and J.-Y. Thibon,
Noncommutative symmetric functions,\\
eprint \href{http://arxiv.org/abs/hep-th/9407124}{arXiv:hep-th/9407124} (1994)
}%

\BiblioItem{Naimark Shtern: Theory of group representations}
{
М. А. Наймарк,
Теория представления групп,\\
М., Наука, 1976
}%

\BiblioItem{Barut Raczka: Theory of group representations}
{
А. Барут, Р. Рончка,
Теория представления групп и её приложения,\\
Перевод с английского А. У. Климыка и А. М. Гаврилика
под редакцией Я. А. Смородинского,\\
М., Мир, 1980
}%

\BiblioItem{Mihalev Pilz: concise handbook of algebra}
{
Aleksandr Vasilevich Mikhalev; G\"{u}nter Pilz;
The concise handbook of algebra;\\
Kluwer Academic Publishers, 2002
}%

\BiblioItem{Shafarevich: Basic notions of algebra}
{
И. Р. Шафаревич,
Основные понятия алгебры,\\
В сборнике "Современные проблемы математики. Фундаментальные направления
(Итоги науки и техники. ВИНИТИ АН СССР",
М., 1986, {\bf 11} 3 - 289
М., Мир, 1980
}%

\BiblioItem{Coppel: Number Theory}
{
W.A. Coppel,
Number Theory: An Introduction to Mathematics,\\
Springer, 2009
}%

\BiblioItem{978-0486497952}
{
Michael J. Field,
Differential Calculus and Its Applications,\\
Dover Publications, 2012; ISBN-13: 978-0486497952
}%

\BiblioItem{Elsgolts: Differential Equations}
{
Л. Э. Эльсгольц,
Дифференциальные уравнения и вариационное исчисление,
М., Наука, 1971 
}%

\BiblioItem{Baez Huerta: algebra of grand unified theories}
{
John Baez; John Huerta;
The algebra of grand unified theories;\\
Bull. Amer. Math. Soc. {\bf 47} (2010), 483-552
}%

\BiblioItem{J. Fan: Determinants}
{
J. Fan, Determinants and multiplicative functionals
on quaternion matrices, \textit{Linear Algebra and Its
Applications} {\bf 369}, pp. 193-201, (2003).
}%

\BiblioItem{Carl Faith 1}
{
К. Фейс, Алгебра: кольца, модули и категории, том I,
М., Мир, 1973
}%

\BiblioItem{Gilson Nimmo Ohta}
{
 C.R.Gilson, J.J.C.Nimmo, Y.Ohta, Quasideterminant solutions of a non-Abelian Hirota-Miwa
 equation, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 40}(42), pp.
 12607-12617,(2007).
}%

\BiblioItem{Haider Hassan}
{
B. Haider, M. Hassan, Quasideterminant solutions of an integrable chiral model in two
 dimensions, \textit{Journal of Physics A: Mathematical and Theoretical} {\bf 42} (35), art. no.
 355211, (2009).
}%

%\BiblioItem{Pareigis}
%{
%Bodo Pareigis, Categories and Functors,
%Academic Press - New York - London, 1970
%}%

%\BiblioItem{Beachy}
%{
%John A. Beachy, Introductory Lectures on Rings i Modules,
%Cambridge University Press, 1999
%}%

\BiblioItem{0702447}
{
I.I. Kyrchei, Cramer's rule for quaternion systems of linear equations,
\textit{Journal of Mathematical Sciences} {\bf 155}(6), 839-858, (2008).
 Translated from  \textit{Fundamental and Appl. Math.}
 {\bf 13}(4), pp.67-94, (2007). (in Russian)\\
eprint
\href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447}
(2007)
}%

\BiblioItem{1004.4380}
{
I.I. Kyrchei, Cramer's rule for some quaternion matrix
    equations,  \textit{Applied Mathematics and Computation} {\bf 217}(5), pp.2024-2030, (2010).\\eprint
\href{http://arxiv.org/abs/1004.4380
}{arXiv:math.RA/arXiv:1004.4380 } (2010)
}%

\BiblioItem{1005.0736}
{
I.I. Kyrchei,Determinantal representations of the Moore-Penrose inverse
 over the quaternion skew field and corresponding Cramer's rules,
 \\
eprint
\href{http://arxiv.org/abs/1005.0736}{arXiv:math.RA/1005.0736}
(2010)
}%

\BiblioItem{0412.391}
{
Александр Клейн,
Многообразие базисов,\\
eprint \href{http://arxiv.org/abs/math.DG/0412391}{arXiv:math.DG/0412391} (2007)
}%

\BiblioItem{0405.027}
{
Александр Клейн,
Система отсчета в общей теории относительности,
eprint \href{http://arxiv.org/abs/gr-qc/0405027}{arXiv:gr-qc/0405027} (2008)
}%

\BiblioItem{0405.028}
{
Александр Клейн,
Метрико\hyph аффинное многообразие,\\
eprint \href{http://arxiv.org/abs/gr-qc/0405028}{arXiv:gr-qc/0405028} (2008)
}%

\BiblioItem{0612.111}
{
Александр Клейн,
Бикольцо матриц,\\
eprint \href{http://arxiv.org/abs/math.OA/0612111}{arXiv:math.OA/0612111} (2007)
}%

\BiblioItem{0701.238}
{
Александр Клейн,
Лекции по линейной алгебре над телом,\\
eprint \href{http://arxiv.org/abs/math.GM/0701238}{arXiv:math.GM/0701238} (2010)
}%

\BiblioItem{0702.561}
{
Александр Клейн,
Расслоенная $\mathfrak{F}$\Hyph алгебра,\\
eprint \href{http://arxiv.org/abs/math.DG/0702561}{arXiv:math.DG/0702561} (2007)
}%

\BiblioItem{math.RA-0501237}
{
Александр Клейн,
Векторное пространство над телом,\\
eprint \href{http://arxiv.org/abs/math.RA/0412391}{arXiv:math.RA/0501237} (2007)
}%

\BiblioItem{math.RA-0501237v1}
{
Aleks Kleyn,
Module Over Division Ring, version 1,\\
eprint \href{http://arxiv.org/abs/math/0501237v1}{arXiv:math.RA/0501237v1} (2005)
}%

\BiblioItem{0707.2246}
{
Александр Клейн,
Расслоенное соответствие,\\
eprint \href{http://arxiv.org/abs/0707.2246}{arXiv:0707.2246} (2007)
}%

\BiblioItem{0803.2620}
{
Александр Клейн,
Морфизм \Ts представлений,\\
eprint \href{http://arxiv.org/abs/0803.2620}{arXiv:0803.2620} (2008)
}%

\BiblioItem{0803.3276}
{
Александр Клейн,
Преобразование Лоренца и принцип общековариантности,\\
eprint \href{http://arxiv.org/abs/0803.3276}{arXiv:0803.3276} (2009)
}%

\BiblioItem{0812.4763}
{
Александр Клейн,
Введение в математический анализ над телом,\\
eprint \href{http://arxiv.org/abs/0812.4763}{arXiv:0812.4763} (2010)
}%

\BiblioItem{0906.0135}
{
Александр Клейн,
Введение в геометрию над телом,\\
eprint \href{http://arxiv.org/abs/0906.0135}{arXiv:0906.0135} (2010)
}%

\BiblioItem{0909.0855}
{
Александр Клейн,
Этюд о кватернионах,\\
eprint \href{http://arxiv.org/abs/0909.0855}{arXiv:0909.0855} (2010)
}%

\BiblioItem{0912.3315}
{
Александр Клейн,
Представление универсальной алгебры,\\
eprint \href{http://arxiv.org/abs/0912.3315}{arXiv:0912.3315} (2010)
}%

\BiblioItem{0912.4061}
{
Александр Клейн,
Линейное уравнение в конечномерной алгебре,\\
eprint \href{http://arxiv.org/abs/0912.4061}{arXiv:0912.4061} (2010)
}%

\BiblioItem{1001.4852}
{
Александр Клейн,
Матрица линейных отображений,\\
eprint \href{http://arxiv.org/abs/1001.4852}{arXiv:1001.4852} (2010)
}%

\BiblioItem{1003.1544}
{
Александр Клейн,
Линейные отображения свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1003.1544}{arXiv:1003.1544} (2010)
}%

\BiblioItem{1006.2597}
{
Александр Клейн,
Производная Гато и интеграл над банаховой алгеброй,\\
eprint \href{http://arxiv.org/abs/1006.2597}{arXiv:1006.2597} (2010)
}%

\BiblioItem{1011.3102}
{
Александр Клейн,
Полилинейное отображение свободной алгебры,\\
eprint \href{http://arxiv.org/abs/1011.3102}{arXiv:1011.3102} (2010)
}%

\BiblioItem{1104.5197}
{
Александр Клейн,
$C^*$-рапсодия,\\
eprint \href{http://arxiv.org/abs/1104.5197}{arXiv:1104.5197} (2011)
}%

\BiblioItem{1105.4307}
{
Александр Клейн,
Алгебра с сопряжением,\\
eprint \href{http://arxiv.org/abs/1105.4307}{arXiv:1105.4307} (2011)
}%

\BiblioItem{1107.1139}
{
Александр Клейн,
Линейные отображения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1107.1139}{arXiv:1107.1139} (2011)
}%

\BiblioItem{1107.5037}
{
Александр Клейн,
Ортогональный базис и движение в финслеровой геометрии,\\
eprint \href{http://arxiv.org/abs/1107.5037}{arXiv:1107.5037} (2011)
}%

\BiblioItem{1202.6021}
{
Александр Клейн,
Отображения сопряжения алгебры кватернионов,\\
eprint \href{http://arxiv.org/abs/1202.6021}{arXiv:1202.6021} (2012)
}%

\BiblioItem{1211.6965}
{
Александр Клейн,
Свободная алгебра со счётным базисом,\\
eprint \href{http://arxiv.org/abs/1211.6965}{arXiv:1211.6965} (2012)
}%

\BiblioItem{1305.4547}
{
Александр Клейн,
Нормированная $\Omega$-группа,\\
eprint \href{http://arxiv.org/abs/1305.4547}{arXiv:1305.4547} (2013)
}%

\BiblioItem{8433-5163}
{
Aleks Kleyn,
Linear Maps of Free Algebra: First Steps in Noncommutative Linear Algebra,\\
Lambert Academic Publishing, 2010
}%

\BiblioItem{8443-0072}
{
Aleks Kleyn,
Representation Theory: Representation of Universal Algebra,\\
Lambert Academic Publishing, 2011
}%

\BiblioItem{4776-3181}
{
Aleks Kleyn.\\
Linear Algebra over Division Ring: System of Linear Equations.\\
Create Space, 2012; ISBN-13: 978-1477631812
}%

\BiblioItem{CACAA.01.291}
{
Aleks Kleyn,
Introduction into Calculus over Division Ring.\\
Clifford Analysis, Clifford Algebras and their applications,
Vol 1, Issue 4, pages 291 - 355, 2012
}%

\BiblioItem{GJSFRA.13.1.39}
{
Aleks Kleyn,
Reference frame and Lorentz transformation,\\
Global Journals of Science Frontier Research A,
volume 13, issue 1, pages 39 - 55, 2013 
}%

\BiblioItem{Lauve: Quantum coordinates}
{
A. Lauve, Quantum- and quasi-Plucker coordinates,
\textit{Journal of Algebra} {\bf 296}(2), pp.440-461,
(2006).
}%

\BiblioItem{Lewis D. W. Quaternion algebras}
{
Lewis D. W. Quaternion algebras and the algebraic legacy
of Hamilton's quaternions, \textit{Irish Math. Soc. Bulletin} {\bf
57}, pp. 41-64, (2006).
}%

\BiblioItem{0812.2865}
{
Jos\'e Miguel Figueroa-O'Farrill,
Three lectures on 3-algebras,
eprint \href{http://arxiv.org/abs/0812.2865}{arXiv:0812.2865} (2008)
}%

\BiblioItem{1202.0951}
{
Daniel Edward Clark,
Deconvolution of point processes,
eprint \href{http://arxiv.org/abs/1202.0951}{arXiv:1202.0951} (2012)
}%

\BiblioItem{1202.4546}
{
Ming-Liang Hu,
Disentanglement, Bell-nonlocality violation
and teleportation capacity of the decaying tripartite states,
eprint \href{http://arxiv.org/abs/1202.4546}{arXiv:1202.4546} (2012)
}%

\BiblioItem{1203.1629}
{
Borivoje Dakic, Yannick Ole Lipp, Xiaosong Ma, Martin Ringbauer,
Sebastian Kropatschek, Stefanie Barz, Tomasz Paterek, Vlatko Vedral,
Anton Zeilinger, Caslav Brukner, Philip Walther,
Quantum Discord as Optimal Resource for Quantum Communication,
eprint \href{http://arxiv.org/abs/1203.1629}{arXiv:1203.1629} (2012)
}%

\BiblioItem{Li Nimmo: Darboux transformations}
{
C.X.Li, J.J.C. Nimmo, Darboux transformations for a twisted
derivation and quasideterminant solutions to the super KdV
equation, \textit{Proceedings of the Royal Society A:
Mathematical, Physical and Engineering Sciences} {\bf 466} (2120),
pp. 2471-2493, (2010)
}%

\BiblioItem{Schiebold: Cauchy-type determinants}
{
C. Schiebold, Cauchy-type determinants and integrable
systems, \textit{Linear Algebra and Its Applications} {\bf 433}
(2), pp. 447-475, (2010)
}%

\BiblioItem{Suzuki: Noncommutative spectral decomposition}
{
T. Suzuki, Noncommutative
spectral decomposition with qua\-si\-de\-ter\-mi\-nant, \textit{Advances in
Mathematics} {\bf 217}(5), pp. 2141-2158, (2008)
}%

\BiblioItem{1105.3456}
{
C. W. F. Everitt, D. B. DeBra, B. W. Parkinson, J. P. Turneaure, J. W. Conklin,
M. I. Heifetz, G. M. Keiser, A. S. Silbergleit, T. Holmes, J. Kolodziejczak,
M. Al-Meshari, J. C. Mester, B. Muhlfelder, V. Solomonik, K. Stahl, P. Worden,
W. Bencze, S. Buchman, B. Clarke, A. Al-Jadaan, H. Al-Jibreen, J. Li, J. A. Lipa,
J. M. Lockhart, B. Al-Suwaidan, M. Taber, S. Wang,\\
Gravity Probe B: Final Results of a Space Experiment to Test General Relativity,\\
eprint \href{http://arxiv.org/abs/1105.3456}{arXiv:1105.3456[math-ph]} (2011)
}%

\BiblioItem{0009305}
{
G. S. Asanov.
Can Neutrinos and High-Energy Particles Test Finsler Metric of Space-Time?\\
eprint \href{http://arxiv.org/abs/hep-ph/0009305}{arXiv:hep-ph/0009305} (2000)
}%

\BiblioItem{Asanov 2004}
{
Г. С. Асанов.
Финслероид - пространство с углом и скалярным произведением.\\
Гиперкомплексные числа в геометрии и физике, {\bf 1}, 2004, с. 43 - 67
}%

\BiblioItem{1004.3007}
{
Sergiu I. Vacaru,
Principles of Einstein-Finsler Gravity and Perspectives in Modern Cosmology,\\
eprint \href{http://arxiv.org/abs/1004.3007}{arXiv:1004.3007[gr-qc]} (2010)
}%

\BiblioItem{1012.4148}
{
Sergiu I. Vacaru.
Principles of Einstein-Finsler Gravity and Cosmology.\\
eprint \href{http://arxiv.org/abs/1012.4148}{arXiv:1012.4148[physics.gen-ph]} (2010)
}%

\BiblioItem{1112.5641}
{
Christian Pfeifer, Mattias N.R. Wohlfarth.
Finsler geometric extension of Einstein gravity.\\
eprint \href{http://arxiv.org/abs/1112.5641}{arXiv:1112.5641[gr-qc]} (2011)
}%

\BiblioItem{0711.0056}
{
Zhe Chang, Xin Li.
Lorentz Invariance Violation and Symmetry in Randers\Hyph Finsler Spaces.\\
eprint \href{http://arxiv.org/abs/0711.0056}{arXiv:0711.0056[hep-th]} (2011)
}%

\BiblioItem{Rund Finsler geometry}
{
Х. Рунд,
Дифференциальная геометрия финслеровых пространств.
\\
Перевод с английского Г. С. Асанова под редакцией Э. Г. Позняка,
М., Наука, 1981
}%

\BiblioItem{Smirnov vol 1}
{
В. И. Смирнов,
Курс высшей математики, том первый.
\\
М., Наука, 1974
}%

\BiblioItem{Beem Dostoglou Ehrlich}
{
John K. Beem, Stamatis A. Dostoglou, Paul E. Ehrlich,
Advances in differential geometry and general relativity.
\\
American Mathematical Society, 2004
}%

\BiblioItem{978-0719033414}
{
Malcolm Pemberton, Nicholas Rau,
Mathematics for economists: an introductory textbook.
\\
Manchester University Press, November 2001; ISBN-13: 978-0719033414
}%

\BiblioItem{0 521 59180 5}
{
Cyrus D. Cantrell,
Modern mathematical methods for physicists and engineers.
\\
Cambridge University Press, 2000
}%

\BiblioItem{Arveson spectral theory}
{
William Arveson,
A short course on spectral theory.
\\
Springer - Verlag, New York, 2002
}%

\BiblioItem{Robert Hermann}
{
Robert Hermann,
Topics in the mathematics of quantum mechanics.
\\
Math Sci Press, 1973
}%

\BiblioItem{9705.009}%q-alg-9705009
{
John C. Baez,
An Introduction to n-Categories,\\
eprint \href{http://arxiv.org/abs/q-alg/9705009}{arXiv:q-alg/9705009} (1997)
}%

\BiblioItem{0105.155}
{
John C. Baez,
The Octonions,\\
eprint \href{http://arxiv.org/abs/math.RA/0105155}{arXiv:math.RA/0105155} (2002)
}%

\BiblioItem{John Baez: Math Blogs}
{
John C. Baez,
What do mathematicians need to know about blogging?,\\
Notices of the American Mathematical Society,
(2010), 3, {\bf 57}, 333,\\
\url{http://www.ams.org/notices/201003/rtx100300333p.pdf}
}%

\BiblioItem{Tolstoi about Anna Karenina}
{
Константин Паустовский. Золотая роза, в сборнике Книга скитаний.
Картя молдовеняскэ, Кишинёв, 1978
}%
%Л. Н. Толстой в воспоминаниях современиков, т. 1, М. 1955, с. 231 - 232

\BiblioItem
{Cohn: Universal Algebra}
{
П. Кон,
Универсальная алгебра,
М., Мир, 1968
}%

\BiblioItem
{Cohn: Algebra 3}
{
Paul M. Cohn,
Algebra, Volume 3,
John Wiley \& Sons, 1991
}%

\BiblioItem
{Cohn: Skew Fields}
{
Paul M. Cohn,
Skew Fields,
Cambridge University Press, 1995
}%

\BiblioItem
{Maunder: Algebraic Topology}
{
C. R. F. Maunder,
Algebraic Topology,
Dover Publications, Inc, Mineola, New York, 1996
}%

\BiblioItem{Pommaret: Partial Differential Equations}
{
Ж. Поммаре,
Системы уравнений с частными производными и псевдогруппы Ли,
М., Мир, 1983
}%

\BiblioItem{Bourbaki: Set Theory}
{
Н. Бурбаки,
Теория множеств, перевод с французского Г. Н. Поварова и Ю. А.
Шихановича под редакцией В. А. Успенского,
М. Мир, 1965
}%

\BiblioItem{Bourbaki: Algebra 1}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem{Bourbaki: Algebra 2}
{
Н. Бурбаки,
Алгебра: алгебраические структуры, линейная и полилинейная алгебра,
перевод с французского Д. А. Райкова,
М.,
государственное издательство физико\Hyph математической литературы, 1962
}%

\BiblioItem
{Bourbaki: General Topology 1}
{
Н. Бурбаки,
Общая топология, основные структуры,
перевод с французского Д. А. Райкова,
М. Наука, 1968
}

\BiblioItem{Bourbaki: General Topology: Chapter 3 - 8}
{
Н. Бурбаки,
Общая топология. Топологические группы.
Числа и связанные с ними группы и пространства.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: General Topology: Chapter 5 - 10}
{
Н. Бурбаки,
Общая топология. Использование вещественных чисел в общей топологии.
\\
перевод с французского С. Н. Крачковского под редакцией Д. А. Райкова,
\\
М. Наука, 1975
}

\BiblioItem{Bourbaki: Topological Vector Space}
{
Н. Бурбаки,
Топологические векторные пространства,
перевод с французского Д. А. Райкова,
М. Иностранная литература, 1959
}

\BiblioItem{Bourbaki: Coxeter Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, главы 4 - 6,
Перевод с французского А. И. Кострикина и А. Н. Тюрина
под редакцией А. И. Кострикина,
М. Мир, 1986
}

\BiblioItem{Bourbaki: Real Group Lie}
{
Н. Бурбаки,
Группы и алгебры Ли, Компактные вещественные группы,
Перевод с французского И. А. Кострикина под редакцией А. А. Кирилова,
М. Мир, 1986
}

\BiblioItem{Shabat: Complex Analysis}
{
Шабат Б. В.,
Введение в комплексный анализ,
М. Наука, 1969
}

\BiblioItem{Pontryagin: Topological Group}
{
Понтрягин Л. С.,
Непрерывные группы,
М. Едиториал УРСС, 2004
}

\BiblioItem
{Eisenhart: Riemannian Geometry}
{
Eisenhart,
Riemannian Geometry,
Princeton University Press, Princeton, 1949
}

\BiblioItem
{Eisenhart: Continuous Groups of Transformations}
{
Л. П. Эйзенхарт,
Непрерывные группы преобразований,
перевод с английского М. М. Постникова,
М., Иностранная литература, 1947
}

\BiblioItem
{Condon Odabasi}
{
Edward Uhler Condon, Halis Odabasi,
Atomic Structure,
CUP Archive, 1980
}

\BiblioItem{Postnikov: Differential Geometry}
{
Постников М. М.,
Лекции по геометрии, семестр IV, Дифференциальная геометрия,
М. Наука, 1983
}

\BiblioItem{Fihtengolts: Calculus volume 1}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 1,
М. Наука, 1969
}

\BiblioItem{Fihtengolts: Calculus volume 2}
{
Фихтенгольц Г. М.,
Курс дифференциального и интегрального исчисления, том 2,
М. Наука, 1969
}

\BiblioItem{Hatcher: Algebraic Topology}
{
Allen Hatcher,
Algebraic Topology,
Cambridge University Press, 2002
}

\BiblioItem{geometry of differential equations}
{
А. М. Виноградов, И. С. Красильщик, В. В. Лычагин,
Введение в геометрию нелинейных дифференциальных уравнений,
М. Наука, 1986
}

\BiblioItem{cohomological analysis}
{
A. M. Vinogradov,
Cohomological Analysis of Partial Differential Equations
and Secondary Calculus,
American Mathematical Society, 2001
}

\BiblioItem{0801.1734}
{
Brandon S. DiNunno, Richard A. Matzner,
The Volume Inside a Black Hole,\\
eprint \href{http://arxiv.org/abs/0801.1734v1}{arXiv:0801.1734v1} (2008)
}

\BiblioItem{0702.447}
{
Ivan Kyrchei,
Cramer's rule for some quaternion matrix equations,\\
eprint \href{http://arxiv.org/abs/math/0702447}{arXiv:math.RA/0702447} (2007)
}

\BiblioItem{Izrail M. Gelfand: Quaternion Groups}
{
I. M. Gelfand, M. I. Graev,
Representation of Quaternion Groups over Localy Compact and
Functional Fields,\\
Functs. Anal. Prilozh. {\bf 2} (1968) 20 - 35;\\
Izrail Moiseevich Gelfand, Semen Grigorevich Gindikin,\\
Izrail M. Gelfand: Collected Papers, volume II, 435 - 449,\\
Springer, 1989
}

\BiblioItem{Richard D. Schafer}
{
Richard D. Schafer,
An Introduction to Nonassociative Algebras,
Dover Publications, Inc., New York, 1995
}

\BiblioItem{Bamberg Sternberg}
{
Paul Bamberg, Shlomo Sternberg,
A course in mathematics for students of physics,
Cambridge University Press, 1991
}

\BiblioItem{Conway Smith}
{
John Horton Conway, Derek Alan Smith,
On quaternions and octonions: their geometry, arithmetic, and symmetry,
A K Peters, Natick, Massachussets, 2003
}

\BiblioItem{Fueter}
{
Fueter, R.
Die Funktionentheorie der Differentialgleichungen $\Delta u = 0$ und
$\Delta \Delta u = 0$ mit vier reellen Variablen.
Comment. Math. Helv. {\bf 7} (1935), 307-330
}

\BiblioItem{Sudbery Quaternionic Analysis}
{
A. Sudbery,
Quaternionic Analysis,
Math. Proc. Camb. Phil. Soc. (1979), {\bf 85}, 199 - 225
}

\BiblioItem{0902.4771}
{
Fabrizio Colombo, Graziano Gentili, Irene Sabadini,
A Cauchy kernel for slice regular functions,\\
eprint \href{http://arxiv.org/abs/0902.4771v1}{arXiv:0902.4771v1} (2009)
}

\BiblioItem{Vadim Komkov}
{
Vadim Komkov,
Variational Principles of Continuum Mechanics with Engineering Applications: Critical Points Theory,\\
Springer, 1986
}

\BiblioItem{Alain Connes 1994}
{
Alain Connes,
Noncommutative Geometry,\\
Academic Press, 1994
}

\BiblioItem{Hamilton papers 3}
{
Sir William Rowan Hamilton,
The Mathematical Papers, Vol. III, Algebra,\\
Cambridge at the University Press, 1967
}

\BiblioItem{Hamilton Elements of Quaternions 1}
{
Sir William Rowan Hamilton,
Elements of Quaternions, Volume I,\\
Longmans, Green, and Co., London, New York, and Bombay, 1899
}

\BiblioItem{Cartan geometry in reper}
{
Эли Картан,
Риманова геометрия в ортогональном репере,
По лекциям Эли Картана, читанным в Сорбонне в 1926 - 1927 гг.,\\
перевод и редакция проф. С. П. Финикова,\\
издательство МГУ, 1960
}

\BiblioItem{Cartan differential form}
{
Анри Картан.
Дифференцииальное исчисление. Дифференциальные формы.\\
М. Мир, 1971
}

\BiblioItem{Arnautov Glavatsky Mikhalev}
{
V. I. Arnautov, S. T. Glavatsky, A. V. Mikhalev,\\
Introduction to the theory of topological rings and modules,
Volume 1995,\\
Marcel Dekker, Inc, 1996
}

\BiblioItem{Moore Yaqub}
{
Hal G. Moore, Adil Yaqub,
A first course in linear algebra with applications,
Edition 3, Academic Press, 1998 
}

\BiblioItem{math.CV-0405471}
{
S. V. Ludkovsky,
Differentiable functions of Cayley-Dickson numbers,\\
eprint \href{http://arxiv.org/abs/math.CV/0405471}{arXiv:math.CV/0405471} (2004)
}%

\BiblioItem{W.Bertram H.Glockner K.Neeb}
{
W.Bertram, H.Glockner, K.Neeb,
Differential Calculus over General Base Fields and Rings,
Expositiones Mathematicae (2004), Volume 22, Issue 3, Pages 213-282
}

\CloseBiblio



==> Convention.Russian.tex <==
%auto-ignore
\input{\FilePrefix Convention.Eq}

\section{Соглашения}

\ePrints{0812.4763,0906.0135,0908.3307,0909.0855,0912.3315,1003.1544}
\Items{1006.2597}
\ifx\Semafor\ValueOn
\begin{convention}
Функция и отображение - синонимы. Однако существует
традиция соответствие между кольцами или векторными
пространствами называть отображением, а отображение
поля действительных чисел или алгебры кватернионов называть функцией.
Я тоже следую этой традиции,
хотя встречается текст, в котором неясно, какому термину надо
отдать предпочтение.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1001.4852}
\Items{1003.1544,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
В любом выражении, где появляется индекс, я предполагаю,
что этот индекс может иметь внутреннюю структуру.
Например, при рассмотрении алгебры $A$ координаты $a\in A$
относительно базиса $\Basis e$ пронумерованы индексом $i$.
Это означает, что $a$ является вектором. Однако, если $a$
является матрицей, нам необходимо два индекса, один нумерует
строки, другой - столбцы. В том случае, когда мы уточняем структуру
индекса, мы будем начинать индекс с символа $\cdot$ в соответствующей
позиции.
Например, если я рассматриваю матрицу $a^i_j$ как элемент векторного
пространства, то я могу записать элемент матрицы в виде $a^{\cdot}{}^i_j$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0908.3307,0912.4061,1006.2597,1011.3102}
\Items{Calculus.Paper,1211.6965,4910-5816,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
В выражении вида
\ShowEq{Sum over repeated index}
предполагается сумма по индексу $s$.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855}
\ifx\Semafor\ValueOn
\begin{convention}
Тело $D$ можно рассматривать как $D$\Hyph векторное пространство
размерности $1$. Соответственно этому, мы можем изучать не только
гомоморфизм тела $D_1$ в тело $D_2$, но и линейное отображение тел.
\qed
\end{convention}
\fi

\ePrints{0912.4061}
\ifx\Semafor\ValueOn
\begin{convention}
Для данного поля $F$, если не оговорено противное,
мы будем рассматривать конечномерную $F$\Hyph алгебру.
%без делителей нуля.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,4776-3181}
\ifx\Semafor\ValueOn
\begin{convention}
Несмотря на некоммутативность произведения многие утверждения
сохраняются, если заменить например правое представление на
левое представление или правое векторное пространство на левое
векторное пространство.
Чтобы сохранить эту симметрию в формулировках теорем
я пользуюсь симметричными обозначениями.
Например, я рассматриваю \Ds векторное пространство
и \sD векторное пространство.
Запись \Ds векторное пространство можно прочесть
как D\Hyph star\Hyph векторное пространство либо
как левое векторное пространство.
Запись \Ds линейно зависимые векторы можно прочесть
как D\Hyph star\Hyph линейно зависимые векторы либо
как векторы, линейно зависимые слева.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,1211.6965,4910-5816,CACAA.01.195,GJSFRF.Basis,1302.7204}
\Items{CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
\label{convention: we use separate color for index of element}
Пусть $A$ - свободная алгебра
с конечным или счётным базисом.
При разложении элемента алгебры $A$ относительно базиса $\Basis e$
мы пользуемся одной и той же корневой буквой для обозначения этого
элемента и его координат.
В выражении $a^2$ не ясно - это компонента разложения элемента
$a$ относительно базиса или это операция возведения в степень.
Для облегчения чтения текста мы будем индекс элемента алгебры выделять
цветом. Например,
\ShowEq{Expansion relative basis in algebra}
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,GJSFRF.Basis,1302.7204,CACAA.02.97}
\ifx\Semafor\ValueOn
\begin{convention}
%\label{convention: }
Очень трудно провести границу между модулем и алгеброй.
Тем более, иногда в процессе построения мы должны сперва
доказать, что множество $A$ является модулем,
а потом мы доказываем, что это множество является алгеброй.
Поэтому для записи координат элемента модуля
мы также будем пользоваться соглашением
\ref{convention: we use separate color for index of element}.
\qed
\end{convention}
\fi

\ePrints{1302.7204,CACAA.02.97,MIntegral,MSimplex,MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Элемент
\ePrints{1302.7204,CACAA.02.97,MSimplex}
\ifx\Semafor\ValueOn
$D$\Hyph алгебры
\else
$\Omega$\Hyph группы
\fi
$A$ называется
\AddIndex{$A$\Hyph числом}{A number}.
Например, комплексное число также называется
$C$\Hyph число, а кватернион называется $H$\Hyph число.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763}
\ifx\Semafor\ValueOn
\begin{convention}
Отождествление вектора и матрицы его координат
может привести к неоднозначности в равенстве
\ShowEq{Identification can lead to ambiguity, 1}
где $\Basis e$ - базис векторного пространства.
Поэтому мы будем записывать равенство
\EqRef{Identification can lead to ambiguity, 1}
в виде
\ShowEq{Identification can lead to ambiguity, 2}
чтобы видеть, где записан вектор.
\qed
\end{convention}
\fi

\ePrints{0701.238,0812.4763,0906.0135,0908.3307,0909.0855,0912.4061}
\Items{1001.4852,1003.1544,1006.2597,1104.5197,1105.4307,1107.1139}
\Items{1202.6021,MQuater,CACAA.01.195}
\ifx\Semafor\ValueOn
\begin{convention}
Если свободная конечномерная алгебра имеет единицу,
то мы будем отождествлять
вектор базиса $\Vector e_{\gi 0}$ с единицей алгебры.
\qed
\end{convention}
\fi

\ePrints{1104.5197,1105.4307}
\ifx\Semafor\ValueOn
\begin{convention}
Хотя алгебра является свободным модулем над некоторым
кольцом, мы не пользуемся векторными обозначениями
при записи элементов алгебры. В тех случаях, когда я рассматриваю
матрицу координат элемента алгебры, я буду пользоваться векторными
обозначениями для записи соответствующего элемента.
Чтобы не возникала неоднозначность при записи сопряжения,
я буду обозначать $a^*$ элемент, сопряжённый элементу $a$.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072,1111.6035,1102.5168}
\ifx\Semafor\ValueOn
\begin{convention}
В \citeBib{Cohn: Universal Algebra}
произвольная операция алгебры обозначена буквой $\omega$,
и $\Omega$ - множество операций некоторой универсальной алгебры.
Соответственно, универсальная алгебра с множеством операций
$\Omega$ обозначается $\Omega$\Hyph алгебра.
Аналогичные обозначения мы видим в
\citeBib{Burris Sankappanavar} с той небольшой разницей,
что операция в алгебре обозначена буквой $f$
и $\mathcal F$ - множество операций.
Я выбрал первый вариант обозначений, так как в этом случае
легче видно, где я использую операцию.
\qed
\end{convention}
\fi

\ePrints{0906.0135,0912.3315,8443-0072}
\ifx\Semafor\ValueOn
\begin{convention}
Так как число универсальных алгебр в башне представлений переменно,
то мы будем пользоваться векторными обозначениями для башни
представлений. Множество
$(A_1,...,A_n)$ $\Omega_i$\Hyph алгебр $A_i$, $i=1$, ..., $n$
мы будем обозначать $\Vector A$. Множество представлений
$(f_{1,2},...,f_{n-1,n})$ этих алгебр мы будем обозначать $\Vector f$.
Так как разные алгебры имеют разный тип, мы также
будем говорить о множестве $\Vector{\Omega}$\Hyph алгебр.
\ePrints{8443-0072}
\ifx\Semafor\ValueOn
Символом
\else
По отношению к множеству $\Vector A$
мы также будем пользоваться матричными обозначениями, предложенными
в разделе \xRef{0701.238}{section: Concept of Generalized Index}.
Например, символом
\fi
$\Vector A_{[1]}$ мы будем обозначать
множество $\Vector{\Omega}$\Hyph алгебр $(A_2,...,A_n)$.
В соответствующем обозначении $(\VX A,\Vector f)$ башни
представлений подразумевается, что $\Vector f=(f_{2,3},...,f_{n-1,n})$.
\qed
\end{convention}

\begin{convention}
Так как мы пользуемся векторными обозначениями для элементов
башни представлений, необходимо соглашение о записи операций.
Предполагается, что операции выполняются покомпонентно. Например,
\ShowEq{vector notation in tower of representations}
\qed
\end{convention}
\fi

\ePrints{8443-0072,1111.6035,0906.0135,NewAffine,1102.5168,1305.4547,MIntegral}
\Items{1003.3714,4820-2669,MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Пусть $A$ - $\Omega_1$\Hyph алгебра.
Пусть $B$ - $\Omega_2$\Hyph алгебра.
Запись
\ShowEq{A->*B}
означает, что определено представление $\Omega_1$\Hyph алгебры $A$
в $\Omega_2$\Hyph алгебре $B$.
\qed
\end{convention}
\fi

\ePrints{0702.561,0707.2246,0803.2620}
\ifx\Semafor\ValueOn
\begin{convention}
Я пользуюсь стрелкой $\xymatrix{\arp[r]&}$
на диаграмме для обозначения проекции расслоения.
Я пользуюсь стрелкой $\xymatrix{\ars[r]&}$
на диаграмме для обозначения сечения расслоения.
\qed
\end{convention}
\fi

\ePrints{0912.3315}
\ifx\Semafor\ValueOn
\begin{remark}
Я считаю диаграммы отображений важным инструментом. Однако временами возникает
желание увидеть диаграмму трёх мерной, что увеличило бы её выразительную
мощность. Кто знает какие сюрпризы готовит будущее.
В 1992 на конференции в Казани я рассказывал своим коллегам
какие преимущества имеет компьютерная подготовка статей.
Спустя 8 лет из письма из Казани я узнал, что теперь можно
готовить статьи с помощью LaTeX.
\qed
\end{remark}
\fi

\ePrints{1001.4852,1003.1544,1006.2597,1011.3102}
\Items{Calculus.Paper}
\ifx\Semafor\ValueOn
\begin{convention}
Если в некотором выражении используется несколько
операций, среди которых есть операция $\circ$, то предполагается,
что операция $\circ$ выполняется первой.
Ниже приведен пример эквивалентных выражений.
\ShowEq{list circ expressions}
\qed
\end{convention}
\fi

%\ePrints{0906.0135,NewAffine}
%\ifx\Semafor\ValueOn
%\item
%Пусть $\VX X$ - базис башни представлений $(\Vector A,\Vector f)$.
%Мы будем называть $\Omega_n$\Hyph слово
%$w_n(\Vector f,\VX X,x_n)$ координатами $x_n\in A_n$
%относительно базиса $\VX X$.
%\fi

\ePrints{1107.1139}
\ifx\Semafor\ValueOn
\begin{convention}
Для данной $D$\Hyph алгебры $A$
левый сдвиг
\ShowEq{left shift, D algebra}
определён равенством
\ShowEq{left shift 1, D algebra}
и правый сдвиг
\ShowEq{right shift, D algebra}
определён равенством
\ShowEq{right shift 1, D algebra}
\qed
\end{convention}
\fi

\ePrints{MBasis}
\ifx\Semafor\ValueOn
\begin{convention}
Мы будем полагать,
что рассматриваемая мера является полной мерой.
\qed
\end{convention}
\fi

\ifx\PrintPaper\undefined
Без сомнения, у читателя могут быть вопросы,
замечания, возражения. Я буду признателен любому отзыву.
\fi



==> Index.Russian.tex <==
%auto-ignore
\OpenIndex
\SetIndexSpace%
\Index%1%1%1-форма
   {$1$\Hyph форма}%
   {1-form}%
\SetIndexSpace%
\Index%2%2%2- арное расслоенное отношение
   {$2$\Hyph арное расслоенное отношение}%
   {2 ary fibered relation}%
\SetIndexSpace%
\Index%819%A%A алгебра многочленов над D алгеброй
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Index%5%A%A- значная функция
   {$A$\Hyph значная функция}%
   {A valued function}%
\Index%693%A%A линейное отображение модулей
   {$A$\Hyph линейное отображение модулей}%
   {A linear map of modules}%
\Index%685%A%A- модуль
   {$A$\Hyph модуль}%
   {module over algebra}%
\Index%818%A%A число
   {$A$\Hyph число}%
   {A number}%
\Index%603%A%A(A) отображение
   {$\mathcal A(A)$\Hyph отображение}%
   {A(A) mapping}%
\Index%680%A%Acr линейное отображение модулей
   {\Acr линейное отображение модулей}%
   {Acr linear map of modules}%
\Index%764%A%ACRcirc линейная комбинация
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination}%
\Index%582%A%Arc базис в векторном пространстве
   {$A\RCstar$\Hyph базис в векторном пространстве}%
   {Arc basis, vector space}%
\Index%789%A%Astar антилинейное отображение алгебры с сопряжением
   {$A\star$\Hyph антилинейное отображение алгебры с сопряжением}%
   {antilinear mapping of algebra with conjugation}%
\Index%575%A%Astar векторное пространство
   {$A\star$\Hyph векторное пространство}%
   {Astar vector space}%
\Index%583%A%Astar линейное отображение векторных пространств
   {$A\star$\Hyph линейное отображение векторных пространств}%
   {Astar linear map of vector spaces}%
\Index%660%A%Astar- модуль
   {$A\star$\Hyph модуль}%
   {Astar-module}%
\Index%665%A%Astar- произведение вектора на скаляр
   {$A\star$\Hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, Astar module}%
\Index%579%A%Astar-произведение вектора на скаляр
   {$A\star$\hyph произведение вектора на скаляр}%
   {Astar product of vector over scalar, vector space}%
\Index%3%A%j i-CR квазидетерминант
   {$(^j_i)$\hyph \CR квазидетерминант}%
   {j i cr-quasideterminant}%
\SetIndexSpace%
\Index%799%B%b множество
   {$B$\Hyph множество}%
   {B set}%
\SetIndexSpace%
\Index%6%C%c строка матрицы
   {\subs строка матрицы}%
   {c row}%
\Index%7%C%CR матричная группа
   {\CR матричная группа}%
   {cr-matrix group}%
\Index%8%C%CR обратный элемент бикольца
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Index%9%C%CR произведение матриц
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Index%589%C%cr произведение матриц отображений
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Index%10%C%CR степень
   {\CR степень}%
   {cr power}%
\Index%11%C%crd векторное пространство
   {\crd векторное пространство}%
   {crd vector space}%
\Index%768%C%Cstar-алгебра
   {$C^*$\Hyph алгебра}%
   {Cstar-algebra}%
\Index%12%C%c-строка матрицы
   {$c$\hyph строка матрицы}%
   {c-row}%
\SetIndexSpace%
\Index%251%D%D- алгебра
   {$D$\Hyph алгебра}%
   {D algebra}%
\Index%549%D%D- аффинная связность на многообразии аффинной связности
   {$D$\Hyph аффинная связность на многообразии аффинной связности}%
   {D affine connection, affine manifold}%
\Index%23%D%d аффинное пространство
   {$D$\Hyph аффинное пространство}%
   {d affine space}%
\Index%14%D%D- вектор- функция
   {$D$\Hyph вектор\Hyph функция}%
   {d vector function}%
\Index%48%D%D- значная переменная
   {$D$\Hyph значная переменная}%
   {D valued variable}%
\Index%581%D%D линейный функционал
   {$D$\Hyph линейный функционал}%
   {D linear functional}%
\Index%584%D%D- модуль
   {$D$\Hyph модуль}%
   {D module}%
\Index%71%D%D- модуль
   {$D$\Hyph модуль}%
   {D-module}%
\Index%18%D%dcr векторное пространство
   {\dcr векторное пространство}%
   {dcr vector space}%
\Index%38%D%dcr производная Гато отображения f D- векторного пространства V в D- векторное пространство W
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Index%26%D%Drc базис в векторном расслоении
   {\Drc базис в векторном расслоении}%
   {drc basis, vector bundle}%
\Index%17%D%drc вектор
   {\drc вектор}%
   {drc vector}%
\Index%28%D%drc векторное пространство
   {\drc векторное пространство}%
   {drc vector space}%
\Index%19%D%drc векторное пространство r строк
   {\drc векторное пространство \subs строк}%
   {subs rows drc vector space}%
\Index%36%D%Drc линейное отображение векторных расслоений
   {\Drc линейное отображение векторных расслоений}%
   {drc linear map of vector bundles}%
\Index%70%D%drc представление группы
   {\drc представление группы}%
   {drc linear representation of group}%
\Index%779%D%Dstar антилинейное отображение кольца с сопряжением
   {$D\star$\Hyph антилинейное отображение кольца с сопряжением}%
   {antilinear mapping of ring with conjugation}%
\Index%771%D%Dstar антилинейный гомоморфизм
   {$D\star$\Hyph антилинейный гомоморфизм}%
   {Dstar antilinear homomorphism}%
\Index%39%D%Dstar- векторное поле
   {$\mathcal D\star$\Hyph векторное поле}%
   {Dstar vector field}%
\Index%41%D%Dstar- векторное расслоение
   {$\mathcal D\star$\Hyph векторное расслоение}%
   {Dstar vector bundle}%
\Index%769%D%Dstar линейный гомоморфизм
   {$D\star$\Hyph линейный гомоморфизм}%
   {Dstar linear homomorphism}%
\Index%46%D%Dstar производная Гато функции f тела D
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Index%47%D%Dstar производная Фреше отображения f тела D в точке x
   {\Ds производная Фреше отображения $f$ тела $D$ в точке $x$}%
   {Frechet Dstar derivative of map, division ring}%
\Index%40%D%Dstar-векторное пространство
   {$D\star$\hyph векторное пространство}%
   {Dstar vector space}%
\Index%43%D%Dstar-линейная комбинация векторных полей
   {$\mathcal D\star$\hyph линейная комбинация векторных полей}%
   {linear composition of vector fields}%
\Index%156%D%Dstar-модуль
   {$D\star$\Hyph модуль}%
   {Dstar-module}%
\Index%44%D%Dstar-произведение вектора на скаляр
   {$D\star$\hyph произведение вектора на скаляр}%
   {Dstar product of vector over scalar, vector space}%
\Index%45%D%Dstar-произведение векторного поля на скаляр
   {$\mathcal D\star$\hyph произведение векторного поля на скаляр}%
   {Dstar product of vector field over scalar, vector space}%
\Index%15%D%D-векторное пространство
   {$D$\hyph векторное пространство}%
   {D vector space}%
\Index%32%D%rcd линейная оболочка в векторном пространстве
   {\rcd линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\SetIndexSpace%
\Index%50%E%enhanced Lie group
   {enhanced Lie group}%
   {enhanced Lie group}%
\SetIndexSpace%
\Index%55%G%$G$\Hyph пространство
   {$G$\Hyph пространство}%
   {GSpace}%
\Index%52%G%G- система отсчёта
   {$G$\Hyph система отсчёта}%
   {G reference frame}%
\Index%53%G%G-basis векторного пространства
   {$G$\Hyph базис векторного пространства}%
   {G-basis}%
\Index%54%G%G-координаты базиса
   {$G$\Hyph координаты базиса}%
   {G-coordinates}%
\SetIndexSpace%
\Index%596%J%j i RCcirc квазидетерминант
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant}%
\Index%678%J%ji- квазидетерминант
   {$(ji)$\hyph квазидетерминант}%
   {j i quasideterminant}%
\SetIndexSpace%
\Index%57%M%m- вектор
   {$m$\Hyph вектор}%
   {m-vector}%
\Index%56%M%m- мерный параллепипед
   {$m$\Hyph мерный параллепипед}%
   {m dimensional parallelepiped}%
\SetIndexSpace%
\Index%726%N%n алгебра над кольцом
   {$n$\Hyph алгебра над кольцом}%
   {n algebra over ring}%
\Index%58%N%n- арное расслоенное отношение
   {$n$\Hyph арное расслоенное отношение}%
   {fibered relation}%
\SetIndexSpace%
\Index%4%R%j i-RC квазидетерминант
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant}%
\Index%728%R%R- модуль
   {$R$\Hyph модуль}%
   {R- module}%
\Index%59%R%r строка матрицы
   {\sups строка матрицы}%
   {r row}%
\Index%60%R%RC вырожденная матрица
   {\RC вырожденная матрица}%
   {RC singular matrix}%
\Index%61%R%RC главная минорная матрица
   {\RC главная минорная матрица}%
   {RC-major minor}%
\Index%62%R%RC квазидетерминант
   {\RC квазидетерминант}%
   {RC-quasideterminant}%
\Index%63%R%RC матричная группа
   {\RC матричная группа}%
   {rc-matrix group}%
\Index%64%R%RC невырожденная матрица
   {\RC невырожденная матрица}%
   {RC nonsingular matrix}%
\Index%65%R%RC обратный элемент бикольца
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Index%66%R%RC произведение матриц
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Index%590%R%rc произведение матриц отображений
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Index%67%R%RC ранг матрицы
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Index%68%R%RC степень
   {\RC степень}%
   {rc power}%
\Index%600%R%RCcirc вырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph вырожденная матрица $\mathcal A(A)$\Hyph отображений}%
   {RCcirc singular matrix of A(A) mappings}%
\Index%599%R%RCcirc вырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph вырожденная матрица эндоморфизмов}%
   {RCcirc singular matrix of endomorphisms}%
\Index%597%R%RCcirc квазидетерминант
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Index%601%R%RCcirc невырожденная матрица A(A) отображений
   {$\RCcirc$\Hyph невырожденная матрица $A(A)$\Hyph отображений}%
   {RCcirc nonsingular matrix of A(A) mappings}%
\Index%598%R%RCcirc невырожденная матрица эндоморфизмов
   {$\RCcirc$\Hyph невырожденная матрица эндоморфизмов}%
   {RCcirc nonsingular matrix of endomorphisms}%
\Index%602%R%RCcirc невырожденная система аддитивных уравнений
   {$\RCcirc$\Hyph невырожденная система аддитивных уравнений}%
   {RCcirc nonsingular system of additive equations}%
\Index%765%R%RCcircA линейная комбинация
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination}%
\Index%22%R%rcd автоморфизм векторного пространства
   {\rcd автоморфизм векторного пространства}%
   {automorphism of vector space}%
\Index%759%R%rcd аффинная плоскость
   {\rcd аффинная плоскость}%
   {rcd affine plane}%
\Index%736%R%rcd аффинное пространство
   {\rcd аффинное пространство}%
   {rcd affine space}%
\Index%111%R%rcd аффинный базис
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Index%27%R%rcd вектор
   {\rcd вектор}%
   {rcd vector}%
\Index%69%R%rcd векторное пространство
   {\rcd векторное пространство}%
   {rcd vector space}%
\Index%29%R%rcd векторное пространство c строк
   {\rcd векторное пространство \sups строк}%
   {sups rows rcd vector space}%
\Index%31%R%rcd изоморфизм векторных пространств
   {\rcd изоморфизм векторных пространств}%
   {isomorphism of vector spaces}%
\Index%37%R%rcd линейным Tstar- представление группы
   {\rcd линейным \Ts представление группы}%
   {rcd linear Tstar representation of group}%
\Index%13%R%rcd производная Гато отображения f D-векторного пространства V в D-векторное пространство W
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Index%72%R%r-строка матрицы
   {$r$\hyph строка матрицы}%
   {r-row}%
\Index%510%R%частная rcd производная Гато отображения fb по переменной xa
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map with respect to variable, D vector space}%
\SetIndexSpace%
\Index%73%S%RCstarS,RCstarT- линейное отображение векторных пространств
   {$(\RCstar S,\RCstar T)$\Hyph линейное отображение векторных пространств}%
   {rcs rct linear map of vector spaces}%
\Index%74%S%SRCstar,TRCstar- линейное отображение векторных расслоений
   {$(\mathcal S\RCstar,\mathcal T\RCstar)$\Hyph линейное отображение векторных расслоений}%
   {src trc linear map of vector bundles}%
\Index%112%S%Sstar, star T-бимодуль
   {($S\star$, $\star T$)\hyph бимодуль}%
   {(Sstar,starT)-bimodule}%
\Index%669%S%star A- модуль
   {$\star A$\Hyph модуль}%
   {starA-module}%
\Index%78%S%star D-векторное пространство
   {$\star D$\hyph векторное пространство}%
   {starD-vector space}%
\Index%79%S%star R-модуль
   {$\star R$\hyph модуль}%
   {starR-module}%
\Index%674%S%starA- произведение вектора на скаляр
   {$\star A$\Hyph произведение вектора на скаляр}%
   {starA product of vector over scalar, starA module}%
\Index%735%S%starD аффинное пространство
   {$\star D$\Hyph аффинное пространство}%
   {starD affine space}%
\Index%192%S%starD- векторное пространство
   {$\star D$\Hyph векторное пространство}%
   {starD vector space}%
\Index%76%S%starD производная Гато функции f тела D
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Index%198%S%starD-произведение вектора на скаляр
   {$\star D$\hyph произведение вектора на скаляр}%
   {starD product of vector over scalar, vector space}%
\Index%82%S%starT- представление Omega1 алгебры A в Omega2 алгебре M
   {\sT представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {starT representation of algebra}%
\Index%83%S%starT- представление расслоенной Omega- алгебры
   {\sT представление расслоенной $\Omega$\Hyph алгебры}%
   {starT representation of fibered Omega-algebra}%
\Index%84%S%starT- представление расслоенной группы
   {\sT представление расслоенной группы}%
   {starT representation of fibered group}%
\Index%85%S%starT- преобразование
   {\sT преобразование}%
   {starT transformation}%
\Index%86%S%starT- преобразование расслоения
   {\sT преобразование расслоения}%
   {starT transformation of bundle}%
\Index%80%S%starT- сдвиг
   {\sT сдвиг}%
   {starT shift}%
\Index%81%S%starT- сдвиг на расслоении групп
   {\sT сдвиг на расслоении групп}%
   {starT shift, fibered group}%
\SetIndexSpace%
\Index%823%T%T_1 пространство
   {$T_1$\Hyph пространство}%
   {T1 space}%
\Index%87%T%Tstar- векторное пространство матриц
   {\Ts векторное пространство матриц}%
   {matrices vector space}%
\Index%90%T%Tstar- представление Omega1 алгебры A в Omega2 алгебре M
   {\Ts представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {Tstar representation of algebra}%
\Index%91%T%Tstar- представление расслоенной Omega- алгебры
   {\Ts представление расслоенной $\Omega$\Hyph алгебры}%
   {Tstar representation of fibered Omega-algebra}%
\Index%92%T%Tstar- преобразование
   {\Ts преобразование}%
   {Tstar transformation}%
\Index%93%T%Tstar- преобразование расслоения
   {\Ts преобразование расслоения}%
   {Tstar transformation of bundle}%
\Index%89%T%Tstar- сдвиг
   {\Ts сдвиг}%
   {Tstar shift}%
\SetIndexSpace%
\Index%645%А%абелевая Omega группа
   {абелевая $\Omega$\Hyph группа}%
   {Abelian Omega group}%
\Index%560%А%автоморфизм башни представлений
   {автоморфизм башни представлений}%
   {automorphism of tower of representations}%
\Index%94%А%автоморфизм представления Omega алгебры
   {автоморфизм представления $\Omega$\Hyph алгебры}%
   {automorphism of representation}%
\Index%95%А%автопараллельная кривая
   {автопараллельная кривая}%
   {auto parallel line}%
\Index%805%А%аддитивное отображение
   {аддитивное отображение}%
   {additive map}%
\Index%99%А%активное starT- представление
   {активное \sT представление}%
   {active representation, vector space}%
\Index%100%А%активное представление
   {активное представление}%
   {active representation}%
\Index%716%А%активное представление группы в многообразии базисов башни представлений
   {активное представление группы $G(\Vector  f)$ в многообразии базисов  башни представлений}%
   {active representation in basis manifold, tower of representations}%
\Index%569%А%активное представление группы в многообразии базисов представления
   {активное представление группы $G(f)$ в многообразии базисов представления}%
   {active representation in basis manifold}%
\Index%715%А%активное преобразование многообразия базисов башни представлений
   {активное преобразование многообразия базисов башни представлений}%
   {active transformation of basis, tower of representations}%
\Index%326%А%активное преобразование многообразия базисов представления
   {активное преобразование многообразия базисов представления}%
   {active transformation of basis, representation}%
\Index%101%А%активное преобразование на многообразии базисов
   {активное преобразование на многообразии базисов}%
   {active transformation}%
\Index%102%А%активное преобразование на множестве rcd базисов
   {активное преобразование на множестве \rcd базисов}%
   {active transformation, vector space}%
\Index%103%А%алгебра E кватернионов над полем F
   {алгебра $E$ кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Index%808%А%алгебра Бореля
   {алгебра Бореля}%
   {Borel algebra}%
\Index%104%А%алгебра Ли группы Ли
   {алгебра Ли группы Ли}%
   {algebra Lie group Lie}%
\Index%487%А%алгебра многочленов над D алгеброй
   {алгебра многочленов над $D$\Hyph алгеброй}%
   {algebra of polynomials over D algebra}%
\Index%797%А%алгебра множеств
   {алгебра множеств}%
   {algebra of sets}%
\Index%607%А%алгебра над кольцом
   {алгебра над кольцом}%
   {algebra over ring}%
\Index%639%А%алгебра октонионов
   {алгебра октонионов}%
   {octonion algebra}%
\Index%618%А%алгебра рациональных отображений алгебры
   {алгебра рациональных отображений алгебры}%
   {algebra of rational mappings of algebra}%
\Index%780%А%алгебра с сопряжением
   {алгебра с сопряжением}%
   {algebra with conjugation}%
\Index%786%А%алгебра скаляров алгебры
   {алгебра скаляров алгебры}%
   {scalar algebra of algebra}%
\Index%775%А%алгебра скаляров кольца
   {алгебра скаляров кольца}%
   {scalar algebra of ring}%
\Index%400%А%алгебра частных алгебры с сопряжением
   {алгебра частных алгебры с сопряжением}%
   {algebra of fractions of algebra with conjugation}%
\Index%623%А%алгебра, противоположная алгебре
   {алгебра, противоположная алгебре $P$}%
   {opposite algebra}%
\Index%105%А%альтернативное представление матрицы
   {альтернативное представление матрицы}%
   {Alternative representation}%
\Index%106%А%антигомоморфизм расслоенных групп
   {антигомоморфизм расслоенных групп}%
   {antihomomorphism of fibered groups}%
\Index%107%А%антисимметричное 2- арное расслоенное отношение
   {антисимметричное $2$\Hyph арное расслоенное отношение}%
   {antisymmetric 2 ary fibered relation}%
\Index%108%А%арность операции
   {арность операции}%
   {arity of operation}%
\Index%617%А%ассоциативная D алгебра
   {ассоциативная $D$\Hyph алгебра}%
   {associative D algebra}%
\Index%832%А%ассоциативная Omega группа
   {ассоциативная $\Omega$\Hyph группа}%
   {associative Omega group}%
\Index%616%А%ассоциатор D алгебры
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Index%733%А%аффинная структура на множестве
   {аффинная структура на множестве}%
   {affine structure on set}%
\Index%682%А%аффинное представление группы Ли
   {аффинное представление группы Ли}%
   {affine representation of Lie group}%
\Index%758%А%аффинное преобразование
   {аффинное преобразование}%
   {affine transformation}%
\Index%109%А%аффинное преобразование на многообразии базисов
   {аффинное преобразование на многообразии базисов}%
   {affine transformation}%
\Index%734%А%аффинное пространство
   {аффинное пространство}%
   {affine space}%
\Index%110%А%аффинный базис
   {аффинный базис}%
   {Affine Basis}%
\Index%842%А%аффинный функционал
   {аффинный функционал}%
   {affine functional}%
\SetIndexSpace%
\Index%113%Б%база отображения
   {база отображения}%
   {base of map}%
\Index%114%Б%база расслоенного соответствия
   {база расслоенного соответствия}%
   {base of fibered correspondence}%
\Index%16%Б%базис drc векторного пространства r строк
   {базис \drc векторного пространства \subs строк}%
   {basis, r rows drc vector space}%
\Index%653%Б%базис алгебры L(A;A)
   {базис алгебры $\mathcal L(A;A)$}%
   {basis of algebra L(A,A)}%
\Index%567%Б%базис башни представлений
   {базис башни представлений}%
   {basis of tower of representations}%
\Index%197%Б%базис в D векторном пространстве
   {базис в $D$\Hyph векторном пространстве}%
   {basis, D vector space}%
\Index%24%Б%базис в rcd векторном пространстве
   {базис в \rcd векторном пространстве}%
   {basis, rcd vector space}%
\Index%25%Б%базис в rcd векторном пространстве c строк
   {базис в \rcd векторном пространстве \sups строк}%
   {basis, c rows rcd vector space}%
\Index%115%Б%базис векторного пространства
   {базис векторного пространства}%
   {Basis}%
\Index%783%Б%базис Гамеля
   {базис Гамеля}%
   {Hamel basis}%
\Index%659%Б%базис модуля
   {базис модуля}%
   {basis, module}%
\Index%329%Б%базис представления
   {базис представления}%
   {basis of representation}%
\Index%791%Б%базис Шаудера
   {базис Шаудера}%
   {Schauder basis}%
\Index%223%Б%базис, двойственный базису
   {базис, двойственный базису}%
   {dual basis}%
\Index%49%Б%базис, дуальный базису
   {базис, дуальный базису}%
   {basis dual to basis}%
\Index%116%Б%базовый вектор представления группы Ли над алгеброй A
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Index%118%Б%базовый оператор группы Ли
   {базовый оператор группы Ли}%
   {Lie group basic operators}%
\Index%503%Б%банахова D- алгебра
   {банахова $D$\Hyph алгебра}%
   {Banach algebra}%
\Index%313%Б%банаховый D- модуль
   {банаховый $D$\Hyph модуль}%
   {Banach module}%
\Index%531%Б%башня подпредставлений
   {башня подпредставлений}%
   {tower of subrepresentations}%
\Index%532%Б%башня подпредставлений башни представлений, порождённая кортежем множеств
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%
\Index%119%Б%башня представлений Omega алгебр
   {башня представлений $\Vector{\Omega}$\Hyph алгебр}%
   {tower of representations of algebras}%
\Index%120%Б%башня расслоений
   {башня расслоений}%
   {tower of bundles}%
\Index%324%Б%башня эффективных представлений
   {башня эффективных представлений}%
   {tower of effective representations}%
\Index%121%Б%бесконечно малый генератор представления
   {бесконечно малый генератор представления}%
   {infinitesimal generator}%
\Index%122%Б%бикольцо
   {бикольцо}%
   {biring}%
\Index%798%Б%борелевское множество
   {борелевское множество}%
   {Borel set}%
\Index%803%Б%борелевское отображение
   {борелевское отображение}%
   {Borel-measurable map}%
\SetIndexSpace%
\Index%123%В%вектор Киллинга второго рода
   {вектор Киллинга второго рода}%
   {Killing vector second type}%
\Index%782%В%вектор отображения
   {вектор отображения}%
   {vector of mapping}%
\Index%785%В%вектор элемента алгебры
   {вектор элемента алгебры}%
   {vector of algebra}%
\Index%774%В%вектор элемента кольца
   {вектор элемента кольца}%
   {vector of ring}%
\Index%727%В%векторное пространство над полем
   {векторное пространство над полем}%
   {vector space over field}%
\Index%125%В%векторное расслоение
   {векторное расслоение}%
   {vector bundle}%
\Index%126%В%векторный потенциал
   {векторный потенциал}%
   {vector potential}%
\Index%124%В%вектор-столбец
   {вектор\hyph столбец}%
   {column vector}%
\Index%127%В%вектор-строка
   {вектор\hyph строка}%
   {row vector}%
\Index%847%В%вертикальная компонента вектора
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Index%849%В%вертикальное подпространство
   {вертикальное подпространство}%
   {vertical subspace}%
\Index%850%В%вертикальный вектор
   {вертикальный вектор}%
   {vertical vector}%
\Index%128%В%вполне интегрируемая система
   {вполне интегрируемая система}%
   {completely integrable system}%
\Index%651%В%времениподобный вектор
   {времениподобный вектор}%
   {timelike vector}%
\Index%829%В%всюду плотное множество
   {всюду плотное множество}%
   {everywhere dense subset}%
\Index%830%В%вторая аксиома счётности
   {вторая аксиома счётности}%
   {second axiom of countability}%
\Index%129%В%второй закон Ньютона
   {второй закон Ньютона}%
   {Second Newton law}%
\Index%838%В%выпуклое множество
   {выпуклое множество}%
   {convex set}%
\Index%130%В%вырожденное линейное отображение
   {вырожденное линейное отображение}%
   {singular linear map}%
\SetIndexSpace%
\Index%132%Г%геометрический объект в векторном пространстве
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Index%133%Г%геометрический объект в координатном представлении
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Index%698%Г%геометрический объект в координатном представлении, определённом в Omega_2- алгебре
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Index%134%Г%геометрический объект в координатном представлении, определённом в rcd векторном пространстве
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Index%719%Г%геометрический объект в координатном представлении, определённом в кортеже Omega- алгебр
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Index%704%Г%геометрический объект типа
   {геометрический объект типа $H$}%
   {geometric object of type H, representation g}%
\Index%135%Г%геометрический объект типа A
   {геометрический объект типа $A$ в векторном пространстве}%
   {geometric object of type A, vector space}%
\Index%700%Г%геометрический объект, определённый в Omega_2- алгбре
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Index%136%Г%геометрический объект, определённый в rcd векторном пространстве
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Index%722%Г%геометрический объект, определённый в кортеже Omega- алгебр
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Index%767%Г%главный идеал
   {главный идеал}%
   {principal ideal}%
\Index%137%Г%голономные координаты вектора
   {голономные координаты вектора}%
   {vector holonomic coordinates}%
\Index%138%Г%голономные координаты связности
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Index%140%Г%гомоморфизм расслоенных групп
   {гомоморфизм расслоенных групп}%
   {homomorphism of fibered groups}%
\Index%139%Г%гомоморфизм расслоенных универсальных алгебр
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Index%848%Г%горизонтальная компонента вектора
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Index%851%Г%горизонтальное подпространство
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Index%852%Г%горизонтальный вектор
   {горизонтальный вектор}%
   {horizontal vector}%
\Index%568%Г%группа автоморфизмов представления
   {группа автоморфизмов представления}%
   {group of automorphisms of representation}%
\Index%141%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%142%Г%группа аффинных преобразований
   {группа аффинных преобразований}%
   {affine transformation group}%
\Index%845%Г%группа линейных преобразований
   {группа линейных преобразований}%
   {linear transformation group}%
\Index%143%Г%группа симметрии
   {группа симметрии}%
   {symmetry group}%
\Index%144%Г%группа симметрии
   {группа симметрии}%
   {SymmetryGroup}%
\Index%145%Г%группа стабилизации
   {группа стабилизации}%
   {stability group}%
\Index%146%Г%групповая алгебра
   {групповая алгебра}%
   {group algebra}%
\SetIndexSpace%
\Index%147%Д%движение на многообразии базисов
   {движение на многообразии базисов}%
   {movement transformation}%
\Index%586%Д%движение пространства Минковского
   {движение пространства Минковского}%
   {motion, Minkowski space}%
\Index%755%Д%двойной определитель
   {двойной определитель}%
   {double determinant}%
\Index%148%Д%декартова степень A множества B
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Index%149%Д%декартова степень A расслоения B
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Index%594%Д%декартова степень n H алгебры
   {декартова степень $n$ $\mathfrak{H}$\Hyph алгебры}%
   {Cartesian power of algebra}%
\Index%150%Д%декартова степень n расслоения E
   {декартова степень $n$ расслоения $\Bundle E$}%
   {Cartesian power n of bundle E}%
\Index%855%Д%декартово произведение мер
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Index%151%Д%декартово произведение расслоений
   {декартово произведение расслоений}%
   {Cartesian product of bundles}%
\Index%152%Д%декартово произведение расслоенных пространств
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces}%
\Index%820%Д%делитель многочлена
   {делитель многочлена}%
   {divisor of polynomial}%
\Index%814%Д%делитель нуля
   {делитель нуля}%
   {zero divisor}%
\Index%153%Д%диагональ в расслоении
   {диагональ в расслоении}%
   {diagonal in bundle}%
\Index%725%Д%диаграмма представлений
   {диаграмма представлений}%
   {diagram of representations}%
\Index%154%Д%диаграмма соответствий
   {диаграмма соответствий}%
   {diagram of correspondences}%
\Index%157%Д%дифференциал Гато отображения
   {дифференциал Гато отображения}%
   {Gateaux differential of map}%
\Index%159%Д%дуальное пространство к rcd векторному пространству
   {дуальное пространство к \rcd векторному пространству}%
   {dual space of rcd vector space}%
\SetIndexSpace%
\Index%796%Е%единица кольца множеств
   {единица кольца множеств}%
   {unit of ring of sets}%
\Index%315%Е%единичная сфера в алгебре
   {единичная сфера в $D$\Hyph алгебре}%
   {unit sphere in algebra}%
\Index%160%Е%единичная сфера в теле
   {единичная сфера в теле}%
   {unit sphere in division ring}%
\Index%523%Е%единичный вектор
   {единичный вектор}%
   {unit vector}%
\Index%837%Е%единичный интервал
   {единичный интервал}%
   {unit interval}%
\SetIndexSpace%
\Index%576%З%закон ассоциативности для Astar- векторного пространства
   {закон ассоциативности для $A\star$\Hyph векторного пространства}%
   {associative law, Astar vector space}%
\Index%585%З%закон ассоциативности для Astar линейных отображений векторных пространств
   {закон ассоциативности для $A\star$\Hyph линейных отображений векторных пространств}%
   {associative law for Astar linear mappings of vector spaces}%
\Index%662%З%закон ассоциативности для Astar- модуля
   {закон ассоциативности для $A\star$\Hyph модуля}%
   {associative law, Astar module over algebra}%
\Index%654%З%закон ассоциативности для D- модуля
   {закон ассоциативности для $D$\Hyph модуля}%
   {associative law, D module}%
\Index%162%З%закон ассоциативности для Drc линейных отображений векторных расслоений
   {закон ассоциативности для \Drc линейных отображений векторных расслоений}%
   {associative law for drc linear maps of vector bundles}%
\Index%163%З%закон ассоциативности для Dstar- векторного пространства
   {закон ассоциативности для $D\star$\Hyph векторного пространства}%
   {associative law, Dstar vector space}%
\Index%164%З%закон ассоциативности для Dstar- векторных полей
   {закон ассоциативности для $\mathcal D\star$\Hyph векторных полей}%
   {associative law, Dstar vector fields}%
\Index%161%З%закон ассоциативности для rcd линейных отображений векторных пространств
   {закон ассоциативности для \rcd линейных отображений векторных пространств}%
   {associative law for rcd linear maps of vector spaces}%
\Index%671%З%закон ассоциативности для starA- модуля
   {закон ассоциативности для $\star A$\Hyph модуля}%
   {associative law, starA module over algebra}%
\Index%501%З%закон ассоциативности для starD- векторного пространства
   {закон ассоциативности для $\star D$\Hyph векторного пространства}%
   {associative law, starD vector space}%
\Index%165%З%закон ассоциативности для ковариантного starT- представления
   {закон ассоциативности для ковариантного \sT представления}%
   {associative law for covariant starT representation}%
\Index%166%З%закон ассоциативности для ковариантного Tstar- представления
   {закон ассоциативности для ковариантного \Ts представления}%
   {associative law for covariant Tstar representation}%
\Index%167%З%закон ассоциативности для парных представлений
   {закон ассоциативности для парных представлений}%
   {associative law for twin representations}%
\Index%168%З%закон ассоциативности произведения расслоенных соответствий
   {закон ассоциативности произведения расслоенных соответствий}%
   {associative law, composition of fibered correspondences}%
\Index%577%З%закон дистрибутивности для Astar- векторного пространства
   {закон дистрибутивности для $A\star$\Hyph векторного пространства}%
   {distributive law, Astar vector space}%
\Index%663%З%закон дистрибутивности для Astar- модуля
   {закон дистрибутивности для $A\star$\Hyph модуля}%
   {distributive law, Astar module over algebra}%
\Index%655%З%закон дистрибутивности для D- модуля
   {закон дистрибутивности для $D$\Hyph модуля}%
   {distributive law, D module}%
\Index%169%З%закон дистрибутивности для Dstar- векторного пространства
   {закон дистрибутивности для $D\star$\Hyph векторного пространства}%
   {distributive law, Dstar vector space}%
\Index%170%З%закон дистрибутивности для Dstar- векторных полей
   {закон дистрибутивности для $\mathcal D\star$\Hyph векторных полей}%
   {distributive law, Dstar vector fields}%
\Index%672%З%закон дистрибутивности для starA- модуля
   {закон дистрибутивности для $\star A$\Hyph модуля}%
   {distributive law, starA module over algebra}%
\Index%625%З%закон дистрибутивности для starD- векторного пространства
   {закон дистрибутивности для $\star D$\Hyph векторного пространства}%
   {distributive law, starD vector space}%
\Index%578%З%закон унитарности для Astar- векторного пространства
   {закон унитарности для $A\star$\Hyph векторного пространства}%
   {unitarity law, Astar vector space}%
\Index%664%З%закон унитарности для Astar- модуля
   {закон унитарности для $A\star$\Hyph модуля}%
   {unitarity law, Astar module over algebra}%
\Index%656%З%закон унитарности для D- модуля
   {закон унитарности для $D$\Hyph модуля}%
   {unitarity law, D module}%
\Index%171%З%закон унитарности для Dstar- векторного пространства
   {закон унитарности для $D\star$\Hyph векторного пространства}%
   {unitarity law, Dstar vector space}%
\Index%172%З%закон унитарности для Dstar- векторных полей
   {закон унитарности для $\mathcal D\star$\Hyph векторных полей}%
   {unitarity law, Dstar vector fields}%
\Index%673%З%закон унитарности для starA- модуля
   {закон унитарности для $\star A$\Hyph модуля}%
   {unitarity law, starA module over algebra}%
\Index%199%З%закон унитарности для starD- векторного пространства
   {закон унитарности для $\star D$\Hyph векторного пространства}%
   {unitarity law, starD vector space}%
\Index%807%З%замкнутый шар
   {замкнутый шар}%
   {closed ball}%
\Index%825%З%замыкание множества
   {замыкание множества}%
   {closure of set}%
\SetIndexSpace%
\Index%459%И%идеал алгебры
   {идеал алгебры}%
   {ideal of algebra}%
\Index%800%И%измеримое отображение
   {измеримое отображение}%
   {measurable map}%
\Index%266%И%изоморфизм представлений Omega- алгебры
   {изоморфизм представлений $\Omega$\Hyph алгебры}%
   {isomorphism of repesentations of Omega algebra}%
\Index%173%И%изоморфизм расслоенных Omega- алгебр
   {изоморфизм расслоенных $\Omega$\Hyph алгебр}%
   {isomorphism of fibered Omega-algebras}%
\Index%648%И%изотропный вектор
   {изотропный вектор}%
   {isotropic vector}%
\Index%745%И%инволюция в кватернионной алгебре
   {инволюция в кватернионной алгебре}%
   {involution, quaternion algebra}%
\Index%844%И%интеграл отображения
   {интеграл отображения}%
   {integral of map}%
\Index%843%И%интегрируемое отображение
   {интегрируемое отображение}%
   {integrable map}%
\Index%174%И%инфинитезимальные образующие группы Ли
   {инфинитезимальные образующие группы Ли}%
   {infinitesimal generators of group Lie}%
\SetIndexSpace%
\Index%175%К%категория drc векторных пространств
   {категория \drc векторных пространств}%
   {category of drc vector spaces}%
\Index%176%К%категория Tstar- представлений Omega1 алгебры A
   {категория \Ts представлений $\Omega$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Index%177%К%категория Tstar- представлений Omega1 алгебры из категории A
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Index%178%К%категория приведенных расслоенных соответствий
   {категория приведенных расслоенных соответствий}%
   {category of reduced fibered correspondences}%
\Index%179%К%категория расслоенных соответствий над диагональю
   {категория расслоенных соответствий над диагональю}%
   {category of fibered correspondences over diagonal}%
\Index%555%К%квадратичная форма на теле
   {квадратичная форма на теле}%
   {quadratic form, division ring}%
\Index%551%К%квадратичное отображение тела
   {квадратичное отображение тела}%
   {Quadratic Map of Division Ring}%
\Index%180%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine transformation}%
\Index%181%К%квазиаффинное преобразование на многообразии базисов
   {квазиаффинное преобразование на многообразии базисов}%
   {quasi affine drc transformation}%
\Index%182%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement, division ring}%
\Index%183%К%квазидвижение на многообразии базисов
   {квазидвижение на многообразии базисов}%
   {quasi movement}%
\Index%75%К%квазидвижение пространства Минковского
   {квазидвижение пространства Минковского}%
   {Quasimotion, Minkowski space}%
\Index%679%К%квазидетерминант
   {квазидетерминант}%
   {quasideterminant definition}%
\Index%604%К%квазизамкнутое кольцо отображений
   {квазизамкнутое кольцо отображений}%
   {quasiclosed ring of mappings}%
\Index%746%К%кватернион, сопряженный к кватерниону
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Index%741%К%кватернионная алгебра
   {кватернионная алгебра}%
   {quaternion algebra}%
\Index%184%К%ковариантное starT- представление группы
   {ковариантное \sT представление группы}%
   {covariant starT representation of group}%
\Index%185%К%ковариантное starT- представление расслоенной группы
   {ковариантное \sT представление расслоенной группы}%
   {covariant starT representation of fibered group}%
\Index%186%К%ковариантное Tstar- представление группы
   {ковариантное \Ts представление группы}%
   {covariant Tstar representation of group}%
\Index%187%К%ковариантное Tstar- представление расслоенной группы
   {ковариантное \Ts представление расслоенной группы}%
   {covariant Tstar representation of fibered group}%
\Index%188%К%кольцо имеет характеристику 0
   {кольцо имеет характеристику $0$}%
   {ring has characteristic 0}%
\Index%189%К%кольцо имеет характеристику p
   {кольцо имеет характеристику $p$}%
   {ring has characteristic p}%
\Index%794%К%кольцо множеств
   {кольцо множеств}%
   {ring of sets}%
\Index%778%К%кольцо с сопряжением
   {кольцо с сопряжением}%
   {ring with conjugation}%
\Index%615%К%коммутативная D алгебра
   {коммутативная $D$\Hyph алгебра}%
   {commutative D algebra}%
\Index%190%К%коммутативная диаграмма соответствий
   {коммутативная диаграмма соответствий}%
   {commutative diagram of correspondences}%
\Index%614%К%коммутатор D алгебры
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Index%815%К%компактное множество
   {компактное множество}%
   {compact set}%
\Index%191%К%компактно-открытая топология
   {компактно\hyph открытая топология}%
   {compact open topology}%
\Index%193%К%компонента линейного отображения
   {компонента линейного отображения}%
   {component of linear map}%
\Index%647%К%компонента полилинейного отображения
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Index%629%К%компонента производной Гато
   {компонента производной Гато}%
   {component of Gateaux derivative}%
\Index%633%К%компонента производной Гато второго порядка
   {компонента производной Гато второго порядка}%
   {component of Gateaux derivative of Second Order}%
\Index%202%К%контравариантное starT- представление группы
   {контравариантное \sT представление группы}%
   {contravariant starT representation of group}%
\Index%200%К%контравариантное starT- представление расслоенной группы
   {контравариантное \sT представление расслоенной группы}%
   {contravariant starT representation of fibered group}%
\Index%201%К%контравариантное Tstar- представление группы
   {контравариантное \Ts представление группы}%
   {contravariant Tstar representation of group}%
\Index%203%К%контравариантное Tstar- представление расслоенной группы
   {контравариантное \Ts представление расслоенной группы}%
   {contravariant Tstar representation of fibered group}%
\Index%691%К%координатная матрица вектора
   {координатная матрица вектора}%
   {coordinate matrix of vector}%
\Index%205%К%координатная матрица векторного поля в Drc базисе
   {координатная матрица векторного поля в \Drc базисе}%
   {coordinate matrix of vector field in drc basis}%
\Index%206%К%координатная матрица множества векторов
   {координатная матрица множества векторов}%
   {coordinate matrix of set of vectors}%
\Index%208%К%координатная система отсчёта
   {координатная система отсчёта}%
   {coordinate reference frame}%
\Index%210%К%координатное Drc векторное расслоение
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Index%209%К%координатное rcd векторное пространство
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Index%211%К%координатное векторное пространство
   {координатное векторное пространство}%
   {coordinate vector space}%
\Index%697%К%координатное представление в Omega_2- алгебре
   {координатное представление в $\Omega_2$\Hyph алгебре}%
   {coordinate representation, Omega_2 algebra}%
\Index%212%К%координатное представление в rcd векторном пространстве
   {координатное представление в \rcd векторном пространстве}%
   {coordinate representation, rcd vector space}%
\Index%720%К%координатное представление в кортеже Omega- алгебр
   {координатное представление в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinate tower of representations, Omega algebra}%
\Index%213%К%координатное представление группы в векторном пространстве
   {координатное представление группы в векторном пространстве}%
   {coordinate representation, vector space}%
\Index%214%К%координатный rcd изоморфизм
   {координатный \rcd изоморфизм}%
   {coordinate rcd isomorphism}%
\Index%215%К%координатный изоморфизм
   {координатный изоморфизм}%
   {coordinate isomorphism}%
\Index%325%К%координаты базиса представления
   {координаты базиса представления}%
   {coordinates of basis relative to basis, representation}%
\Index%216%К%координаты вектора
   {координаты вектора}%
   {coordinates of vector}%
\Index%286%К%координаты вектора относительно базиса Гамеля
   {координаты вектора относительно базиса Гамеля}%
   {coordinates of vector, Hamel basis}%
\Index%676%К%координаты вектора относительно базиса Шаудера
   {координаты вектора относительно базиса Шаудера}%
   {coordinates of vector, Schauder basis}%
\Index%217%К%координаты векторного поля в Drc базисе
   {координаты векторного поля в \Drc базисе}%
   {coordinates of vector field in drc basis}%
\Index%218%К%координаты геометрического объекта
   {координаты геометрического объекта}%
   {coordinates of geometric object, vector space}%
\Index%701%К%координаты геометрического объекта в Omega_2- алгбре
   {координаты геометрического объекта в $\Omega_2$\Hyph алгбре $M$}%
   {coordinates of geometric object, representation g}%
\Index%219%К%координаты геометрического объекта в rcd векторном пространстве
   {координаты геометрического объекта в \rcd векторном пространстве}%
   {coordinates of geometric object, rcd vector space}%
\Index%220%К%координаты геометрического объекта в координатном rcd векторном пространстве
   {координаты геометрического объекта в координатном \rcd векторном пространстве}%
   {coordinates of geometric object, coordinate rcd vector space}%
\Index%221%К%координаты геометрического объекта в координатном представлении
   {координаты геометрического объекта в координатном представлении}%
   {coordinates of geometric object, coordinate vector space}%
\Index%721%К%координаты геометрического объекта в координатном пространстве башни представлений
   {координаты геометрического объекта в координатном пространстве башни представлений}%
   {coordinates of geometric object, coordinate tower of representations}%
\Index%699%К%координаты геометрического объекта в координатном пространстве представления
   {координаты геометрического объекта в координатном пространстве представления}%
   {coordinates of geometric object, coordinate representation}%
\Index%723%К%координаты геометрического объекта в кортеже Omega- алгебр
   {координаты геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {coordinates of geometric object, tower of representations g}%
\Index%222%К%координаты множества векторов
   {координаты множества векторов}%
   {coordinates of set of vectors}%
\Index%224%К%координаты представления
   {координаты представления}%
   {coordinates of representation, drc vector space}%
\Index%225%К%координаты представления
   {координаты представления}%
   {coordinates of representation}%
\Index%737%К%координаты точки rcd аффинного пространства относительно базиса
   {координаты точки \rcd аффинного пространства относительно базиса}%
   {coordinates in rcd affine space}%
\Index%730%К%координаты точки аффинного пространства относительно базиса
   {координаты точки $A$ аффинного пространства $\overset{\circ}{A}$ относительно базиса $(O,\Basis e)$}%
   {coordinates in affine space}%
\Index%558%К%координаты элемента представления относительно множества
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Index%711%К%координаты эндоморфизма башни представлений
   {координаты эндоморфизма башни представлений}%
   {coordinates of endomorphism, tower of representations}%
\Index%696%К%координаты эндоморфизма представления
   {координаты эндоморфизма представления}%
   {coordinates of endomorphism, representation}%
\Index%634%К%корень полинома
   {корень полинома}%
   {root of polynomial}%
\Index%708%К%кортеж Omega слов элементов башни представления относительно кортежа множеств образующих
   {кортеж $\Vector{\Omega}$\Hyph слов элемента башни представления относительно кортежа множеств образующих}%
   {tuple of words relative to tuple of generating sets, tower of representations}%
\Index%535%К%кортеж координат элемента относительно кортежа множеств
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Index%533%К%кортеж множеств образующих башни подпредставлений
   {кортеж множеств образующих башни подпредставлений}%
   {tuple of generating sets of tower subrepresentations}%
\Index%534%К%кортеж множеств образующих башни представлений
   {кортеж множеств образующих башни представлений}%
   {tuple of generating sets of tower of representations}%
\Index%713%К%кортеж отношений эквивалентности, порождённых башней представлений
   {кортеж отношений эквивалентности, порождённых башней представлений $\Vector f$}%
   {tuple of equivalence of tower of representations}%
\Index%530%К%кортеж стабильных множеств башни представлений
   {кортеж стабильных множеств башни представлений}%
   {tuple of stable sets of tower of representations}%
\Index%226%К%косое произведение векторов
   {косое произведение векторов}%
   {skew product of vectors}%
\Index%821%К%коэффициент многочлена
   {коэффициент многочлена}%
   {coefficient of polynomial}%
\Index%550%К%коэффициенты D- аффинной связности на многообразии
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Index%538%К%коэффициенты связности в D аффинном пространстве
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Index%227%К%кривизна Картана
   {кривизна Картана}%
   {Cartan curvature}%
\Index%537%К%криволинейные координаты точки аффинного пространства
   {криволинейные координаты точки аффинного пространства}%
   {curvilinear coordinates of point in affine space}%
\SetIndexSpace%
\Index%33%Л%Drc линейно независимые векторные поля
   {линейно независимые векторные поля}%
   {linearly independent vector fields}%
\Index%158%Л%левая дробь
   {левая дробь}%
   {left fraction}%
\Index%754%Л%левое алгебраическое дополнение элемента матрицы
   {левое алгебраическое дополнение элемента матрицы}%
   {left cofactor, matrix}%
\Index%228%Л%левое векторное пространство
   {левое векторное пространство}%
   {left vector space}%
\Index%756%Л%левое двойное алгебраическое дополнение элемента матрицы
   {левое двойное алгебраическое дополнение элемента матрицы}%
   {left double cofactor}%
\Index%229%Л%левоинвариантное векторное поле
   {левоинвариантное векторное поле}%
   {left invariant vector}%
\Index%230%Л%левостороннее ковариантное представление группы
   {левостороннее ковариантное представление группы}%
   {left-side covariant representation of group}%
\Index%231%Л%левостороннее контравариантное представление группы
   {левостороннее контравариантное представление группы}%
   {left-side contravariant representation of group}%
\Index%232%Л%левостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {левостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {left-side representation of algebra}%
\Index%233%Л%левостороннее представление расслоенной Omega- алгебры
   {левостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {left-side representation of fibered Omega-algebra}%
\Index%234%Л%левостороннее преобразование
   {левостороннее преобразование}%
   {left-side transformation}%
\Index%235%Л%левостороннее преобразование расслоения
   {левостороннее преобразование расслоения}%
   {left-side transformation of bundle}%
\Index%236%Л%левые структурные константы алгебры Ли
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Index%513%Л%левый главный идеал
   {левый главный идеал}%
   {left principal ideal}%
\Index%812%Л%левый делитель нуля
   {левый делитель нуля}%
   {left zero divisor}%
\Index%681%Л%левый идеал алгебры
   {левый идеал алгебры}%
   {left ideal of algebra}%
\Index%237%Л%левый модуль нaд кольцом
   {левый модуль нaд кольцом $D$}%
   {left module over ring}%
\Index%661%Л%левый модуль над D- алгеброй A
   {левый модуль над $D$\Hyph алгеброй $A$}%
   {left module over algebra}%
\Index%731%Л%левый сдвиг R- модуля
   {левый сдвиг $R$\Hyph модуля}%
   {left shift of module}%
\Index%238%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift}%
\Index%239%Л%левый сдвиг на группе
   {левый сдвиг на группе}%
   {left shift, group}%
\Index%240%Л%левый сдвиг на расслоении групп
   {левый сдвиг на расслоении групп}%
   {Tstar shift, fibered group}%
\Index%88%Л%линейная комбинация векторов
   {линейная комбинация векторов}%
   {linear combination of  vectors}%
\Index%686%Л%линейная комбинация векторов A- модуля
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Index%98%Л%линейнное отображение, порождённое отображением
   {линейное отображение, порождённое отображением}%
   {linear map generated by map}%
\Index%688%Л%линейно зависимое множество A- модуля
   {линейно зависимое множество $A$\Hyph модуля}%
   {linear dependent vectors, module}%
\Index%20%Л%линейно зависимые векторные поля
   {линейно зависимые векторные поля}%
   {linearly dependent vector fields}%
\Index%21%Л%линейно зависимые векторы
   {линейно зависимые векторы}%
   {linearly dependent vectors}%
\Index%687%Л%линейно независимое множество A- модуля
   {линейно независимое множество $A$\Hyph модуля}%
   {linear independent vectors, module}%
\Index%34%Л%линейно независимые векторы
   {линейно независимые векторы}%
   {linearly independent vectors}%
\Index%613%Л%линейное отображение
   {линейное отображение}%
   {linear map}%
\Index%398%Л%линейное отображение D векторных пространств
   {линейное отображение $D$\Hyph векторных пространств}%
   {linear map of D vector spaces}%
\Index%35%Л%линейное отображение rcd векторных пространств
   {линейное отображение \rcd векторных пространств}%
   {linear map of rcd vector spaces}%
\Index%97%Л%линейное отображение тела
   {линейное отображение тела}%
   {linear map of division ring}%
\Index%244%Л%линейное представление группы
   {линейное представление группы}%
   {linear representation of group}%
\Index%608%Л%линейное представление группы Ли
   {линейное представление группы Ли}%
   {linear representation of Lie group}%
\Index%740%Л%линейное преобразование rcd аффинного пространства
   {линейное преобразование \rcd аффинного пространства}%
   {linear transformation, rcd affine space}%
\Index%630%Л%линейный геометрический объект
   {линейный геометрический объект}%
   {linear geometric object}%
\Index%397%Л%линейный функционал
   {линейный функционал}%
   {linear functional}%
\Index%245%Л%лифт отображения
   {лифт отображения}%
   {lift of map}%
\Index%246%Л%лифт соответствия
   {лифт соответствия}%
   {lift of correspondence}%
\Index%247%Л%локальная система отсчёта
   {локальная система отсчёта}%
   {local reference frame}%
\Index%248%Л%локально компактное в точке p пространство
   {локально компактное в точке $p$ пространство}%
   {locally compact at point space}%
\Index%249%Л%локально компактное пространство
   {локально компактное пространство}%
   {locally compact space}%
\SetIndexSpace%
\Index%250%М%малая группа
   {малая группа}%
   {little group}%
\Index%772%М%матрица антилинейного гомоморфизма
   {матрица антилинейного гомоморфизма}%
   {matrix of antilinear homomorphism}%
\Index%252%М%матрица билинейной функции
   {матрица билинейной функции}%
   {matrix of bilinear function}%
\Index%552%М%матрица квадратичного отображения
   {матрица квадратичного отображения}%
   {matrix of quadratic map, division ring}%
\Index%770%М%матрица линейного гомоморфизма
   {матрица линейного гомоморфизма}%
   {matrix of linear homomorphism}%
\Index%194%М%матрица линейного отображения
   {матрица линейного отображения}%
   {matrix of linear map}%
\Index%591%М%матрица линейных отображений
   {матрица линейных отображений}%
   {matrix of linear mappings}%
\Index%588%М%матрица отображений
   {матрица отображений}%
   {matrix of mappings}%
\Index%253%М%матрица расслоенного Drc линейного отображения
   {матрица расслоенного \Drc линейного отображения}%
   {matrix of fibered drc linear map}%
\Index%595%М%матрица эндоморфизмов Omega алгебры
   {матрица эндоморфизмов $\Omega$\Hyph алгебры}%
   {matrix of endomorphisms of Omega algebra}%
\Index%527%М%матрица Якоби Гато отображения
   {матрица Якоби\Hyph Гато отображения}%
   {Jacobi Gateaux matrix of map}%
\Index%254%М%метрико-аффинное многообразие
   {метрико-аффинное многообразие}%
   {metric-affine manifold}%
\Index%96%М%метрический тензор в пространстве Минковского
   {метрический тензор в пространстве Минковского}%
   {metric tensor, Minkowski space}%
\Index%642%М%минорная матрица
   {минорная матрица}%
   {minor matrix}%
\Index%556%М%многообразие D- аффинной связности
   {многообразие $D$\Hyph аффинной связности}%
   {manifold with D- affine connections}%
\Index%257%М%многообразие базисов \rcd аффинного пространства
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Index%255%М%многообразие базисов rcd векторного пространства
   {многообразие базисов \rcd векторного пространства}%
   {basis manifold of rcd vector space}%
\Index%256%М%многообразие базисов аффинного пространства
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Index%714%М%многообразие базисов башни представлений
   {многообразие базисов башни представлений}%
   {basis manifold tower of representations}%
\Index%258%М%многообразие базисов векторного пространства
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Index%259%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space}%
\Index%260%М%многообразие базисов евклидова пространства
   {многообразие базисов евклидова пространства}%
   {Basis Manifold, Euclid Space, division ring}%
\Index%536%М%многообразие базисов представления
   {многообразие базисов представления}%
   {basis manifold representation F algebra}%
\Index%261%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space, division ring}%
\Index%262%М%многообразие базисов центро-аффинного пространства
   {многообразие базисов центро-аффинного пространства}%
   {Basis Manifold, Central Affine Space}%
\Index%263%М%многообразие систем отсчёта
   {многообразие систем отсчёта}%
   {reference frame manifold}%
\Index%804%М%многочлен
   {многочлен}%
   {polynomial}%
\Index%571%М%множество Omega_2- слов представления
   {множество $\Omega_2$\Hyph слов представления}%
   {word set of representation}%
\Index%562%М%множество координат представления
   {множество координат представления}%
   {coordinate set of representation}%
\Index%709%М%множество кортежей Omega- слов башни представлений
   {множество кортежей $\Vector\Omega$\Hyph слов башни представлений}%
   {word set of tower of representations}%
\Index%563%М%множество кортежей координат башни представлений
   {множество кортежей координат башни представлений}%
   {coordinate set of tower of representations}%
\Index%626%М%множество нулей алгебры
   {множество нулей алгебры}%
   {set of zeros of algebra}%
\Index%331%М%множество образующих подпредставления
   {множество образующих подпредставления}%
   {generating set of subrepresentation}%
\Index%332%М%множество образующих представления
   {множество образующих представления}%
   {generating set of representation}%
\Index%628%М%множество обратимых элементов алгебры
   {множество обратимых элементов алгебры}%
   {set of invertible elements of algebra}%
\Index%828%М%множество, плотное в множестве
   {множество, плотное в множестве}%
   {dense in set}%
\Index%787%М%модуль векторов алгебры
   {модуль векторов алгебры}%
   {vector module of algebra}%
\Index%776%М%модуль векторов кольца
   {модуль векторов кольца}%
   {vector module of ring}%
\Index%611%М%модуль над кольцом
   {модуль над кольцом}%
   {module over ring}%
\Index%264%М%морфизм Tstar- представлений расслоенной Omega- алгебры
   {морфизм \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {morphism of representations of fibered Omega algebra}%
\Index%265%М%морфизм из башни Tstar- представлений в башню Tstar- представлений
   {морфизм из башни \Ts представлений в башню \Ts представлений}%
   {morphism from tower of representations into tower of representations}%
\Index%267%М%морфизм представлений Omega1 алгебры в Omega2 алгебре
   {морфизм представлений $\Omega_1$\Hyph алгебры в $\Omega_2$\Hyph алгебре}%
   {morphism of representations of Omega1 algebra in Omega2 algebra}%
\Index%268%М%морфизм представлений из f в g
   {морфизм представлений из $f$ в $g$}%
   {morphism of representations from f into g}%
\Index%732%М%морфизм представления f
   {морфизм представления $f$}%
   {morphism of representation f}%
\Index%269%М%морфизм расслоенных Tstar- представлений из F в G
   {морфизм расслоенных \Ts представлений из $\Bundle F$ в $\Bundle G$}%
   {morphism of fibered representations from f into g}%
\Index%831%М%открытое множество
   {открытое множество}%
   {open set}%
\SetIndexSpace%
\Index%763%Н%направление над коммутативным кольцом
   {направление над коммутативным кольцом}%
   {direction over commutative ring}%
\Index%738%Н%начало системы координат star D аффинного пространства
   {начало системы координат $\star D$\Hyph аффинного пространства}%
   {origin of coordinate system of starD affine space}%
\Index%729%Н%начало системы координат аффинного пространства
   {начало системы координат аффинного пространства}%
   {origin of coordinate system of affine space}%
\Index%649%Н%не полная Omega алгебра
   {не полная $\Omega$\Hyph алгебра}%
   {not complete Omega algebra}%
\Index%632%Н%не полная группа
   {не полная группа}%
   {not complete group}%
\Index%272%Н%невырожденная билинейная функция
   {невырожденная билинейная функция}%
   {nonsingular bilinear function}%
\Index%273%Н%невырожденная система drc линейных уравнений
   {невырожденная система \rcd линейных уравнений}%
   {nonsingular system of linear equations}%
\Index%553%Н%невырожденное квадратичное отображение тела
   {невырожденное квадратичное отображение тела}%
   {regular quadratic map, division ring}%
\Index%274%Н%невырожденное преобразование
   {невырожденное преобразование}%
   {nonsingular transformation}%
\Index%643%Н%невырожденный тензор
   {невырожденный тензор}%
   {nonsingular tensor}%
\Index%330%Н%невырожденный эндоморфизм представления
   {невырожденный эндоморфизм представления}%
   {regular endomorphism of representation}%
\Index%275%Н%неголономная координата
   {неголономная координата}%
   {anholonomic coordinate}%
\Index%276%Н%неголономные координаты вектора
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Index%277%Н%неголономные координаты на многообразии
   {неголономные координаты на многообразии}%
   {anholonomic coordinates on manifold}%
\Index%278%Н%неголономные координаты связности
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Index%835%Н%независимые точки
   {независимые точки}%
   {independent points}%
\Index%279%Н%неметричность
   {неметричность}%
   {nonmetricity}%
\Index%280%Н%непрерывное отображение
   {непрерывное отображение}%
   {continuous map}%
\Index%610%Н%непрерывное отображение нескольких переменных
   {непрерывное отображение нескольких переменных}%
   {continuous multivariable map}%
\Index%281%Н%непрерывное соответствие
   {непрерывное соответствие}%
   {continuous correspondence}%
\Index%668%Н%непрерывный базис
   {непрерывный базис}%
   {continues basis}%
\Index%346%Н%норма в D- алгебре
   {норма в $D$\Hyph алгебре}%
   {norm on D algebra}%
\Index%460%Н%норма в D-модуле
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Index%742%Н%норма в кватернионной алгебре
   {норма в кватернионной алгебре}%
   {norm, quaternion algebra}%
\Index%282%Н%норма кватерниона
   {норма кватерниона}%
   {norm of quaternion}%
\Index%283%Н%норма на D- векторном пространстве
   {норма на $D$\Hyph векторном пространстве}%
   {norm on D vector space}%
\Index%675%Н%норма на Omega группе
   {норма на $\Omega$\Hyph группе}%
   {norm on Omega group}%
\Index%641%Н%норма на кольце
   {норма на кольце}%
   {norm on ring}%
\Index%284%Н%норма на теле
   {норма на теле}%
   {absolute value on division ring}%
\Index%657%Н%норма операции
   {норма операции}%
   {norm of operation}%
\Index%314%Н%норма отображения
   {норма отображения}%
   {norm of map}%
\Index%285%Н%норма полилинейного отображения
   {норма полилинейного отображения}%
   {norm of polymap}%
\Index%801%Н%норма представления
   {норма представления}%
   {norm of representation}%
\Index%196%Н%норма функционала
   {норма функционала}%
   {norm of functional}%
\Index%343%Н%нормированная D-алгебра
   {нормированная $D$\Hyph алгебра}%
   {normed D algebra}%
\Index%792%Н%нормированная Omega группа
   {нормированная $\Omega$\Hyph группа}%
   {normed Omega group}%
\Index%287%Н%нормированное D-векторное пространство
   {нормированное $D$\Hyph векторное пространство}%
   {normed D vector space}%
\Index%640%Н%нормированное кольцо
   {нормированное кольцо}%
   {normed ring}%
\Index%288%Н%нормированное тело
   {нормированное тело}%
   {valued division ring}%
\Index%364%Н%нормированный D-модуль
   {нормированный $D$\Hyph модуль}%
   {normed D module}%
\Index%692%Н%нормированный базис
   {нормированный базис}%
   {normal basis}%
\SetIndexSpace%
\Index%289%О%образующая линейного отображения
   {образующая линейного отображения}%
   {generator of linear map}%
\Index%290%О%обратное приведенное расслоенное соответствие
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence}%
\Index%291%О%обратное расслоенное соответствие
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence}%
\Index%292%О%обращение Адамара матрицы
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Index%293%О%объект неголономности
   {объект неголономности}%
   {anholonomity object}%
\Index%294%О%однородное отображение степени k над полем F
   {однородное отображение степени $k$ над полем $F$}%
   {homogeneous map of degree over field, D vector space}%
\Index%295%О%однородное пространство группы
   {однородное пространство группы}%
   {homogeneous space of group}%
\Index%296%О%однородное расслоение расслоенной группы
   {однородное расслоение расслоенной группы}%
   {homogeneous bundle of fibered group}%
\Index%631%О%однородный линейный геометрический объект
   {однородный линейный геометрический объект}%
   {homogeneous linear geometric object}%
\Index%689%О%однородный многочлен степени
   {однородный многочлен степени $n$}%
   {homogeneous polynomial of power}%
\Index%297%О%однотранзитивное представление Omega- алгебры A
   {однотранзитивное представление $\Omega$\Hyph алгебры $A$}%
   {single transitive representation of algebra}%
\Index%298%О%однотранзитивное представление группы
   {однотранзитивное представление группы}%
   {single transitive representation of group}%
\Index%299%О%однотранзитивное представление расслоенной Omega- алгебры
   {однотранзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {single transitive representation of fibered Omega-algebra}%
\Index%766%О%одночлен степени
   {одночлен степени $k$}%
   {monomial of power}%
\Index%300%О%операция на расслоении
   {операция на расслоении}%
   {operation on bundle}%
\Index%301%О%определённая слева алгебра Ли группы Ли
   {определённая слева алгебра Ли группы Ли}%
   {left defined Lie algebra}%
\Index%302%О%определённая справа алгебра Ли группы Ли
   {определённая справа алгебра Ли группы Ли}%
   {right defined Lie algebra}%
\Index%303%О%определитель матрицы
   {определитель матрицы}%
   {determinant}%
\Index%304%О%орбита Tstar- представления группы
   {орбита \Ts представления группы}%
   {orbit of Tstar  representation of group}%
\Index%624%О%орбита линейного отображения
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Index%305%О%орбита представления группы
   {орбита представления группы}%
   {orbit of representation of group}%
\Index%306%О%орбита представления расслоенной группы
   {орбита представления расслоенной группы}%
   {orbit of representation of fibered group}%
\Index%636%О%ортогональность в пространстве Минковского
   {ортогональность в пространстве Минковского}%
   {Minkowski orthogonality}%
\Index%637%О%ортогональный базис в пространстве Минковского
   {ортогональный базис в пространстве Минковского}%
   {orthogonal basis, Minkowski space}%
\Index%307%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Index%308%О%ортонормированный базис
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Index%638%О%ортонормированный базис в пространстве Минковского
   {ортонормированный базис в пространстве Минковского}%
   {orthonormal basis, Minkowski space}%
\Index%309%О%отклонение траекторий
   {отклонение траекторий}%
   {deviation of trajectories}%
\Index%793%О%открытый шар
   {открытый шар}%
   {open ball}%
\Index%706%О%отношение эквивалентности порождённое представлением
   {отношение эквивалентности, порождённое представлением $f$}%
   {equivalence of representation}%
\Index%502%О%отображение n D- значных переменных
   {отображение $\gi n$ $D$\Hyph значных переменных}%
   {map of n D valued variables}%
\Index%312%О%отображение колец полилинейное над коммутативным кольцом
   {отображение колец полилинейное над коммутативным кольцом}%
   {map polylinear over commutative ring, ring}%
\Index%316%О%отображение типа G на многообразии
   {отображение типа $G$ на многообразии}%
   {map of type G on manifold}%
\Index%505%О%отображение, дифференцируемое по Гато
   {отображение, дифференцируемое по Гато}%
   {map differentiable in Gateaux sense}%
\Index%506%О%отображение, непрерывное по совокупности аргументов
   {отображение, непрерывное по совокупности аргументов}%
   {map continuous with respect to set of arguments}%
\Index%572%О%отображение, полилинейное над конечномерными алгебрами
   {отображение, полилинейное над конечномерными алгебрами}%
   {map polylinear over finite dimensional algebras}%
\Index%677%О%отображение, проективное над коммутативным кольцом
   {отображение, проективное над коммутативным кольцом}%
   {map projective over commutative ring}%
\SetIndexSpace%
\Index%317%П%параллелограмм
   {параллелограмм}%
   {parallelogram}%
\Index%739%П%параллельный сдвиг rcd аффинного пространства
   {параллельный сдвиг \rcd аффинного пространства}%
   {parallel shift, rcd affine space}%
\Index%684%П%парные представления D- алгебры
   {парные представления $D$\Hyph алгебры}%
   {twin representations of D algebra}%
\Index%587%П%парные представления ассоциативной алгебры
   {парные представления ассоциативной алгебры}%
   {twin representations of associative algebra}%
\Index%318%П%парные представления группы
   {парные представления группы}%
   {twin representations of group}%
\Index%319%П%парные представления расслоенной группы
   {парные представления расслоенной группы}%
   {twin representations of fibered group}%
\Index%320%П%парные представления тела
   {парные представления тела}%
   {twin representations of division ring}%
\Index%321%П%пассивное starT- представление
   {пассивное \sT представление}%
   {passive starT representation}%
\Index%333%П%пассивное представление
   {пассивное представление}%
   {passive representation}%
\Index%718%П%пассивное представление группы в многообразии базисов башни представлений
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов башни представлений}%
   {passive representation in basis manifold, tower of representations}%
\Index%695%П%пассивное представление группы в многообразии базисов представления
   {пассивное представление группы $G(f)$ в многообразии базисов представления}%
   {passive representation in basis manifold}%
\Index%717%П%пассивное преобразование многообразия базисов башни представлений
   {пассивное преобразование многообразия базисов башни представлений}%
   {passive transformation of basis, tower of representations}%
\Index%570%П%пассивное преобразование многообразия базисов представления
   {пассивное преобразование многообразия базисов представления}%
   {passive transformation of basis, representation}%
\Index%335%П%пассивное преобразование на многообразии базисов
   {пассивное преобразование на многообразии базисов}%
   {passive transformation}%
\Index%336%П%пассивное преобразование на множестве rcd базисов
   {пассивное преобразование на множестве \rcd базисов}%
   {passive transformation, vector space}%
\Index%337%П%первый закон Ньютона
   {первый закон Ньютона}%
   {First Newton law}%
\Index%338%П%перенос Картана
   {перенос Картана}%
   {Cartan transport}%
\Index%339%П%перенос Френе
   {перенос Френе}%
   {Frenet transport}%
\Index%827%П%подгруппа Omega группы
   {подгруппа $\Omega$\Hyph группы}%
   {subgroup of Omega group}%
\Index%334%П%подпредставление представления
   {подпредставление представления}%
   {subrepresentation of representation}%
\Index%322%П%подпредставление, порождённое множеством X
   {подпредставление, порождённое множеством $X$}%
   {subrepresentation generated by set}%
\Index%340%П%подрасслоение
   {подрасслоение}%
   {subbundle}%
\Index%341%П%подрасслоение Dstar-векторного расслоения
   {подрасслоение $\mathcal D\star$\hyph векторного расслоения}%
   {subbundle of Dstar vector bundle}%
\Index%806%П%полиаддитивное отображение
   {полиаддитивное отображение}%
   {polyadditive map}%
\Index%345%П%полиалинейное косо симметричное отображение
   {полиалинейное косо симметричное отображение}%
   {polylinear map skew symmetric}%
\Index%344%П%поливектор
   {поливектор}%
   {polyvector}%
\Index%609%П%полилинейное отображение
   {полилинейное отображение}%
   {polylinear map}%
\Index%347%П%полилинейное симметричное отображение
   {полилинейное симметричное отображение}%
   {polylinear map symmetric}%
\Index%760%П%полиморфизм представлений
   {полиморфизм представлений}%
   {polymorphism of representations}%
\Index%853%П%полная мера
   {полная мера}%
   {complete measure}%
\Index%811%П%полная нормированная Omega группа
   {полная нормированная $\Omega$\Hyph группа}%
   {complete Omega group}%
\Index%348%П%полная система линейных дифференциальных уравнений в частных производны
   {полная система линейных дифференциальных уравнений в частных производны}%
   {Complete System of Linear Partial Differential Equations}%
\Index%270%П%полное кольцо
   {полное кольцо}%
   {complete ring}%
\Index%349%П%полное тело
   {полное тело}%
   {complete division ring}%
\Index%826%П%пополнение нормированной Omegaгруппы
   {пополнение нормированной $\Omega$\Hyph группы}%
   {completion of normed Omega group}%
\Index%834%П%пополнение представления
   {пополнение представления}%
   {completion of representation}%
\Index%241%П%последовательность Коши
   {последовательность Коши}%
   {Cauchy sequence}%
\Index%816%П%последовательность сходится
   {последовательность сходится}%
   {sequence converges}%
\Index%854%П%последовательность сходится почти всюду
   {последовательность сходится почти всюду}%
   {converges almost everywhere}%
\Index%817%П%последовательность сходится равномерно
   {последовательность сходится равномерно}%
   {sequence converges uniformly}%
\Index%352%П%потенциальная энергия
   {потенциальная энергия}%
   {potential energy}%
\Index%30%П%правая дробь
   {правая дробь}%
   {right fraction}%
\Index%753%П%правое алгебраическое дополнение элемента матрицы
   {правое алгебраическое дополнение элемента матрицы}%
   {right cofactor, matrix}%
\Index%353%П%правое векторное пространство
   {правое векторное пространство}%
   {right vector space}%
\Index%757%П%правое двойное алгебраическое дополнение элемента матрицы
   {правое двойное алгебраическое дополнение элемента матрицы}%
   {right double cofactor}%
\Index%354%П%правоинвариантное векторное поле
   {правоинвариантное векторное поле}%
   {right invariant vector}%
\Index%355%П%правостороннее ковариантное представление группы
   {правостороннее ковариантное представление группы}%
   {right-side covariant representation of group}%
\Index%356%П%правостороннее контравариантное представление группы
   {правостороннее контравариантное представление группы}%
   {right-side contravariant representation of group}%
\Index%357%П%правостороннее представление Omega1 алгебры A в Omega2 алгебре M
   {правостороннее представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {right-side representation of algebra}%
\Index%358%П%правостороннее представление расслоенной Omega- алгебры
   {правостороннее представление расслоенной $\Omega$\Hyph алгебры}%
   {right-side representation of fibered Omega-algebra}%
\Index%359%П%правостороннее преобразование
   {правостороннее преобразование}%
   {right-side transformation}%
\Index%360%П%правые структурные константы алгебры Ли
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Index%242%П%правый главный идеал
   {правый главный идеал}%
   {right principal ideal}%
\Index%813%П%правый делитель нуля
   {правый делитель нуля}%
   {right zero divisor}%
\Index%42%П%правый идеал алгебры
   {правый идеал алгебры}%
   {right ideal of algebra}%
\Index%361%П%правый модуль нaд кольцом
   {правый модуль нaд кольцом $D$}%
   {right module over ring}%
\Index%362%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift}%
\Index%363%П%правый сдвиг на группе
   {правый сдвиг на группе}%
   {right shift, group}%
\Index%670%П%праый модуль над D- алгеброй A
   {правый модуль над $D$\Hyph алгеброй $A$}%
   {right module over algebra}%
\Index%467%П%предел последовательности
   {предел последовательности}%
   {limit of sequence}%
\Index%365%П%предел соответствия по фильтру
   {предел соответствия по фильтру}%
   {limit of correspondence with respect to the filter}%
\Index%366%П%предел фильтра
   {предел фильтра}%
   {limit of filter}%
\Index%367%П%предельное множество фильтра
   {предельное множество фильтра}%
   {limit set of filter}%
\Index%702%П%представитель геометрического объекта в drc векторном пространстве
   {представитель геометрического объекта в \drc векторном пространстве}%
   {representative of geometric object, drc vector space}%
\Index%703%П%представитель геометрического объекта в Omega_2- алгбре
   {представитель геометрического объекта в $\Omega_2$\Hyph алгбре}%
   {representative of geometric object, representation g}%
\Index%368%П%представитель геометрического объекта в rcd векторном пространстве
   {представитель геометрического объекта в \rcd векторном пространстве}%
   {representative of geometric object, rcd vector space}%
\Index%369%П%представитель геометрического объекта в векторном пространстве
   {представитель геометрического объекта в векторном пространстве}%
   {representative of geometric object, vector space}%
\Index%724%П%представитель геометрического объекта в кортеже Omega- алгебр
   {представитель геометрического объекта в кортеже $\VX\Omega$\Hyph алгебр}%
   {representative of geometric object, tower of representations g}%
\Index%370%П%представление Omega- алгебры A в категории B
   {представление $\Omega$\Hyph алгебры $A$ в категории $\mathcal B$}%
   {representation of Omega algebra in category}%
\Index%529%П%представление Omega алгебры в башне представлений
   {представление $\Omega$\Hyph алгебры в башне представлений}%
   {representation of Omega algebra in tower of representations}%
\Index%528%П%представление Omega алгебры в представлении
   {представление $\Omega$\Hyph алгебры в представлении}%
   {representation of Omega algebra in representation}%
\Index%371%П%представление Omega1 алгебры A в Omega2 алгебре M
   {представление $\Omega_1$\Hyph алгебры $A$ в $\Omega_2$\Hyph алгебре $M$}%
   {representation of algebra}%
\Index%372%П%представление группы
   {представление группы}%
   {representation of group}%
\Index%117%П%представление, сопряжённое представлению
   {представление, сопряжённое представлению}%
   {representation conjugated to representation}%
\Index%373%П%преобразование Лоренца
   {преобразование Лоренца}%
   {Lorentz transformation}%
\Index%375%П%преобразование расслоения
   {преобразование расслоения}%
   {transformation of bundle}%
\Index%374%П%преобразование универсальной алгебры
   {преобразование универсальной алгебры}%
   {transformation of universal algebra}%
\Index%376%П%преобразование, согласованное с эквивалентностью 
   {преобразование, согласованное с эквивалентностью }%
   {transformation coordinated with equivalence}%
\Index%377%П%приведенное декартово произведение расслоений
   {приведенное декартово произведение расслоений}%
   {reduced Cartesian product of bundles}%
\Index%378%П%приведенное декартово произведение расслоенных пространств
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces}%
\Index%380%П%приведенное расслоенное соответствие в A
   {приведенное расслоенное соответствие в $\Bundle{A}$}%
   {reduced fibered correspondence in A}%
\Index%379%П%приведенное расслоенное соответствие из A в B
   {приведенное расслоенное соответствие из $\mathcal{A}$ в $\Bundle{B}$}%
   {reduced fibered correspondence from A to B}%
\Index%761%П%приведенный полиморфизм представлений
   {приведенный полиморфизм представлений}%
   {reduced polymorphism of representations}%
\Index%381%П%приводимое бикольцо
   {приводимое бикольцо}%
   {reducible biring}%
\Index%382%П%принцип двойственности для бикольца
   {принцип двойственности для бикольца}%
   {duality principle for biring}%
\Index%383%П%принцип двойственности для бикольца матриц
   {принцип двойственности для бикольца матриц}%
   {duality principle for biring of matrices}%
\Index%705%П%принцип инвариантности в \drc векторном пространстве
   {принцип инвариантности в \drc векторном пространстве}%
   {invariance principle}%
\Index%710%П%принцип инвариантности в башне представлений универсальных алгебр
   {принцип инвариантности в башне представлений универсальных алгебр}%
   {invariance principle, tower of representations g}%
\Index%385%П%принцип инвариантности в векторном пространстве
   {принцип инвариантности в векторном пространстве}%
   {invariance principle, vector space}%
\Index%384%П%принцип инвариантности в представлении универсальной алгебры
   {принцип инвариантности в представлении универсальной алгебры}%
   {invariance principle, representation g}%
\Index%386%П%продолжение соответствия
   {продолжение соответствия}%
   {extension of correspondence}%
\Index%195%П%проективное отображение непрерывно по направлению над полем
   {проективное отображение непрерывно по направлению над полем}%
   {projective map is continuous in direction over field}%
\Index%387%П%проекция расслоения E вдоль слоя E
   {проекция расслоения $\Bundle E$ вдоль слоя $E$}%
   {projection of bundle along fiber}%
\Index%388%П%произведение геометрического объекта и константы
   {произведение геометрического объекта и константы}%
   {product of geometric object and constant}%
\Index%389%П%произведение геометрического объекта и константы в векторном пространстве
   {произведение геометрического объекта и константы в векторном пространстве}%
   {product of geometric object and constant, vector space}%
\Index%390%П%произведение групп
   {произведение групп}%
   {product of groups}%
\Index%683%П%произведение линейного отображения на скаляр
   {произведение линейного отображения на скаляр}%
   {product of linear map over scalar}%
\Index%856%П%произведение мер
   {произведение мер}%
   {product of measures}%
\Index%666%П%произведение многочленов
   {произведение многочленов}%
   {product of polynomials}%
\Index%392%П%произведение морфизмов Tstar- представлений расслоенной Omega- алгебры
   {произведение морфизмов \Ts представлений расслоенной $\Omega$\Hyph алгебры}%
   {product of morphisms of representations of fibered Omega algebra}%
\Index%561%П%произведение морфизмов башни представлений
   {произведение морфизмов башни представлений}%
   {product of morphisms of tower of representations}%
\Index%391%П%произведение морфизмов представлений универсальной алгебры
   {произведение морфизмов представлений универсальной алгебры}%
   {product of morphisms of representations of universal algebra}%
\Index%271%П%произведение отображения на скаляр
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Index%393%П%произведение приведенных расслоенных соответствий
   {произведение приведенных расслоенных соответствий}%
   {composition of reduced fibered correspondences}%
\Index%394%П%произведение расслоенных соответствий
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Index%395%П%произведением объектов в категории
   {произведением объектов в категории}%
   {product of objects in category}%
\Index%396%П%производная Гато второго порядка
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Index%627%П%производная Гато отображения
   {производная Гато отображения}%
   {Gateaux derivative of map}%
\Index%399%П%производная Гато порядка n
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Index%401%П%производная Картана
   {производная Картана}%
   {Cartan derivative}%
\Index%402%П%производная Ли
   {производная Ли}%
   {Lie derivative}%
\Index%403%П%производная Ли метрики
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Index%404%П%производная Ли связности
   {производная Ли связности}%
   {Lie derivative of connection}%
\Index%810%П%простое отображение
   {простое отображение}%
   {simple map}%
\Index%405%П%простой поливектор
   {простой поливектор}%
   {simple polyvector}%
\Index%342%П%пространственноподобный вектор
   {пространственноподобный вектор}%
   {spacelike vector}%
\Index%635%П%пространство Минковского
   {пространство Минковского}%
   {Minkowski space, Finsler}%
\Index%406%П%пространство орбит Tstar- представления
   {пространство орбит \Ts представления}%
   {space of orbits of Ts representation}%
\Index%407%П%пространство отображений
   {пространство отображений}%
   {mapping space}%
\Index%408%П%противоположная расслоенная предупорядоченность
   {противоположная расслоенная предупорядоченность}%
   {opposite fibered preordering}%
\Index%409%П%прямая сумма представлений
   {прямая сумма представлений}%
   {direct sum of representations}%
\Index%410%П%прямое произведение D- векторных пространств
   {прямое произведение $D$\Hyph векторных пространств}%
   {direct product of D vector spaces}%
\Index%411%П%прямое произведение rcd векторных пространств
   {прямое произведение \rcd векторных пространств}%
   {direct product, rcd vector space}%
\Index%412%П%прямое произведение Tstar- представлений группы
   {прямое произведение \Ts представлений группы}%
   {direct product of Tstar representations of group}%
\Index%413%П%прямое произведение представлений группы
   {прямое произведение представлений группы}%
   {direct product of representations of group}%
\Index%414%П%прямое произведение представлений расслоенной группы
   {прямое произведение представлений расслоенной группы}%
   {direct product of representations of fibered group}%
\Index%415%П%прямое произведение тел
   {прямое произведение тел}%
   {direct product of division rings}%
\Index%540%П%псевдоэвклидова метрика на теле
   {псевдоэвклидова метрика на теле}%
   {pseudo-Euclidean metric on division ring}%
\Index%548%П%псевдоэвклидово скалярное произведение в D- векторном пространстве
   {псевдоэвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {pseudo-Euclidean scalar product, vector space}%
\Index%543%П%псевдоэвклидово скалярное произведение на теле
   {псевдоэвклидово скалярное произведение на теле}%
   {pseudo-Euclidean scalar product on division ring}%
\Index%416%П%пфаффова производная
   {пфаффова производная}%
   {pfaffian derivative}%
\SetIndexSpace%
\Index%204%Р%разложение вектора относительно базиса сходится
   {разложение вектора относительно базиса сходится}%
   {expansion converges}%
\Index%621%Р%разложение вектора относительно базиса сходится нормально
   {разложение вектора относительно базиса сходится нормально}%
   {expansion converges normally}%
\Index%417%Р%размерность rcd векторного пространства
   {размерность \rcd векторного пространства}%
   {dimension of vector space}%
\Index%554%Р%ранг квадратичного отображения тела
   {ранг квадратичного отображения тела}%
   {rank of quadratic map, division ring}%
\Index%749%Р%ранг эрмитовой матрицы по главным минорам
   {ранг эрмитовой матрицы по главным минорам}%
   {rank of Hermitian matrix by principal minors}%
\Index%419%Р%расслоение уровня 2
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Index%418%Р%расслоение уровня n
   {расслоение уровня $n$}%
   {bundle of level n}%
\Index%420%Р%расслоенная Omega- алгебра
   {расслоенная $\Omega$\Hyph алгебра}%
   {fibered Omega-algebra}%
\Index%421%Р%расслоенная Omega- подалгебра
   {расслоенная $\Omega$\Hyph подалгебра}%
   {fibered Omega-subalgebra}%
\Index%422%Р%расслоенная группа
   {расслоенная группа}%
   {fibered group}%
\Index%423%Р%расслоенная группа стабилизации
   {расслоенная группа стабилизации}%
   {fibered stability group}%
\Index%424%Р%расслоенная малая группа
   {расслоенная малая группа}%
   {fibered little group}%
\Index%425%Р%расслоенная предупорядоченность
   {расслоенная предупорядоченность}%
   {fibered preordering}%
\Index%426%Р%расслоенная упорядоченность
   {расслоенная упорядоченность}%
   {fibered ordering}%
\Index%427%Р%расслоенная эквивалентность
   {расслоенная эквивалентность}%
   {fibered equivalence}%
\Index%428%Р%расслоенное кольцо
   {расслоенное кольцо}%
   {fibered ring}%
\Index%429%Р%расслоенное подмножество
   {расслоенное подмножество}%
   {fibered subset}%
\Index%430%Р%расслоенное соответствие в A
   {расслоенное соответствие в $\Bundle{A}$}%
   {fibered correspondence in A}%
\Index%431%Р%расслоенное соответствие гомоморфизма
   {расслоенное соответствие гомоморфизма}%
   {fibered correspondence of homomorphism}%
\Index%432%Р%расслоенное соответствие из A в B
   {расслоенное соответствие из $\Bundle A$ в $\Bundle B$}%
   {fibered correspondence from A to B}%
\Index%433%Р%расслоенный естественный морфизм
   {расслоенный естественный морфизм}%
   {fibered natural morphism}%
\Index%434%Р%расслоенный координатный Drc изоморфизм
   {расслоенный координатный \Drc изоморфизм}%
   {fibered coordinate drc isomorphism}%
\Index%435%Р%расслоенный морфизм из расслоения A в B
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Index%436%Р%расслоенный морфизм отождествления
   {расслоенный морфизм отождествления}%
   {fibered identification morphism}%
\Index%437%Р%расширенная матрица drc линейных уравнений
   {расширенная матрица \drc линейных уравнений}%
   {extended matrix, system of drc linear equations}%
\Index%438%Р%расширенная матрица rcd линейных уравнений
   {расширенная матрица \rcd линейных уравнений}%
   {extended matrix, system of rcd linear equations}%
\Index%439%Р%рефлексивное 2- арное расслоенное отношение
   {рефлексивное $2$\Hyph арное расслоенное отношение}%
   {reflexive 2 ary fibered relation}%
\Index%839%Р%ряд сходится нормально
   {ряд сходится нормально}%
   {series converges normally}%
\Index%440%Р%ряд Тейлора
   {ряд Тейлора}%
   {Taylor series, division ring}%
\SetIndexSpace%
\Index%606%С%свободная алгебра над кольцом
   {свободная алгебра над кольцом}%
   {free algebra over ring}%
\Index%441%С%свободное Tstar- представление группы
   {свободное \Ts представление группы}%
   {free representation of group}%
\Index%442%С%свободное Tstar- представление расслоенной группы
   {свободное \Ts представление расслоенной группы}%
   {free representation of fibered group}%
\Index%690%С%свободный A- модуль
   {свободный $A$\Hyph модуль}%
   {free A module}%
\Index%612%С%свободный модуль над кольцом
   {свободный модуль над кольцом}%
   {free module over ring}%
\Index%833%С%связное множество
   {связное множество}%
   {connected set}%
\Index%846%С%связность в главном расслоении
   {связность в главном расслоении}%
   {connection in principal bundle}%
\Index%443%С%связность Картана
   {связность Картана}%
   {Cartan connection}%
\Index%694%С%сечение расслоения
   {сечение расслоения}%
   {section of bundle}%
\Index%444%С%символ Картана
   {символ Картана}%
   {Cartan symbol}%
\Index%445%С%символ Кронекерa
   {символ Кронекерa}%
   {Kronecker symbol}%
\Index%446%С%симметричное 2- арное расслоенное отношение
   {симметричное $2$\Hyph арное расслоенное отношение}%
   {symmetric 2 ary fibered relation}%
\Index%447%С%симметричное билинейное отображение D- векторного пространства в тело
   {симметричное билинейное отображение $D$\Hyph векторного пространства в тело}%
   {symmetric bilinear map, vector space to division ring}%
\Index%650%С%симметричное полилинейное отображение в ассоциативную алгебру
   {симметричное полилинейное отображение в ассоциативную алгебру}%
   {polylinear map symmetric, associative algebra}%
\Index%836%С%симплекс
   {симплекс}%
   {simplex}%
\Index%448%С%синхронизация системы отсчёта
   {синхронизация системы отсчёта}%
   {synchronization of reference frame}%
\Index%449%С%система drc линейных уравнений
   {система \drc линейных уравнений}%
   {system of drc linear equations}%
\Index%311%С%система rcd линейных уравнений
   {система \rcd линейных уравнений}%
   {system of rcd linear equations}%
\Index%605%С%система аддитивных уравнений
   {система аддитивных уравнений}%
   {system of additive equations}%
\Index%450%С%система отсчёта в пространстве событий
   {система отсчёта в пространстве событий}%
   {reference frame in event space}%
\Index%781%С%скаляр отображения
   {скаляр отображения}%
   {scalar of mapping}%
\Index%784%С%скаляр элемента алгебры
   {скаляр элемента алгебры}%
   {scalar of algebra}%
\Index%773%С%скаляр элемента кольца
   {скаляр элемента кольца}%
   {scalar of ring}%
\Index%451%С%скалярный потенциал
   {скалярный потенциал}%
   {scalar potential}%
\Index%452%С%скорость отклонения
   {скорость отклонения}%
   {speed of deviation}%
\Index%743%С%след кватерниона
   {след кватерниона}%
   {trace, quaternion algebra}%
\Index%453%С%смешанная частная производная Гато
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Index%454%С%соответствие гомоморфизма
   {соответствие гомоморфизма}%
   {correspondence of homomorphism}%
\Index%455%С%соответствие, непрерывное на множестве
   {соответствие, непрерывное на множестве}%
   {correspondence continuous on the set}%
\Index%788%С%сопряжение в алгебре
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Index%777%С%сопряжение в кольце
   {сопряжение в кольце}%
   {conjugation in ring}%
\Index%840%С%сопряжённое аффинное пространство
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Index%841%С%сопряжённое векторное пространство
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Index%580%С%сопряжённый D  модуль
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Index%457%С%стабильное множество представления
   {стабильное множество представления}%
   {stable set of representation}%
\Index%458%С%стандартная компонента дифференциала Гато
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Index%456%С%стандартная компонента линейного отображения
   {стандартная компонента линейного отображения}%
   {standard component of linear map}%
\Index%461%С%стандартная компонента над полем F билинейного отображения f
   {стандартная компонента над полем $F$ билинейного отображения $f$}%
   {standard component of bilinear map, division ring}%
\Index%462%С%стандартная компонента полилинейного отображения
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Index%463%С%стандартная компонента тензора
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Index%466%С%стандартное представление квадратичного отображения тела над полем F
   {стандартное представление квадратичного отображения тела над полем $F$}%
   {quadratic map, standard representation, division ring}%
\Index%464%С%стандартное представление линейного отображения
   {стандартное представление линейного отображения}%
   {linear map, standard representation}%
\Index%468%С%стандартное представление матрицы
   {стандартное представление матрицы}%
   {Standard representation}%
\Index%469%С%стандартное представление над полем F билинейного отображения тела
   {стандартное представление над полем $F$ билинейного отображения тела}%
   {bilinear map, standard representation, division ring}%
\Index%470%С%стандартное представление полилинейного отображения
   {стандартное представление полилинейного отображения}%
   {polylinear map, standard representation}%
\Index%465%С%стандартное представление производной Гато
   {стандартное представление производной Гато}%
   {Gateaux derivative, standard representation}%
\Index%471%С%стандартные координаты rcd базиса
   {стандартные координаты \rcd базиса}%
   {standard coordinates of rcd basis}%
\Index%472%С%стандартные координаты базиса
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Index%822%С%старший коэффициент многочлена
   {старший коэффициент многочлена}%
   {leading coefficient of polynomial}%
\Index%857%С%степень меры
   {степень меры}%
   {power of measure}%
\Index%750%С%столбцовый определитель
   {столбцовый определитель}%
   {column determinant}%
\Index%748%С%строчный определитель
   {строчный определитель}%
   {row determinant}%
\Index%473%С%структурные константы
   {структурные константы}%
   {structural constants}%
\Index%474%С%сужение соответствия \Phi на множество C
   {сужение соответствия $\Phi$ на множество $C$}%
   {restriction of correspondence}%
\Index%476%С%сумма геометрических объектов
   {сумма геометрических объектов}%
   {sum of geometric objects}%
\Index%477%С%сумма геометрических объектов в векторном пространстве
   {сумма геометрических объектов в векторном пространстве}%
   {sum of geometric objects, vector space}%
\Index%351%С%сумма линейных отображений
   {сумма линейных отображений}%
   {sum of linear maps}%
\Index%667%С%сумма многочленов
   {сумма многочленов}%
   {sum of polynomials}%
\Index%712%С%суперпозиция координат эндоморфизма башни представлений и элемента
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Index%323%С%суперпозиция координат эндоморфизма представления и элемента
   {суперпозиция координат эндоморфизма представления $f$ и элемента $m$}%
   {superposition of coordinates, representation}%
\Index%51%С%существенные параметры  семейства функций
   {существенные параметры  семейства функций}%
   {essential parameters}%
\SetIndexSpace%
\Index%478%Т%тензор кручения
   {тензор кручения}%
   {torsion tensor}%
\Index%479%Т%тензор напряжённости поля
   {тензор напряжённости поля}%
   {field-strength tensor}%
\Index%802%Т%тензор, обратный тензору
   {тензор, обратный тензору}%
   {inverse tensor}%
\Index%652%Т%тензорная степень
   {тензорная степень}%
   {tensor power}%
\Index%480%Т%тензорное произведение D- векторных пространств
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Index%481%Т%тензорное произведение Dstar векторных пространств
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Index%573%Т%тензорное произведение алгебр
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Index%207%Т%тензорное произведение векторных пространств
   {тензорное произведение векторных пространств}%
   {tensor product of vector spaces}%
\Index%482%Т%тензорное произведение колец над коммутативным кольцом
   {тензорное произведение колец над коммутативным кольцом}%
   {tensor product of rings}%
\Index%483%Т%тензорное произведение представлений
   {тензорное произведение представлений}%
   {tensor product of representations}%
\Index%484%Т%тензорное произведение тел
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Index%485%Т%тип векторного пространства
   {тип векторного пространства}%
   {vector space type}%
\Index%310%Т%топологическая D-алгебра
   {топологическая $D$\Hyph алгебра}%
   {topological D algebra}%
\Index%486%Т%топологическое D- векторное пространство
   {топологическое $D$\Hyph векторное пространство}%
   {topological D vector space}%
\Index%790%Т%топологическое кольцо
   {топологическое кольцо}%
   {topological ring}%
\Index%488%Т%топологическое тело
   {топологическое тело}%
   {topological division ring}%
\Index%824%Т%точка прикосновения множества
   {точка прикосновения множества}%
   {contact point of set}%
\Index%489%Т%транзитивное 2- арное расслоенное отношение
   {транзитивное $2$\Hyph арное расслоенное отношение}%
   {transitive 2 ary fibered relation}%
\Index%490%Т%транзитивное представление Omega- алгебры A
   {транзитивное представление $\Omega$\Hyph алгебры $A$}%
   {transitive representation of algebra}%
\Index%491%Т%транзитивное представление группы
   {транзитивное представление группы}%
   {transitive representation of group}%
\Index%492%Т%транзитивное представление расслоенной Omega- алгебры
   {транзитивное представление расслоенной $\Omega$\Hyph алгебры}%
   {transitive representation of fibered Omega-algebra}%
\SetIndexSpace%
\Index%751%У%упорядоченное слева представление подстановки произведением циклов
   {упорядоченное слева представление подстановки произведением циклов}%
   {left-ordered cycle notation of permutation}%
\Index%752%У%упорядоченное справа представление подстановки произведением циклов
   {упорядоченное справа представление подстановки произведением циклов}%
   {right-ordered cycle notation of permutation}%
\Index%493%У%уравнение Киллинга
   {уравнение Киллинга}%
   {Killing equation}%
\Index%494%У%уравнение Киллинга второго рода
   {уравнение Киллинга второго рода}%
   {Killing equation second type}%
\Index%744%У%условие перестановочности следа
   {условие перестановочности следа}%
   {permutability property of trace}%
\Index%495%У%условие приводимости произведений
   {условие приводимости произведений}%
   {condition of reducibility of products}%
\SetIndexSpace%
\Index%496%Ф%фактор расслоение
   {фактор расслоение}%
   {quotient bundle}%
\Index%497%Ф%фильтр F сходится к A
   {фильтр $\mathfrak{F}$ сходится к $A$}%
   {filter converges}%
\Index%131%Ф%финслерова метрика
   {финслерова метрика}%
   {Finsler metric}%
\Index%574%Ф%финслерова структура
   {финслерова структура}%
   {Finsler structure}%
\Index%77%Ф%финслерово пространство
   {финслерово пространство}%
   {Finsler space}%
\Index%498%Ф%форма кручение
   {форма кручение}%
   {torsion form}%
\Index%499%Ф%формула Тейлора для многочлена
   {формула Тейлора для многочлена}%
   {Taylor polynomial, division ring}%
\Index%243%Ф%фундаментальная последовательность
   {фундаментальная последовательность}%
   {fundamental sequence}%
\Index%504%Ф%функция тела, Dstar дифференцируемая по Фреше
   {функция тела, \Ds дифференцируемая по Фреше}%
   {function Dstar differentiable in Frechet sense, division ring}%
\Index%155%Ф%функция, однородная степени
   {функция, однородная степени $k$}%
   {function homogeneous}%
\SetIndexSpace%
\Index%620%Ц%центр алгебры
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Index%507%Ц%центр кольца D
   {центр кольца $D$}%
   {center of ring}%
\Index%508%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis, division ring}%
\Index%509%Ц%центро-аффинный базис
   {центро-аффинный базис}%
   {Central Affine Basis}%
\SetIndexSpace%
\Index%511%Ч%частная dcr производная Гато отображения f^b по переменной x^a
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map with respect to variable, D vector space}%
\Index%512%Ч%частная производная Гато
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Index%475%Ч%частное линейное отображение
   {частное линейное отображение}%
   {partial linear map}%
\SetIndexSpace%
\Index%566%Э%невырожденный эндоморфизм башни представлений
   {невырожденный эндоморфизм башни представлений}%
   {regular endomorphism of tower of representations}%
\Index%539%Э%эвклидова метрика на теле
   {эвклидова метрика на теле}%
   {Euclidean metric on division ring}%
\Index%547%Э%эвклидово скалярное произведение в D- векторном пространстве
   {эвклидово скалярное произведение в $D$\Hyph векторном пространстве}%
   {Euclidean scalar product, vector space}%
\Index%542%Э%эвклидово скалярное произведение на теле
   {эвклидово скалярное произведение на теле}%
   {Euclidean scalar product on division ring}%
\Index%515%Э%экстремальная кривая
   {экстремальная кривая}%
   {extreme line}%
\Index%559%Э%эндоморфизм башни представлений
   {эндоморфизм башни представлений}%
   {endomorphism of tower of representations}%
\Index%565%Э%эндоморфизм башни представлений, вырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, вырожденный на кортеже множеств образующих}%
   {endomorphism of representation, singular on tuple}%
\Index%564%Э%эндоморфизм башни представлений, невырожденный на кортеже множеств образующих
   {эндоморфизм башни представлений, невырожденный на кортеже множеств образующих}%
   {endomorphism of representation, regular on tuple}%
\Index%557%Э%эндоморфизм представления Omega алгебры
   {эндоморфизм представления $\Omega$\Hyph алгебры}%
   {endomorphism of representation}%
\Index%328%Э%эндоморфизм представления, вырожденный на множестве образующих X
   {эндоморфизм представления, вырожденный на множестве образующих $X$}%
   {endomorphism of representation, singular on set}%
\Index%327%Э%эндоморфизм представления, невырожденный на множестве образующих X
   {эндоморфизм представления, невырожденный на множестве образующих $X$}%
   {endomorphism of representation, regular on set}%
\Index%747%Э%эрмитова матрица
   {эрмитова матрица}%
   {hermitian matrix}%
\Index%544%Э%эрмитова метрика на теле
   {эрмитова метрика на теле}%
   {hermitian metric on division ring}%
\Index%350%Э%эрмитово скалярное произведение в D- векторном пространстве
   {эрмитово скалярное произведение в $D$\Hyph векторном пространстве}%
   {hermitian scalar product, vector space}%
\Index%545%Э%эрмитово скалярное произведение на теле
   {эрмитово скалярное произведение на теле}%
   {hermitian scalar product on division ring}%
\Index%541%Э%эрмитово сопряжение в теле
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Index%546%Э%эрмитово сопряжённый вектор
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Index%500%Э%эффективное Tstar представление Omega- алгебры A
   {эффективное \Ts представление $\Omega$\Hyph алгебры $A$}%
   {effective Tstar representation of algebra}%
\Index%516%Э%эффективное Tstar- представление группы
   {эффективное \Ts представление группы}%
   {effective Tstar representation of group}%
\Index%514%Э%эффективное Tstar- представление расслоенного тела
   {эффективное \Ts представление расслоенного тела}%
   {effective representation of fibered division ring}%
\Index%520%Э%эффективное Tstar- представление расслоенной группы
   {эффективное \Ts представление расслоенной группы}%
   {effective representation of fibered group}%
\Index%517%Э%эффективное представление Omega- алгебры A
   {эффективное представление $\Omega$\Hyph алгебры $A$}%
   {effective representation of algebra}%
\Index%518%Э%эффективное представление группы
   {эффективное представление группы}%
   {effective representation of group}%
\Index%622%Э%эффективное представление кольца
   {эффективное представление кольца}%
   {effective representation of ring}%
\Index%519%Э%эффективное представление расслоенной Omega- алгебры
   {эффективное представление расслоенной $\Omega$\Hyph алгебры}%
   {effective representation of fibered Omega-algebra}%
\Index%521%Э%эффективное представление тела
   {эффективное представление тела}%
   {effective representation of division ring}%
\SetIndexSpace%
\Index%619%Я%ядро алгебры
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%
\Index%522%Я%ядро линейного отображения
   {ядро линейного отображения}%
   {kernel of linear map}%
\Index%524%Я%ядро неэффективности Tstar- представления группы G
   {ядро неэффективности \Ts представления группы $G$}%
   {kernel of inefficiency of Tstar representation of group}%
\Index%525%Я%ядро неэффективности представления группы
   {ядро неэффективности представления группы}%
   {kernel of inefficiency of representation of group}%
\Index%526%Я%ядро неэффективности представления расслоенной группы
   {ядро неэффективности представления расслоенной группы}%
   {kernel of inefficiency of representation of fibered group}%
\Index%593%Я%якобиевая полная система drc дифференциальных уравнений
   {якобиевая полная система \drc дифференциальных уравнений}%
   {Jacobian complete system of drc differential equations}%
\Index%592%Я%якобиевая полная система дифференциальных уравнений
   {якобиевая полная система дифференциальных уравнений}%
   {Jacobian complete system of differential equations}%
\SetIndexSpace%
\Index%809%M%mu измеримое отображение
   {$\mu$\Hyph измеримое отображение}%
   {mu measurable map}%
\SetIndexSpace%
\Index%644%O%Omega группа
   {$\Omega$\Hyph группа}%
   {Omega group}%
\Index%858%O%Omega кольцо
   {\(\Omega\)\Hyph кольцо}%
   {Omega ring}%
\Index%646%O%Omega линейное отображение
   {$\Omega$\Hyph линейное отображение}%
   {Omega linear map}%
\Index%707%O%Omega_2- слово элемента представления относительно множества образующих
   {$\Omega_2$\Hyph слово элемента представления относительно множества образующих}%
   {word of element relative to generating set, representation}%
\SetIndexSpace%
\Index%658%S%sigma алгебра множеств
   {$\sigma$\Hyph алгебра множеств}%
   {sigma algebra of sets}%
\Index%795%S%sigma кольцо множеств
   {$\sigma$\Hyph кольцо множеств}%
   {sigma ring of sets}%
\Index%762%S%sigma-аддитивная мера
   {\(\sigma\)\Hyph аддитивная мера}%
   {sigma-additive measure}%

\CloseIndex


==> Normed.Omega.Russian.tex <==
%auto-ignore
\input{Normed.Omega.Eq}
\ifx\PrintBook\Defined
\chapter{Нормированная \texorpdfstring{$\Omega$}{Omega}-группа}
\fi

\section{Нормированная \texorpdfstring{$\Omega$}{Omega}-группа}
%\label{section: }

Пусть в $\Omega$\Hyph алгебре\footnote{Смотри
определение универсальной алгебры в
\citeBib{Burris Sankappanavar,Cohn: Universal Algebra}.
}
$A$ определена операция сложения,
которая не обязательно коммутативна.

\begin{definition}
Отображение
\ShowEq{f:A->A}
называется
\AddIndex{аддитивным отображением}{additive map},
если
\ShowEq{f(a+b)=}
\qed
\end{definition}

\begin{definition}
\label{definition: polyadditive map}
Отображение
\ShowEq{f:An->A}
называется
\AddIndex{полиаддитивным отображением}{polyadditive map},
если для любого
\ShowEq{fi(a+b)=}
\qed
\end{definition}

\begin{definition}
\label{definition: Omega group}
Если $\Omega$\Hyph алгебра $A$ является группой
относительно операции сложения
и любая операция $\omega\in\Omega$
является полиаддитивным отображением,
то $\Omega$\Hyph алгебра $A$ называется
\AddIndex{$\Omega$\Hyph группой}{Omega group}.\footnote{Вы
можете найти определение $\Omega$\Hyph группы по адресу
\begin{center}\url{http://ncatlab.org/nlab/show/Omega-group}\end{center}
}
Если $\Omega$\Hyph группа $A$ является ассоциативной группой
относительно операции сложения,
то $\Omega$\Hyph алгебра $A$ называется
\AddIndex{ассоциативной $\Omega$\Hyph группой}{associative Omega group}.
Если $\Omega$\Hyph группа $A$ является абелевой группой
относительно операции сложения,
то $\Omega$\Hyph алгебра $A$ называется
\AddIndex{абелевой $\Omega$\Hyph группой}{Abelian Omega group}.
\qed
\end{definition}

\begin{example}
Наиболее очевидный пример $\Omega$\Hyph группы
является собственно группой.
\qed
\end{example}

\begin{example}
Кольцо является $\Omega$\Hyph группой.
\qed
\end{example}

\begin{example}
Бикольцо матриц над телом
(\citeBib{0612.111})
является $\Omega$\Hyph группой.
\qed
\end{example}

\begin{convention}
Мы будем полагать, что рассматриваемая $\Omega$\Hyph группа
абелева.
\qed
\end{convention}

Элемент $\Omega$\Hyph группы $A$ называется
\AddIndex{$A$\Hyph числом}{A number}.

\begin{definition}
Пусть $A$ - $\Omega$\Hyph группа.
Подгруппа $B$ аддитивной группы $A$,
замкнутая относительно операций из $\Omega$,
называется
\AddIndex{подгруппой $\Omega$\Hyph группы}{subgroup of Omega group}
$A$.
\qed
\end{definition}

\begin{definition}
\label{definition: norm on Omega group}
\AddIndex{Норма на $\Omega$\Hyph группе}
{norm on Omega group} $A$\footnote{Определение дано согласно
определению из \citeBib{Bourbaki: General Topology: Chapter 5 - 10},
гл. IX, \S 3, п${}^\circ$2, а также согласно
определению \citeBib{Arnautov Glavatsky Mikhalev}-1.1.12,
с. 23.} - это отображение
\ShowEq{d->|d|}
такое, что
\StartLabelItem
\begin{enumerate}
\ShowEq{|a|>=0}
\ShowEq{|a|=0}
равносильно $a=0$
\ShowEq{|a+b|<=|a|+|b|}
\ShowEq{|-a|=|a|}
\end{enumerate}

$\Omega$\Hyph группа $A$,
наделённая структурой, определяемой заданием на $A$ нормы, называется
\AddIndex{нормированной $\Omega$\Hyph группой}{normed Omega group}.
\qed
\end{definition}

\begin{remark}
Если $\Omega$\Hyph группа $B$
с нормой $\|b\|_B$
является подгруппой
$\Omega$\Hyph группы $A$
с нормой $\|b\|_A$, то мы требуем
\ShowEq{|b|B=|b|A}
\qed
\end{remark}

\begin{theorem}
\label{theorem: |a-b|>|a|-|b|}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Тогда
\ShowEq{|a-b|>|a|-|b|}
\end{theorem}
\begin{proof}
Так как
\ShowEq{a=a-b+b}
то из утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
\ShowEq{|a|<|a-b|+|b|}
Неравенство
\ShowEq{|a-b|>|a|-|b|, 1}
следует из неравенства
\EqRef{|a|<|a-b|+|b|}.
Из утверждения
\RefItem{|-a|=|a|}
и неравенства
\EqRef{|a-b|>|a|-|b|, 1}
следует, что
\ShowEq{|a-b|=|b-a|}
Неравенство
\EqRef{|a-b|>|a|-|b|}
следует из неравенств
\EqRef{|a-b|>|a|-|b|, 1},
\EqRef{|a-b|=|b-a|}.
\end{proof}

\begin{definition}
\label{definition: norm of operation}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$, величина
\ShowEq{norm of operation}
\ShowEq{norm of operation, definition}
называется
\AddIndex{нормой операции}{norm of operation} $\omega$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: |fx|<|f||x|1n}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для $n$\Hyph арной операции $\omega$,
\ShowEq{|a omega|<|omega||a|1n}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{norm of operation, definition}
следует, что
\ShowEq{|a omega|<|omega||a|1n 1}
Неравенство
\EqRef{|a omega|<|omega||a|1n}
следует из неравенства
\EqRef{|a omega|<|omega||a|1n 1}.
\end{proof}

\begin{definition}
\label{definition: open ball}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть $a\in A$.
Множество
\ShowEq{open ball}
называется
\AddIndex{открытым шаром}{open ball}
с центром в $a$.
\qed
\end{definition}

\begin{definition}
\label{definition: closed ball}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть $a\in A$.
Множество
\ShowEq{closed ball}
называется
\AddIndex{замкнутым шаром}{closed ball}
с центром в $a$.
\qed
\end{definition}

\begin{theorem}
Из утверждения
\ShowEq{b in B(a)}
следует утверждение\footnote{Аналогичная
теорема верна для замкнутых шаров.}
\ShowEq{a in B(b)}.
\end{theorem}
\begin{proof}
Теорема следует из определения
\ref{definition: open ball}.
\end{proof}

\begin{definition}
\label{definition: limit of sequence, Omega group}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Элемент $a\in A$ называется 
\AddIndex{пределом последовательности}{limit of sequence}
$a_n$
\ShowEq{limit of sequence, Omega group}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|an-a|<epsilon}{-}
для любого $n>n_0$.
Мы будем также говорить, что
\AddIndex{последовательность $a_n$ сходится}{sequence converges}
к $a$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: limit of sequence, Omega group}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Элемент $a\in A$ является 
пределом последовательности
$a_n$
\DrawEq{a=lim an}{}
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{an in B(a)}{}
для любого $n>n_0$.
\end{theorem}
\begin{proof}
Следствие определений
\ref{definition: open ball},
\ref{definition: limit of sequence, Omega group}.
\end{proof}

\begin{definition}
\label{definition: fundamental sequence}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Последовательность $a_n$, $a_n\in A$ называется 
\AddIndex{фундаментальной}{fundamental sequence}
или \AddIndex{последовательностью Коши}{Cauchy sequence},
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{|ap-aq|<epsilon}{-}
для любых $p$, $q>n_0$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: fundamental sequence}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Последовательность $a_n$, $a_n\in A$ является 
фундаментальной последовательностью,
если для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{aq in B(ap)}
для любых $p$, $q>n_0$.
\end{theorem}
\begin{proof}
Следствие определений
\ref{definition: open ball},
\ref{definition: fundamental sequence}.
\end{proof}

\begin{theorem}
\label{theorem: lim a-b=0 fundamental}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $n=1$, ..., - фундаментальная последовательность.
Пусть $b_n$, $n=1$, ..., - последовательность.
Пусть
\DrawEq{lim a-b=0}{fundamental}
Тогда $b_n$ - фундаментальная последовательность.
\end{theorem}
\begin{proof}
Из равенства
\eqRef{lim a-b=0}{fundamental}
и определения
\ref{definition: limit of sequence, Omega group}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_1$ такое, что
\DrawEq{|an-bn|<epsilon/3}{fundamental}
для любого $n>N_1$.
Согласно определению
\ref{definition: fundamental sequence},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_2$ такое, что
\DrawEq{|ap-aq|<epsilon/3}{fundamental}
для любых $p$, $q>N_2$.
Пусть
\ShowEq{N N1 N2}
Из неравенств
\eqRef{|an-bn|<epsilon/3}{fundamental},
\eqRef{|ap-aq|<epsilon/3}{fundamental}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|bp-bq|<epsilon}
для любых $p$, $q>N$.
Согласно определению
\ref{definition: fundamental sequence},
последовательность $b_n$ - фундаментальная последовательность.
\end{proof}

\begin{theorem}
\label{theorem: lim a=lim b}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $a_n$, $b_n$, $n=1$, ..., - фундаментальные последовательности.
Пусть
\DrawEq{lim a-b=0}{limit}
Если последовательность $a_n$ сходится, то
последовательность $b_n$ сходится и
\ShowEq{lim a=lim b}
\end{theorem}
\begin{proof}
Из равенства
\eqRef{lim a-b=0}{limit}
и определения
\ref{definition: limit of sequence, Omega group}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_1$ такое, что
\DrawEq{|an-bn|<epsilon/2}{lim a=lim b}
для любого $n>N_1$.
Согласно определению
\ref{definition: complete Omega group}
и теореме
\ref{theorem: fundamental sequence has only one limit},
существует предел $a$ последовательности $a_n$.
Согласно определению
\ref{definition: limit of sequence, Omega group},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_2$ такое, что
\ShowEq{|an-a|<epsilon/2}
для любого $n>N_2$.
Пусть
\ShowEq{N N1 N2}
Из неравенств
\eqRef{|an-bn|<epsilon/2}{lim a=lim b},
\EqRef{|an-a|<epsilon/2}
и утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|a-bn|<epsilon}
для любого $n>N$.
Согласно определению
\ref{definition: limit of sequence, Omega group},
последовательность $b_n$ сходится к $a$.
\end{proof}

\begin{definition}
\label{definition: complete Omega group}
Нормированная $\Omega$\Hyph группа $A$ называется 
\AddIndex{полной}{complete Omega group}
если любая фундаментальная последовательность элементов
$\Omega$\Hyph группы $A$ сходится, т. е.
имеет предел в этой $\Omega$\Hyph группе.
\qed
\end{definition}

\begin{theorem}
\label{theorem: fundamental sequence has only one limit}
Пусть $A$ - полная $\Omega$\Hyph группа.
Любая фундаментальная последовательность
имеет один и только один предел.
\end{theorem}
\begin{proof}
Пусть $a_n$, $n=1$, ..., - фундаментальная последовательность.
Согласно определению
\ref{definition: fundamental sequence},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_1$ такое, что
\DrawEq{|ap-aq|<epsilon/3}{only one limit}
для любых $p$, $q>n_1$.
Пусть
\DrawEq{a=lim an}{fundamental}
и
\ShowEq{b=lim an}
Из равенства
\eqRef{a=lim an}{fundamental}
и определения
\ref{definition: limit of sequence, Omega group}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_2$ такое, что
\ShowEq{|ap-a|<epsilon/3}
для любого $p>n_2$.
Из равенства
\EqRef{b=lim an}
и определения
\ref{definition: limit of sequence, Omega group}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_3$ такое, что
\ShowEq{|aq-b|<epsilon/3}
для любого $q>n_3$.
Пусть
\ShowEq{n0123}
Из неравенств
\ShowEq{fundamental sequence ab}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\ShowEq{|a-b|<epsilon pq}
для любых $p$, $q>n_0$.
Следовательно,
\ShowEq{|a-b|=0}
Согласно утверждению
\RefItem{|a|=0},
$a=b$.
\end{proof}

\section{Топология \texorpdfstring{$\Omega$}{Omega}-группы}

\begin{remark}
\label{remark: set of open balls is base of topology}
Инвариантное расстояние на аддитивной группе $\Omega$\Hyph группы $A$
\ShowEq{Invariant distance on additive group}
определяет топологию метрического пространства,
согласующуюся со структурой $\Omega$\Hyph группы в $A$.
Множество открытых шаров нормированной $\Omega$\Hyph группы $A$
является базой топологии,\footnote{Смотри
определение базы топологии в
\citeBib{Kolmogorov Fomin}, страница 87.}
согласованной с расстоянием
\EqRef{Invariant distance on additive group}.
\qed
\end{remark}

\begin{definition}
\label{definition: open set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
$U\subset A$
называется
\AddIndex{открытым}{open set},\footnote{В топологии
обычно сперва определяют открытое множество,
а затем базу топологии.
В случае метрического или нормированного пространства,
удобнее дать определение открытого множества,
опираясь на определение базы топологии.
В этом случае определение основано на одном из свойств
базы топологии. Непосредственная проверка
позволяет убедиться, что определённое таким образом
открытое множество удовлетворяет основным свойствам.
}
если для любого $A$\Hyph числа
\ShowEq{a in U}
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(a) subset U}
\qed
\end{definition}

\begin{definition}
\label{definition: closure of set}
Пусть $B$ - подмножество топологического пространства $A$.
Точка $x\in A$ называется
\AddIndex{точкой прикосновения множества}{contact point of set}
$B$,\footnote{Смотри
определение точки прикосновения и замыкания множества в
\citeBib{Kolmogorov Fomin}, страница 85.}
если для любого
\ShowEq{epsilon in R}
открытый шар
\ShowEq{B(x)}
содержит хотя бы одну точку множества $B$
\ShowEq{B(x) B}
Множество всех точек прикосновения множества $B$ называется
\AddIndex{замыканием множества}{closure of set} $B$.
Замыкание множества $B$ обозначается
\ShowEq{closure of set}
\qed
\end{definition}

\begin{remark}
\label{remark: closure of set}
Множество $B$ замкнуто тогда и только тогда, когда
\ShowEq{closed set}

Это утверждение может быть либо
определением замкнутого множества,
либо теоремой. Например, рассмотрим определение
замкнутого множества как дополнение к открытому множеству.
Если
\ShowEq{x in A-[B]}
то существует окрестность точки $x$,
не содержащая точек множества $B$.
Следовательно,
\ShowEq{A-[B]}
открытое множество.
\qed
\end{remark}

\begin{definition}
\label{definition: dense in set}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Множество
\ShowEq{B subset A}
называется
\AddIndex{плотным в множестве}{dense in set}\footnote{Смотри
также определение в
\citeBib{Kolmogorov Fomin}, страница 59.}
\ShowEq{C subset A} если
\ShowEq{C subset [B]}
Множество
\ShowEq{B subset A}
называется
\AddIndex{всюду плотным}{everywhere dense subset},\footnote{Мы
также говорим, что множество $B$
всюду плотно в $\Omega$\Hyph группе $A$.
}
если
\ShowEq{[B]=A}
\qed
\end{definition}

\begin{definition}
[\AddIndex{вторая аксиома счётности}{second axiom of countability}]
В топологическом пространстве со счётной базой
существует по крайней мере одна база,
состоящая не более чем из счётного числа множеств.\footnote{Смотри
также определению в
\citeBib{Kolmogorov Fomin}, страница 88.
Согласно теореме в
\citeBib{Kolmogorov Fomin}, страницы 88, 89,
в топологическом пространстве со второй аксиомой счётности
существует счётное всюду плотное множество.
}
\qed
\end{definition}

\begin{definition}[Первая аксиома отделимости]
\label{definition: First axiom of separation}
Топологическое пространство $A$ называется
\AddIndex{$T_1$\Hyph пространством}{T1 space},\footnote{Смотри
аналогичное определение в
\citeBib{Kolmogorov Fomin}, с. 94.}
если для точек
\ShowEq{xyA}
существуют окрестности
\ShowEq{Ux x}
и
\ShowEq{Uy y}
такие, что
\ShowEq{Uxy}
\qed
\end{definition}

\begin{theorem}
Любая точка $T_1$\Hyph пространства
является замкнутым множеством.\footnote{Смотри
также замечание после определения в
\citeBib{Kolmogorov Fomin}, с. 94.}
\end{theorem}
\begin{proof}
Если $x\ne y$, то согласно определению
\ref{definition: First axiom of separation},
существует окрестность $O_y$ точки $y$ такая, что
$x\not\in O_y$.
Согласно определению
\ref{definition: closure of set}
\ShowEq{y not in [x]}
Следовательно,
\ShowEq{x=[x]}
Согласно замечанию
\ref{remark: closure of set},
$\{x\}$ - замкнутое множество.
\end{proof}

\begin{theorem}
\label{theorem: First axiom of separation}
Нормированная $\Omega$\Hyph группа $A$
является $T_1$\Hyph пространством
тогда и только тогда, когда
для точек
\ShowEq{xyA}
существуют
открытые шары
\ShowEq{Bx By}
такие, что
\ShowEq{Bxy}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: First axiom of separation},
существуют окрестности
\ShowEq{Ux x}
и
\ShowEq{Uy y}
такие, что
\ShowEq{Uxy}
Согласно замечанию
\ref{remark: set of open balls is base of topology}
и определению на странице
\citeBib{Kolmogorov Fomin}\Hyph 87,
существуют
открытые шары
\ShowEq{Bx By}
такие, что
\ShowEq{Bxy in Uxy}
Следовательно,
\ShowEq{Bxy}
\end{proof}

\begin{convention}
\label{convention: topology of normed Omega group}
Для того, чтобы топология нормированной $\Omega$\Hyph группы $A$
была нетривиальной, мы потребуем следующее.
\StartLabelItem
\begin{enumerate}
\item
$\Omega$\Hyph группа $A$ является $T_1$\Hyph пространством.
\item
Нормированная $\Omega$\Hyph группа $A$
удовлетворяет
второй аксиоме счётности.
\item
Множество
$\{x\}$ не является открытым множеством.
\LabelItem{x is not open}
\end{enumerate}
\qed
\end{convention}

\begin{theorem}
\label{theorem: open ball is not empty}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для любых
\ShowEq{xr in AR}
существует
\ShowEq{y in B(x)}.
\end{theorem}
\begin{proof}
Если мы предположим, что не существует
\ShowEq{y in B(x)},
то в этом случае
\ShowEq{Bo(x)=x}
и множество $\{x\}$ является открытым.
Это утверждение противоречит соглашению
\RefItem{x is not open}.
Следовательно, предположение не верно.
\end{proof}

\begin{theorem}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для любых
\ShowEq{a b in A}
существует
\ShowEq{a c in A}
такой, что
\ShowEq{|c-a|<|b-a|}
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: First axiom of separation},
существует открытый шар $B_o(a,r)$ такой, что
\ShowEq{b not in B(a)}
Согласно определению
\ref{definition: open ball}
\ShowEq{r<|b-a|}
Согласно теореме
\ref{theorem: open ball is not empty},
существует
\ShowEq{c in B(a)}
Согласно определению
\ref{definition: open ball}
\ShowEq{|c-a|<r}
Неравенство
\EqRef{|c-a|<|b-a|}
следует из неравенств
\EqRef{r<|b-a|},
\EqRef{|c-a|<r}.
\end{proof}

\begin{theorem}
\label{theorem: For any a there exists sequence}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для любого $a\in A$
существует последовательность $A$\Hyph чисел
\ShowEq{an ne a}
такая, что
\DrawEq{lim an}{sequence}
\end{theorem}
\begin{proof}
Существуют разные способы построить последовательность $a_n$.

Согласно теореме
\ref{theorem: open ball is not empty}
для любого $n$ существует
\ShowEq{an B(a,1/n)}
Согласно теореме
\ref{theorem: limit of sequence, Omega group},
последовательность $a_n$ сходится к $a$.

В рассматриваемой последовательности возможно, что $a_n=a_{n+1}$.
Однако очевидно, что если
\ShowEq{m>1/|an|}
то
\ShowEq{am ne an}
Мы можем построить последовательность,
в которой все элементы различны.

Пусть $a_1\in A$.
Предположим, мы выбрали $a_n\in A$, $n\ge 1$.
Пусть
\ShowEq{r=|an-a|/2}
Согласно теореме
\ref{theorem: open ball is not empty}
существует
\ShowEq{an B(a,r)}
Согласно равенству
\EqRef{r=|an-a|/2}
и определению
\ref{definition: open ball},
\ShowEq{an ne}
Согласно теореме
\ref{theorem: limit of sequence, Omega group},
последовательность $a_n$ сходится к $a$.
\end{proof}

\begin{theorem}
\label{theorem: sequence in dense set}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть множество
\ShowEq{B subset A}
плотно в множестве
\ShowEq{C subset A}.
Тогда для любого $A$\Hyph числа $b\in C$
существует последовательность $A$\Hyph чисел
\ShowEq{bn in B}
сходящаяся к $b$
\ShowEq{b lim bn}
\end{theorem}
\begin{proof}
Согласно определениям
\ref{definition: closure of set},
\ref{definition: dense in set},
для любого $n>0$ существует $b_n$ такой, что
\ShowEq{bn in B B(b)}
Согласно теореме
\ref{theorem: limit of sequence, Omega group},
последовательность $b_n$ сходится к $b$,
так как
\ShowEq{bn in B(b)}
для любого
\ShowEq{n>1/epsilon}.
\end{proof}

\begin{definition}
\label{definition: compact set}
Множество $T$ топологического пространства называется
\AddIndex{компактным}{compact set},
если любое его открытое покрытие содержит
конечное подпокрытие.\footnote{Смотри также
определение в
\citeBib{Kolmogorov Fomin}, страница 98.
}
\qed
\end{definition}

\begin{definition}
\label{definition: connected set}
Множество $T$ топологического пространства называется
\AddIndex{связным}{connected set},\footnote{Смотри
также определения 1 и 2 в
\citeBib{Bourbaki: General Topology 1}, страницы 169, 170.
}
если существуют открытые множества $B$ и $C$ такие, что из условий
\ShowEq{T in B cup C}
следует
\ShowEq{T cap B cap C empty}.
\qed
\end{definition}

\begin{example}
\label{example: open connected set in real field is open interval}
Связное открытое множество в поле действительных чисел является
открытым интервалом.\footnote{Смотри
замечание 5 в
\citeBib{Kolmogorov Fomin}, страницы 65, 66.
}
\qed
\end{example}

\section{Непрерывное отображение
\texorpdfstring{$\Omega$}{Omega}-группы}

\begin{definition}
\label{definition: continuous map, Omega group}
Отображение
\ShowEq{f A1 A2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
называется \AddIndex{непрерывным}{continuous map}, если
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\ShowEq{|x'-x|<delta}
влечёт
\ShowEq{|f(x)-f(x')|<epsilon}
\qed
\end{definition}

\begin{theorem}
\label{theorem: continuous map, Omega group}
Отображение
\ShowEq{f A1 A2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{b in B(a,delta)}{}
влечёт
\DrawEq{fb in B(fa,epsilon)}{}
\end{theorem}
\begin{proof}
Теорема является следствием определений
\ref{definition: open ball},
\ref{definition: continuous map, Omega group}.
\end{proof}

\begin{theorem}
\label{theorem: continuous map, open set}
Отображение
\ShowEq{f A1 A2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
прообраз открытого множества
является открытым множеством.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{U subset A2}
открытое множество и
\ShowEq{Wf-1U}
\begin{itemize}
\item
Пусть отображение $f$ непрерывно.
Пусть
\ShowEq{a in W}
Тогда
\ShowEq{fa in U}.
Согласно определению
\ref{definition: open set},
существует
\ShowEq{epsilon in R}
такое, что
\ShowEq{B(fa) subset U}
Согласно теореме
\ref{theorem: continuous map, Omega group},
существует такое $\delta>0$, что
\DrawEq{b in B(a,delta)}{open set}
влечёт
\DrawEq{fb in B(fa,epsilon)}{open set}
Из равенств
\EqRef{B(fa) subset U},
\eqRef{fb in B(fa,epsilon)}{open set}
следует, что
\ShowEq{fb in U}
Из равенств
\EqRef{Wf-1U},
\EqRef{fb in U}
следует, что
\ShowEq{b in W}
Так как из утверждения
\eqRef{b in B(a,delta)}{open set}
следует утверждение
\EqRef{b in W},
то
\ShowEq{B(a,delta)subset W}
Согласно определению
\ref{definition: open set}
множество $W$ открыто.
\item
Пусть прообраз открытого множества
является открытым множеством.
Пусть
\ShowEq{U=B(fa)}
Так как $W$ - открытое множество,
то согласно определению
\ref{definition: open set}
существует $\delta>0$ такое, что
\ShowEq{B(a,delta)subset W}
Следовательно, из утверждения
\DrawEq{b in B(a,delta)}{-}
следует
\DrawEq{fb in B(fa,epsilon)}{-}.
Согласно теореме
\ref{theorem: continuous map, Omega group},
отображение $f$ непрерывно.
\end{itemize}
\end{proof}

\begin{theorem}
\label{theorem: image of connected set}
Пусть
\ShowEq{f:X->Y}
непрерывное отображение топологического пространства $X$
в топологическое пространство $Y$.
Пусть $T$ - связное множество топологического пространства $X$.
Тогда $f(T)$ - связное множество
топологического пространства $Y$.\footnote{Смотри также
предложение 4 в
\citeBib{Bourbaki: General Topology 1}, страница 171.
}
\end{theorem}
\begin{proof}
Пусть $B$, $C$ - открытые множества топологического пространства $Y$.
Так как отображение $f$ непрерывно, то согласно теореме
\ref{theorem: continuous map, open set},
множества $f^{-1}(B)$, $f^{-1}(C)$ открыты.
Если утверждения
\ShowEq{connected set}
верны для множеств $B$, $C$, $f(T)$,
то утверждения
\ShowEq{connected set}
верны для множеств $f^{-1}(B)$, $f^{-1}(C)$, $T$.
Если мы предположим, что множество $f(T)$ не связно,
то согласно определению
\ref{definition: connected set}
\ShowEq{B cap C cap f(T) empty}
Из равенства
\EqRef{B cap C cap f(T) empty}
следует, что
\ShowEq{fB cap fC cap T empty}
Согласно определению
\ref{definition: connected set},
множество $T$ не связно.
Это утверждение противоречит предположению теоремы.
Следовательно, множество $f(T)$ связно.
\end{proof}

\begin{theorem}
\label{theorem: image of interval is interval, real field}
Пусть
\ShowEq{f:R->R}
непрерывное отображение поля действительных чисел.
Тогда образ интервала является интервалом.
\end{theorem}
\begin{proof}
Теорема является следствием теоремы
\ref{theorem: image of connected set}
и примера
\ref{example: open connected set in real field is open interval}.
\end{proof}

\begin{theorem}
\label{theorem: f(lim)=lim f()}
Отображение
\ShowEq{f A1 A2}
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$
непрерывно тогда и только тогда, когда
из условия, что
последовательность $A_1$\Hyph чисел $a_n$ сходится,
следует, что
последовательность $A_2$\Hyph чисел $f(a_n)$ сходится
и верно равенство
\ShowEq{f(lim)=lim f()}
\end{theorem}
\begin{proof}
Пусть $A_1$\Hyph число $a$ является пределом последовательности $a_n$
\DrawEq{a=lim an}{f(lim)=lim f()}
\begin{itemize}
\item
Пусть равенство
\EqRef{f(lim)=lim f()}
верно для $A$\Hyph числа $a$.
Равенство
\DrawEq{fa=lim fan}{1}
следует из равенств
\EqRef{f(lim)=lim f()},
\eqRef{a=lim an}{f(lim)=lim f()}.
Из равенства
\eqRef{fa=lim fan}{1}
и теоремы
\ref{theorem: limit of sequence, Omega group},
следует, что для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_2$ такое, что
\DrawEq{fan in B(fa)}{1}
для любого $n>n_2$.
Из равенства
\eqRef{a=lim an}{f(lim)=lim f()}
и теоремы
\ref{theorem: limit of sequence, Omega group},
следует, что для заданного
\ShowEq{delta in R}
существует, зависящее от $\delta$, натуральное число $n_1$ такое, что
\DrawEq{an in B(a,delta)}{1}
для любого $n>n_1$.
Если $n_1\le n_2$,
то оценка $\delta$ завышена.
Мы положим
\ShowEq{delta=|a-an1|/2}
и повторим оценку значения $n_1$.
Очевидно, что новое значение $n_1$ будет больше предыдущего.
Следовательно,
за конечное число итераций мы найдём $\delta$ такое, что $n_1>n_2$
и из утверждения
\eqRef{an in B(a,delta)}{1}
следует утверждение
\eqRef{fan in B(fa)}{1}.
Согласно теореме
\ref{theorem: continuous map, Omega group},
отображение $f$ непрерывно.
\item
Пусть отображение $f$ непрерывно.
Согласно теореме
\ref{theorem: continuous map, Omega group},
для любого сколь угодно малого $\epsilon>0$
существует такое $\delta>0$, что
\DrawEq{b in B(a,delta)}{f(lim)=lim f()}
влечёт
\DrawEq{fb in B(fa,epsilon)}{f(lim)=lim f()}
Из равенства
\eqRef{a=lim an}{f(lim)=lim f()}
и теоремы
\ref{theorem: limit of sequence, Omega group},
следует, что для заданного
\ShowEq{delta in R}
существует, зависящее от $\delta$, натуральное число $n_1$ такое, что
\DrawEq{an in B(a,delta)}{2}
для любого $n>n_1$.
Из равенств
\ShowEq{fan in B(fa), ref}
следует, что для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_1$ такое, что
\DrawEq{fan in B(fa)}{2}
для любого $n>n_1$.
Равенство
\DrawEq{fa=lim fan}{2}
следует из равенства
\eqRef{fan in B(fa)}{2}
и теоремы
\ref{theorem: limit of sequence, Omega group}.
Равенство
\EqRef{f(lim)=lim f()}
следует из равенств
\eqRef{fa=lim fan}{2},
\eqRef{a=lim an}{f(lim)=lim f()}.
\end{itemize}
\end{proof}

\begin{definition}
\label{definition: norm of map, Omega group}
Пусть
\ShowEq{f A1 A2}
отображение нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$.
Величина
\ShowEq{norm of map}
\ShowEq{norm of map, Omega group}
называется
\AddIndex{нормой отображения $f$}{norm of map}.
\qed
\end{definition}

\begin{theorem}
\label{theorem: additive map is continuous}
Пусть
\ShowEq{f A1 A2}
аддитивное отображение
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группу $A_2$ с нормой $\|y\|_2$.
Отображение $f$ непрерывно, если $\|f\|<\infty$.
\end{theorem}
\begin{proof}
Поскольку отображение $f$ аддитивно, то
согласно определению \ref{definition: norm of map, Omega group}
\ShowEq{norm of additive map}
Возьмём произвольное $\epsilon>0$.
Положим $\displaystyle\delta=\frac\epsilon{\|f\|}$.
Тогда из неравенства
\ShowEq{|x-y|<delta}
следует
\ShowEq{|f(x)-f(y)|<epsilon}
Согласно определению \ref{definition: continuous map, Omega group}
отображение $f$ непрерывно.
\end{proof}

\begin{theorem}
\label{theorem: Norm is continues map}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Норма, определённая в $\Omega$\Hyph группе $A$,
является непрерывным отображением $\Omega$\Hyph группы $A$
в поле действительных чисел.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{epsilon in R}
и $a\in A$.
Согласно теореме
\ref{theorem: open ball is not empty}
существует
\ShowEq{b B(a,epsilon)}
Согласно определению
\ref{definition: open ball}
\ShowEq{|a-b|<epsilon}
Из неравенств
\EqRef{|a-b|<epsilon},
\EqRef{|a-b|>|a|-|b|}
следует, что
\ShowEq{|a|-|b|<epsilon}
Так как неравенство
\EqRef{|a|-|b|<epsilon}
является следствием неравенства
\EqRef{|a-b|<epsilon},
то норма непрерывна согласно определению
\ref{definition: continuous map, Omega group}.
\end{proof}

\begin{theorem}
\label{theorem: image of compact set is compact set}
Пусть
\ShowEq{f:A->B}
непрерывное отображение
нормированной $\Omega$\Hyph алгебры $A$ в
нормированную $\Omega$\Hyph алгебру $B$.
Если $C$ - компактное множество $\Omega$\Hyph алгебры $A$,
то образ $f(C)$ является
компактным множеством $\Omega$\Hyph алгебры $B$.
\end{theorem}
\begin{proof}
Пусть $D$ - открытое покрытие множества $f(C)$.
Любое множество
\ShowEq{E in D}
является открытым множеством.
Согласно теореме
\ref{theorem: continuous map, open set},
прообраз $f^{-1}(E)$ является открытым множеством.
Пусть
\ShowEq{D' open cover}
Утверждение
\ShowEq{C subset D'}
следует из утверждения
\ShowEq{fC subset D}
Следовательно, $D'$ является
открытым покрытием множества $C$.
Согласно определению
\ref{definition: compact set},
существует конечное подпокрытие
\ShowEq{E'1...E'n}
Следовательно, покрытие $D$ имеет конечное подпокрытие
\ShowEq{E1...En}
Согласно определению
\ref{definition: compact set},
множество $f(C)$ компактно.
\end{proof}

\begin{theorem}
\label{theorem: norm of compact set is bounded}
Пусть $C$ - компактное множество
нормированной $\Omega$\Hyph группы $A$.
Тогда норма
\ShowEq{|x in C|}
ограничена сверху и снизу.
\end{theorem}
\begin{proof}
Согласно теореме
\ref{theorem: Norm is continues map},
норма является непрерывным отображением $\Omega$\Hyph группы $A$
в поле действительных чисел.
Согласно теореме
\ref{theorem: image of compact set is compact set},
множество
\ShowEq{|x in C| 1}
компактно в поле действительных чисел.
Согласно утверждению
\citeBib{Shilov single 12}\Hyph 3.96.е,
страница 118,
множество $C'$ ограничено и содержит свои точные границы.
\end{proof}

\section{Непрерывность операций в
\texorpdfstring{$\Omega$}{Omega}-группе}

Из утверждения
\RefItem{|a+b|<=|a|+|b|}
и теоремы
\ref{theorem: additive map is continuous}
следует, что сумма в нормированной $\Omega$\Hyph группе
непрерывна.
Из определения
\ref{definition: norm of operation}
следует, что операции в нормированной $\Omega$\Hyph группе
непрерывны.\footnote{Сравни определение
\ref{definition: norm of operation}
нормы операции и определение
\xRef{1211.6965}{definition: norm of polylinear map}
нормы полилинейного отображения.
}
В этом разделе мы рассмотрим утверждения,
связанные с непрерывностью операций.

\begin{theorem}
В нормированной $\Omega$\Hyph группе $A$,
верно следующее неравенство
\ShowEq{|c12-a12|<|c-a|12}
\end{theorem}
\begin{proof}
Из утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
\ShowEq{|c12-a12|<|c-a|12, 1}
Неравенство
\EqRef{|c12-a12|<|c-a|12}
следует из неравенства
\EqRef{|c12-a12|<|c-a|12, 1}.
\end{proof}

\begin{theorem}
\label{theorem: c1+c2 in B}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Для
\ShowEq{c1 c2 in A}
пусть
\ShowEq{c1 c2 in B}
Тогда
\ShowEq{c1+c2 in B}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: open ball}
\ShowEq{c1+c2 in B 1}
Из неравенств
\EqRef{|c12-a12|<|c-a|12},
\EqRef{c1+c2 in B 1}
следует, что
\ShowEq{c1+c2 in B 2}
Утверждение
\EqRef{c1+c2 in B}
следует из неравенства
\EqRef{c1+c2 in B 2}
и определения
\ref{definition: open ball}.
\end{proof}

\begin{theorem}
\label{theorem: lim an+bn}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть последовательность $A$\Hyph чисел $a_n$ сходится и
\DrawEq{lim an}{+}
Пусть последовательность $A$\Hyph чисел $b_n$ сходится и
\ShowEq{lim bn}
Тогда последовательность $A$\Hyph чисел $a_n+b_n$ сходится и
\ShowEq{lim an+bn}
\end{theorem}
\begin{proof}
Из равенства
\eqRef{lim an}{+}
и теоремы
\ref{theorem: limit of sequence, Omega group}
следует, что для заданного
\ShowEq{epsilon in R}
существует $N_a$ такое, что из условия
\ShowEq{n>Na}
следует
\ShowEq{an in B_o}
Из равенства
\EqRef{lim bn}
и теоремы
\ref{theorem: limit of sequence, Omega group}
следует, что для заданного
\ShowEq{epsilon in R}
существует $N_b$ такое, что из условия
\ShowEq{n>Nb}
следует
\ShowEq{bn in B_o}
Пусть
\ShowEq{N Na Nb}
Из равенств
\EqRef{an in B_o},
\EqRef{bn in B_o},
теоремы
\ref{theorem: c1+c2 in B}
и условия $n>N$
следует, что
\ShowEq{an+bn in B_o}
Равенство
\EqRef{lim an+bn}
следует из равенства
\EqRef{an+bn in B_o}
и теоремы
\ref{theorem: limit of sequence, Omega group}.
\end{proof}

\begin{theorem}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Верно следующее неравенство
\ShowEq{|(c-a)omega|<|(c-a)||omega|}
где
\DrawEq{C=max(a,c)}{||}
\end{theorem}
\begin{proof}
Согласно определениям
\ref{definition: polyadditive map},
\ref{definition: Omega group},
\ShowEq{c1 cn omega in B 2}
Из равенства
\EqRef{c1 cn omega in B 2}
и утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
\ShowEq{|c1n omega|<|c1n||omega|}
Из равенства
\eqRef{C=max(a,c)}{||}
и определения
\ref{definition: norm of operation}
следует, что
\ShowEq{c1 cn omega in B 4}
Неравенство
\EqRef{|(c-a)omega|<|(c-a)||omega|}
следует из неравенств
\EqRef{|c1n omega|<|c1n||omega|},
\EqRef{c1 cn omega in B 4}.
\end{proof}

\begin{theorem}
\label{theorem: c1 cn omega in B}
Пусть $A$
- нормированная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Для
\ShowEq{c1 cn in A}
пусть
\ShowEq{c1 cn in B}
Тогда
\ShowEq{c1 cn omega in B}
где
\ShowEq{R=R1+ +Rn}
\ShowEq{C=|a|+R}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: open ball}
\ShowEq{c1 cn omega in B 1}
Неравенство
\DrawEq{|c|<|a|+R}{1n}
следует из неравенства
\EqRef{c1 cn omega in B 1}
и утверждения
\RefItem{|a+b|<=|a|+|b|}.
Неравенство
\ShowEq{C<|a|+R}
следует из неравенства
\eqRef{|c|<|a|+R}{1n}
и равенства
\eqRef{C=max(a,c)}{||}.
Равенство
\EqRef{C=|a|+R}
следует из неравенства
\EqRef{C<|a|+R}.
Утверждение
\EqRef{c1 cn omega in B}
следует из неравенств
\EqRef{|(c-a)omega|<|(c-a)||omega|},
\EqRef{c1 cn omega in B 1}
и равенства
\EqRef{C=|a|+R}.
\end{proof}

\begin{theorem}
\label{theorem: lim a1m...anm omega}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Пусть последовательность $A$\Hyph чисел
\ShowEq{aim}
сходится и
\ShowEq{lim aim}
Тогда последовательность $A$\Hyph чисел
\ShowEq{a1m...anm omega}
сходится и
\ShowEq{lim a1m...anm omega}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{lim aim}
и теоремы
\ref{theorem: limit of sequence, Omega group}
следует, что для заданного
\DrawEq{delta1 in R}{a1m...anm}
существует $M_i$ такое, что из условия
\ShowEq{m>Mi}
следует
\ShowEq{aim in B_o}
Пусть
\ShowEq{M M1 Mn}
Из равенств
\EqRef{aim in B_o},
теоремы
\ref{theorem: c1 cn omega in B}
и условия $m>M$
следует, что
\ShowEq{a1m...anm omega in B_o 1}
\DrawEq{epsilon_1=f(delta_1)}{a1m...anm}
где
\DrawEq{C=|a|+delta}{1n}
Из равенства
\eqRef{C=|a|+delta}{1n}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{a1m...anm}
следует, что
\DrawEq{C>0}{a1m...anm}
Из равенств
\eqRef{epsilon_1=f(delta_1)}{a1m...anm},
\eqRef{C=|a|+delta}{1n}
и утверждения
\eqRef{C>0}{a1m...anm}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon_1=f(delta_1)}{a1m...anm}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $M$ зависит от значения $\delta_1$.
Мы выберем значение $M$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $M$ такое, что из условия
$m>M$
следует
\ShowEq{a1m...anm omega in B_o 2}
Равенство
\EqRef{lim a1m...anm omega}
следует из равенства
\EqRef{a1m...anm omega in B_o 2}
и теоремы
\ref{theorem: limit of sequence, Omega group}.
\end{proof}

\section{Пополнение нормированной \texorpdfstring{$\Omega$}{Omega}-группы}
\label{section: completion of normed Omega group}

\begin{definition}
\label{definition: completion of normed Omega group}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Полная $\Omega$\Hyph группа $B$ называется
\AddIndex{пополнением нормированной $\Omega$\Hyph группы}
{completion of normed Omega group} $A$,\footnote{Существование
пополнения топологического пространства
очень важно, так как позволяет использовать
непрерывность как инструмент для изучения топологического пространства.
Если топологическое пространство имеет дополнительную структуру,
то мы ожидаем, что пополнение имеет такую же структуру.
Смотри определение пополнение метрического пространства в определении
\citeBib{Kolmogorov Fomin}\Hyph 2, страница 71.
Смотри определение пополнение нормированного поля в утверждении
\citeBib{Coppel: Number Theory}\Hyph 6 на странице 270
и в последующем определении на странице 271.
Смотри определение пополнение нормированного векторного пространства
в теореме
\citeBib{978-0486497952}\Hyph 1.11.1 на странице 55.
}
если
\StartLabelItem
\begin{enumerate}
\item
$\Omega$\Hyph группа $A$ является подгруппой
$\Omega$\Hyph группы $B$.\footnote{Точнее,
мы изоморфно отождествляем
$\Omega$\Hyph группу $A$ с некоторой подгруппой
$\Omega$\Hyph группы $B$.
}
\item
\LabelItem{A is everywhere dense in B}
$\Omega$\Hyph группа $A$ всюду плотна в
$\Omega$\Hyph группе $B$.
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
\label{theorem: completion of normed Omega group is unique}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть $B_1$, $B_2$ являются пополнением $\Omega$\Hyph группы $A$.
Существует изоморфизм $\Omega$\Hyph группы\footnote{Мы также говорим,
что пополнение $\Omega$\Hyph группы $A$
единственно с точностью до рассматриваемого изоморфизма.
}
\ShowEq{f:B1->B2}
такой, что
\ShowEq{f:B1->B2 A}
\ShowEq{f:B1->B2 ||}
\end{theorem}
\begin{proof}
Пусть $b_1\in B_1$.
Согласно утверждению
\RefItem{A is everywhere dense in B}
и теореме
\ref{theorem: sequence in dense set}
существует последовательность $A$\Hyph чисел $a_n$ такая, что
\ShowEq{b1=lim an}
Из равенства
\EqRef{b1=lim an}
следует, что последовательность $A$\Hyph чисел $a_n$
является фундаментальной последовательностью
в $\Omega$\Hyph группе $A$.
Следовательно,
последовательность $a_n$ сходится к $b_2$
в полной $\Omega$\Hyph группе $B_2$.
Согласно теореме
\ref{theorem: lim a=lim b},
$B_2$\Hyph число $b_2$ не зависит от выбора
последовательности $a_n$,
сходящейся к $b_1$.
Следовательно,
\ShowEq{fb1=b2}.

Равенство
\EqRef{f:B1->B2 A}
является следствием теоремы
\ref{theorem: For any a there exists sequence}.

Отображение $f$ является биективным, так как выполненное
построение обратимо и мы можем найти $B_1$\Hyph число $b_1$,
соответствующее $B_2$\Hyph числу $b_2$.

Согласно теореме
\ref{theorem: Norm is continues map},
в $\Omega$\Hyph группе $B_1$ верно равенство
\ShowEq{|b1|=lim|an|}
и в $\Omega$\Hyph группе $B_2$ верно равенство
\ShowEq{|b2|=lim|an|}
Равенства
\EqRef{f:B1->B2 ||}
следует из равенств
\EqRef{|b1|=lim|an|},
\EqRef{|b2|=lim|an|}.

Из теорем
\ref{theorem: lim an+bn},
\ref{theorem: lim a1m...anm omega}
следует, что отображение $f$ является изоморфизмом $\Omega$\Hyph группы.
\end{proof}

Доказательство существования
пополнения нормированной $\Omega$\Hyph группы $A$
(теорема
\ref{theorem: completion of normed Omega group})
основано на доказательстве теоремы
\ref{theorem: completion of normed Omega group is unique}.
Если $B$ - полная $\Omega$\Hyph группа,
являющаяся пополнением нормированной $\Omega$\Hyph группы $A$,
то каждое $B$\Hyph число является пределом
фундаментальной последовательности $A$\Hyph чисел.
Поэтому, чтобы построить $\Omega$\Hyph группу $B$,
рассмотрим множество $B'$ фундаментальных
последовательностей $A$\Hyph чисел.

\begin{lemma}
\label{lemma: sim is equivalence relation}
Отношение $\sim$ на множестве $B'$
\ShowEq{sim lim a-b=0}
является отношением эквивалентности.\footnote{Смотри
определение отношения эквивалентности в
\citeBib{Cohn: Universal Algebra}, страница 27.
}
\end{lemma}
\begin{proof}
\ \par
\StartLabelItem
\begin{enumerate}
\item
Так как $a_n=a_n$, то отношение $\sim$ рефлексивно
\ShowEq{a sim a}
\item
Из утверждения
\RefItem{|-a|=|a|}
следует, что
\ShowEq{|a-b|=|b-a| sim}
Следовательно, отношение $\sim$ симметрично
\ShowEq{a sim b b sim a}
\item
Пусть $a_n$, $n=1$, ..., - фундаментальная последовательность
$A$\Hyph чисел.
Пусть $b_n$, $c_n$, $n=1$, ..., - последовательности $A$\Hyph чисел.
Равенство
\DrawEq{lim a-b=0}{sim}
следует из утверждения
\ShowEq{a sim b}.
Равенство
\DrawEq{lim a-c=0}{sim}
следует из утверждения
\ShowEq{a sim c}.

Из теоремы
\ref{theorem: lim a-b=0 fundamental}
и равенства
\eqRef{lim a-b=0}{sim}
следует, что последовательность $b_n$ фундаментальна.
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\eqRef{lim a-b=0}{sim}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_1$ такое, что
\DrawEq{|an-bn|<epsilon/2}{sim}
для любого $n>N_1$.

Из теоремы
\ref{theorem: lim a-b=0 fundamental}
и равенства
\eqRef{lim a-c=0}{sim}
следует, что последовательность $c_n$ фундаментальна.
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\eqRef{lim a-c=0}{sim}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_2$ такое, что
\DrawEq{|an-cn|<epsilon/2}{sim}
для любого $n>N_2$.

Пусть
\ShowEq{N N1 N2}
Из неравенств
\eqRef{|an-bn|<epsilon/2}{sim},
\eqRef{|an-cn|<epsilon/2}{sim}
и утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|bn-cn|<epsilon}
для любого $n>N$.
Равенство
\ShowEq{lim b-c=0}
следует из определения
\ref{definition: limit of sequence, Omega group}.
Утверждение
\ShowEq{b sim c}
следует из равенства
\EqRef{lim b-c=0}.
\item
Из рассуждения
\RefItem{a sim b sim c}
следует, что отношение $\sim$ транзитивно
\ShowEq{a sim b sim c}
\end{enumerate}
Лемма следует
из утверждений
\ShowEq{sim is equivalence relation}
\end{proof}

\begin{lemma}
\label{lemma: a sim b}
\ShowEq{a sim b}
тогда и только тогда, когда
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $n_0$ такое, что
\DrawEq{bn in B(an)}{lemma}
для любого $n>n_0$.
\end{lemma}
\begin{proof}
Согласно определению
\ref{definition: open ball},
утверждение
\eqRef{bn in B(an)}{lemma}
верно тогда и только тогда, когда
\ShowEq{|an-bn|<epsilon}
Теорема верна согласно определению
\ref{definition: limit of sequence, Omega group}.
\end{proof}

Пусть $B$ является множеством классов эквивалентных фундаментальных
последовательностей $A$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{[a]}
для класса последовательностей, эквивалентных последовательности $a_n$.

\begin{lemma}
\label{lemma: B is Abelian group}
Множество $B$ является абелевой группой относительно операции
\ShowEq{[a]+[b]=[a+b]}
\end{lemma}
\begin{proof}
Пусть $A$ - нормированная $\Omega$\Hyph группа.
Пусть последовательности $A$\Hyph чисел
\ShowEq{an, bn}
являются фундаментальными последовательностями.

{\hangindent=1cm
\setlength{\parindent}{1.6cm}
\begin{lemma}
\label{lemma: an+bn fundamental}
Последовательность $A$\Hyph чисел
\ShowEq{an+bn}
является фундаментальной.
\end{lemma}

{\sc Доказательство.}
Так как последовательность $A$\Hyph чисел $a_n$
является фундаментальной,
то согласно определению
\ref{definition: fundamental sequence}
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_a$ такое, что
\DrawEq{|ap-aq|<epsilon/2}{+}
для любых $p$, $q>N_a$.
Так как последовательность $A$\Hyph чисел $b_n$
является фундаментальной,
то согласно определению
\ref{definition: fundamental sequence}
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_b$ такое, что
\ShowEq{|bp-bq|<epsilon/2}
для любых $p$, $q>N_b$.
Пусть
\ShowEq{N Na Nb}
Из неравенств
\ShowEq{an+bn fundamental 1}
и условия $n>N$
следует, что
\ShowEq{an+bn fundamental}
Следовательно,
согласно определению
\ref{definition: fundamental sequence},
последовательность $A$\Hyph чисел
\ShowEq{an+bn}
является фундаментальной.

\begin{lemma}
\label{lemma: a+b sim c+d}
Пусть
\ShowEq{a sim c},
\ShowEq{b sim d}.
Тогда
\ShowEq{a+b sim c+d}
\end{lemma}

{\sc Доказательство.}
Равенство
\DrawEq{lim a-c=0}{+}
следует из утверждения
\ShowEq{a sim c}.
Равенство
\ShowEq{lim b-d=0}
следует из утверждения
\ShowEq{b sim d}.

Из теоремы
\ref{theorem: lim a-b=0 fundamental}
и равенства
\eqRef{lim a-c=0}{+}
следует, что последовательность $c_n$ фундаментальна.
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\eqRef{lim a-c=0}{+}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_1$ такое, что
\DrawEq{|an-cn|<epsilon/2}{+}
для любого $n>N_1$.

Из теоремы
\ref{theorem: lim a-b=0 fundamental}
и равенства
\EqRef{lim b-d=0}
следует, что последовательность $d_n$ фундаментальна.
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\EqRef{lim b-d=0}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_2$ такое, что
\ShowEq{|bn-dn|<epsilon/2}
для любого $n>N_2$.

Пусть
\ShowEq{N N1 N2}
Из неравенств
\EqRef{|c12-a12|<|c-a|12},
\eqRef{|an-cn|<epsilon/2}{+},
\EqRef{|bn-dn|<epsilon/2}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|an+bn|-|cn+dn|<epsilon}
для любого $n>N$.
Равенство
\ShowEq{lim (a+b)-(c+d)=0}
следует из определения
\ref{definition: limit of sequence, Omega group}.
Следовательно, утверждение
\EqRef{a+b sim c+d}
следует из равенства
\EqRef{lim (a+b)-(c+d)=0}.

}%\hangindent

Из леммы
\ref{lemma: an+bn fundamental}
следует, что последовательность
\ShowEq{an+bn}
является фундаментальной последовательностью.
Из леммы
\ref{lemma: a+b sim c+d}
следует, что операция
\EqRef{[a]+[b]=[a+b]}
определена корректно.

\StartLabelItem
\begin{enumerate}
\item
Из равенства
\ShowEq{an+(bn+cn)=(an+bn)+cn}
следует, что операция
\EqRef{[a]+[b]=[a+b]}
ассоциативна
\ShowEq{[a]+([b]+[c])}
\item
Из равенства
\ShowEq{an+bn=bn+an}
следует, что операция
\EqRef{[a]+[b]=[a+b]}
коммутативна
\ShowEq{[a]+[b]=[b]+[a]}
\item
Если положить $b_n=0$, то из равенства
\ShowEq{an+0=an}
следует
\ShowEq{[a]+[0]=[a]}
\item
Из равенства
\ShowEq{an+(-an)=0}
следует
\ShowEq{[a]+[-a]=[0]}
Следовательно, мы можем положить
\ShowEq{-[a]=[-a]}
\end{enumerate}
Лемма является следствием утверждений
\ShowEq{B is Abelian group}
\end{proof}

\begin{lemma}
\label{lemma: [a1n]omega=[a1n omega]}
Мы определим операцию
\ShowEq{omega in Omega}
на множестве $B$,
пользуясь равенством
\ShowEq{[a1n]omega=[a1n omega]}
\end{lemma}
\begin{proof}
Пусть $A$ - нормированная $\Omega$\Hyph группа.

{\hangindent=1cm
\setlength{\parindent}{1.6cm}
\begin{lemma}
\label{lemma: a1m...anm omega fundamental}
Пусть последовательности $A$\Hyph чисел
\ShowEq{a1m...anm}
являются фундаментальными последовательностями.
Последовательность $A$\Hyph чисел
\ShowEq{a1m...anm omega}
является фундаментальной.
\end{lemma}

{\sc Доказательство.}
Так как последовательность
\ShowEq{aim}
является фундаментальной последовательностью \(A\)\Hyph чисел,
то согласно теореме
\ref{theorem: fundamental sequence}
следует, что для заданного
\DrawEq{delta1 in R}{a1m...anm fundamental}
существует, зависящее от \(\delta_1\), натуральное число $M_i$ такое, что
\ShowEq{aiq in B(aip,d1)}
для любых $p$, $q>M_i$.
Пусть
\ShowEq{M M1 Mn}
Из утверждений
\EqRef{aiq in B(aip,d1)}
и теоремы
\ref{theorem: c1 cn omega in B}
следует, что
\ShowEq{a1m...anm omega fundamental 1}
\DrawEq{epsilon_1=f(delta_1)}{a1m...anm fundamental}
где
\DrawEq{C=|ap|+d1}{a1m...anm fundamental}
Из равенства
\eqRef{C=|ap|+d1}{a1m...anm fundamental}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{a1m...anm fundamental}
следует, что
\DrawEq{C>0}{a1m...anm fundamental}
Из равенств
\eqRef{epsilon_1=f(delta_1)}{a1m...anm fundamental},
\eqRef{C=|ap|+d1}{a1m...anm fundamental}
и утверждения
\eqRef{C>0}{a1m...anm fundamental}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon_1=f(delta_1)}{a1m...anm fundamental}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $M$ зависит от значения $\delta_1$.
Мы выберем значение $M$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $M$ такое, что из условия
$p$, $q>M$
следует
\ShowEq{a1m...anm omega fundamental 2}
Из утверждения
\EqRef{a1m...anm omega fundamental 2}
и теоремы
\ref{theorem: fundamental sequence}
следует, что последовательность $A$\Hyph чисел
\ShowEq{a1m...anm omega}
является фундаментальной последовательностью.

\begin{lemma}
\label{lemma: a1n omega sim c1n omega}
Пусть последовательности $A$\Hyph чисел
\ShowEq{a1m...anm}
\ShowEq{c1m...cnm}
являются фундаментальными последовательностями.
Пусть
\ShowEq{a1n sim c1n}
Тогда
\ShowEq{a1n omega sim c1n omega}
\end{lemma}

{\sc Доказательство.}
Из утверждения
\EqRef{a1n sim c1n}
и леммы
\ref{lemma: a sim b}
следует, что
для заданного
\DrawEq{delta1 in R}{a1n omega sim c1n omega}
существует, зависящее от $\delta_1$, натуральное число $M_1$ такое, что
\ShowEq{c in B(a,d1)}
для любого $m>M_1$.
Пусть
\ShowEq{M M1 Mn}
Из утверждений
\EqRef{c in B(a,d1)}
и теоремы
\ref{theorem: c1 cn omega in B}
следует, что
\ShowEq{c1n omega in B(a1n omega) 1}
\DrawEq{epsilon_1=f(delta_1)}{f a1 a2 sim f b1 b2}
где
\DrawEq{C=|an|+d1}{a1n omega sim c1n omega}
Из равенства
\eqRef{C=|an|+d1}{a1n omega sim c1n omega}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{f a1 a2 sim f b1 b2}
следует, что
\DrawEq{C>0}{a1n omega sim c1n omega}
Из равенств
\eqRef{epsilon_1=f(delta_1)}{f a1 a2 sim f b1 b2},
\eqRef{C=|an|+d1}{a1n omega sim c1n omega}
и утверждения
\eqRef{C>0}{a1n omega sim c1n omega}
следует, что $\epsilon_1$ является
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon_1=f(delta_1)}{f a1 a2 sim f b1 b2}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $M$ зависит от значения $\delta_1$.
Мы выберем значение $M$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $M$ такое, что из условия
$m>M$
следует
\ShowEq{c1n omega in B(a1n omega) 2}
Утверждение
\EqRef{a1n omega sim c1n omega}
следует из утверждения
\EqRef{c1n omega in B(a1n omega) 2}
и леммы
\ref{lemma: a sim b}.

}%\hangindent

Из леммы
\ref{lemma: a1m...anm omega fundamental}
следует, что последовательность
\ShowEq{a1m...anm omega}
является фундаментальной последовательностью.
Из леммы
\ref{lemma: a1n omega sim c1n omega}
следует, что операция
\EqRef{[a1n]omega=[a1n omega]}
определена корректно.
\end{proof}

\begin{lemma}
\label{lemma: B is Abelian Omega group}
Абелева группа $B$ является абелевой $\Omega$\Hyph группой.
\end{lemma}
\begin{proof}
Согласно определению
\ref{definition: Omega group},
операция
\ShowEq{omega in Omega}
полиаддитивна.
Из равенства
\ShowEq{(aim+bim)omega=aim omega+bim omega}
следует, что операция
\EqRef{[a1n]omega=[a1n omega]}
полиаддитивна
\ShowEq{([ai]+[bi])omega}
Лемма является следствием определения
\ref{definition: Omega group}.
\end{proof}

\begin{lemma}
\label{lemma: a fundamental => |a| fundamental}
Пусть последовательность $a_n$ является фундаментальной.
Тогда последовательность $\|a_n\|$ является фундаментальной.
\end{lemma}
\begin{proof}
Согласно определению
\ref{definition: fundamental sequence},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\DrawEq{|ap-aq|<epsilon}{||}
для любых $p$, $q>N$.
Из неравенств
\EqRef{|a-b|>|a|-|b|},
\eqRef{|ap-aq|<epsilon}{||}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|ap|-|aq|<epsilon}
для любого $n>N$.
Согласно определению
\ref{definition: fundamental sequence},
последовательность $\|a_n\|$ является фундаментальной.
\end{proof}

\begin{lemma}
\label{lemma: a sym b => lim|a|=lim|b|}
Пусть
\ShowEq{a sim b}.
Тогда
\ShowEq{lim|a|=lim|b|}
\end{lemma}
\begin{proof}
Равенство
\DrawEq{lim a-b=0}{||}
следует из утверждения
\ShowEq{a sim b}.
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\eqRef{lim a-b=0}{||}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|an-bn|<epsilon}
для любого $n>N$.
Из неравенства
\EqRef{|a-b|>|a|-|b|}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|an|-|bn|<epsilon}
для любого $n>N$.
Согласно определению
\ref{definition: limit of sequence, Omega group},
следует, что
\ShowEq{lim |an|-|bn|=0}
Из леммы
\ref{lemma: a fundamental => |a| fundamental}
следует, что последовательности $\|a_n\|$ и $\|b_n\|$
фундаментальны.
Равенство
\EqRef{lim|a|=lim|b|}
следует из теоремы
\ref{theorem: lim a=lim b}.
\end{proof}

\begin{lemma}
\label{lemma: |[a]|=lim |a|}
Мы определим норму на $\Omega$\Hyph группе $B$ равенством
\ShowEq{|[a]|=lim |a|}
\end{lemma}
\begin{proof}
Из лемм
\ref{lemma: a fundamental => |a| fundamental},
\ref{lemma: a sym b => lim|a|=lim|b|}
следует, что равенство
\EqRef{|[a]|=lim |a|}
является корректным определением
отображения
\ShowEq{B->R}

\StartLabelItem
\begin{enumerate}
\item
Согласно утверждению
\RefItem{|a|>=0},
\ShowEq{|an|>=0}.
Следовательно,\footnote{Смотри,
например,
\citeBib{Smirnov vol 1}, страница 58, утверждение 3.
}
\ShowEq{lim|an|>=0}
Из равенства
\EqRef{|[a]|=lim |a|}
и неравенства
\EqRef{lim|an|>=0}
следует, что
\ShowEq{|[a]|>=0}.
Следовательно, утверждение
\RefItem{|a|>=0}
верно для отображения
\EqRef{|[a]|=lim |a|}.
\item
Пусть
\ShowEq{|[a]|=0}.
Из равенства
\EqRef{|[a]|=lim |a|}
следует, что
\ShowEq{lim|an|=0}
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\EqRef{lim|an|=0}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|an|<epsilon}
для любого $n>N$.
Согласно определению
\ref{definition: limit of sequence, Omega group},
\ShowEq{lim an=0}
Из равенств
\EqRef{lim an=0},
\EqRef{sim lim a-b=0}
следует, что
\ShowEq{an sim 0}
Согласно определению
\EqRef{[a]},
\ShowEq{[a]=[0]}.
Следовательно, утверждение
\RefItem{|a|=0}
верно для отображения
\EqRef{|[a]|=lim |a|}.
\item
Согласно утверждению
\RefItem{|a+b|<=|a|+|b|},
\ShowEq{|an+bn|<=|an|+|bn|}
Следовательно,\footnote{Смотри,
например,
\citeBib{Smirnov vol 1}, страница 58, утверждение 3.
}
\ShowEq{lim|an+bn|<=lim|an|+lim|bn|}
Из равенства
\EqRef{|[a]|=lim |a|}
и неравенства
\EqRef{lim|an+bn|<=lim|an|+lim|bn|}
следует, что
\ShowEq{|[a+b]|<=|[a]|+|[b]|}
Из неравенства
\EqRef{|[a+b]|<=|[a]|+|[b]|}
и равенства
\EqRef{[a]+[b]=[a+b]}
следует, что
\ShowEq{|[a]+[b]|<=|[a]|+|[b]|}
Следовательно, утверждение
\RefItem{|a+b|<=|a|+|b|}
верно для отображения
\EqRef{|[a]|=lim |a|}.
\item
Согласно утверждению
\RefItem{|-a|=|a|},
\ShowEq{|-an|=|an|}.
Согласно теореме
\ref{theorem: lim a=lim b}
\ShowEq{lim|-an|=lim|an|}
Из равенств
\EqRef{|[a]|=lim |a|},
\EqRef{lim|-an|=lim|an|}
следует, что
\ShowEq{|[-a]|=|[a]|}
Из равенства
\EqRef{|[-a]|=|[a]|}
и утверждения
\RefItem{-[a]=[-a]}
следует, что
\ShowEq{|-[a]|=|[a]|}
Следовательно, утверждение
\RefItem{|-a|=|a|}
верно для отображения
\EqRef{|[a]|=lim |a|}.
\end{enumerate}

Согласно утверждениям
\ShowEq{|[a]|=lim |a| 1}
и определению
\ref{definition: norm on Omega group},
отображение
\EqRef{|[a]|=lim |a|}
является нормой на $\Omega$\Hyph группе $B$.
\end{proof}

\begin{lemma}
\label{lemma: Omega group A is subgroup of B}
$\Omega$\Hyph группа $A$ является подгруппой
$\Omega$\Hyph группы $B$.
Из условий $a\in A$ и
\DrawEq{a=lim an}{}
следует
\ShowEq{|a|=|[a]|}
\end{lemma}
\begin{proof}
Пусть $a\in A$.
Согласно определениям
\ref{definition: limit of sequence, Omega group},
\ref{definition: fundamental sequence},
последовательность
\ShowEq{an=a}
является фундаментальной и сходится к $a$.
Согласно определению
\EqRef{sim lim a-b=0}
и теореме
\ref{theorem: lim a=lim b},
из условия
\ShowEq{a sim b}
следует
\ShowEq{a=lim bn}
Поэтому мы можем отождествить $a$ и $[a_n]$.
Согласно теоремам
\ref{theorem: lim an+bn},
\ref{theorem: lim a1m...anm omega},
это отождествление является гомоморфизмом
$\Omega$\Hyph группы $A$ в $\Omega$\Hyph группу $B$.
Из равенства
\EqRef{|[a]|=lim |a|}
и теоремы
\ref{theorem: Norm is continues map}
следует, что
\ShowEq{|[a]|=|a|}
Равенство
\EqRef{|a|=|[a]|}
следует из равенства
\EqRef{|[a]|=|a|}.
\end{proof}

\begin{lemma}
\label{lemma: [an]=lim an}
Для любого $B$\Hyph числа $a$ существует последовательность
$A$\Hyph чисел такая, что
\DrawEq{a=lim an}{a=[an]}
\end{lemma}
\begin{proof}
Существует фундаментальная последовательность
$A$\Hyph чисел $a_n$ такая, что
\ShowEq{a=[an]}.
Согласно определению
\ref{definition: fundamental sequence},
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_1$ такое, что
\DrawEq{|ap-aq|<epsilon/2}{a=[an]}
для любых $p$, $q>N_1$.
Согласно леммам
\ref{lemma: B is Abelian group},
\ref{lemma: Omega group A is subgroup of B},
для любого $q>N_1$
\ShowEq{a-aq}
Согласно лемме
\ref{lemma: |[a]|=lim |a|}
\ShowEq{|a-aq|=}
Согласно определению
\ref{definition: limit of sequence, Omega group},
из равенства
\EqRef{|a-aq|=}
следует, что
для любого
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N_2$ такое, что
\ShowEq{|a-aq|<epsilon/2}
для любого $n>N_2$.
Неравенство\footnote{Неравенство
\ShowEq{|a-aq|<epsilon/2 2}
также следует из неравенства
\EqRef{|a-aq|<epsilon/2}.
Неравенство
\ShowEq{|a-aq|<epsilon/2 3}
следует из неравенства
\EqRef{|a-aq|<epsilon/2 2}.
Из неравенств
\eqRef{|ap-aq|<epsilon/2}{a=[an]},
\EqRef{|a-aq|<epsilon/2 3}
и утверждения
\RefItem{|a|>=0}
следует, что
\ShowEq{|a-aq|>=0}
Однако это утверждение очевидно и не интересно для нас.
}
\ShowEq{|a-aq|<epsilon/2 1}
следует из неравенства
\EqRef{|a-aq|<epsilon/2}.
Пусть
\ShowEq{N N1 N2}
Из неравенств
\eqRef{|ap-aq|<epsilon/2}{a=[an]},
\EqRef{|a-aq|<epsilon/2 1}
следует, что
для заданного
\ShowEq{epsilon in R}
существует, зависящее от $\epsilon$, натуральное число $N$ такое, что
\ShowEq{|a-aq|<epsilon}
для любых $q>N$.
Равенство
\eqRef{a=lim an}{a=[an]}
следует из определения
\ref{definition: limit of sequence, Omega group}.
\end{proof}

\begin{theorem}
\label{theorem: completion of normed Omega group}
Пополнение нормированной $\Omega$\Hyph группы $A$ существует.
\end{theorem}
\begin{proof}
Согласно лемме
\ref{lemma: Omega group A is subgroup of B},
$\Omega$\Hyph группа $A$ является подгруппой
$\Omega$\Hyph группы $B$.
Из леммы
\ref{lemma: [an]=lim an}
и теоремы
\ref{theorem: sequence in dense set}
следует, что
$\Omega$\Hyph группа $A$ всюду плотна в
$\Omega$\Hyph группе $B$.
Согласно определению
\ref{definition: completion of normed Omega group},
чтобы доказать теорему,
необходимо доказать, что $\Omega$\Hyph группа $B$
является полной.

Пусть $b_n$ - фундаментальная последовательность $B$\Hyph чисел.
Согласно определениям
\ref{definition: open ball},
\ref{definition: closure of set},
\ref{definition: dense in set},
для любого $n>0$ существует $a_n\in A$ такой, что
\ShowEq{|an-bn|<1/n}
Равенство
\DrawEq{lim a-b=0}{completion}
следует из определения
\ref{definition: limit of sequence, Omega group}.
Из равенства
\eqRef{lim a-b=0}{completion}
и теоремы
\ref{theorem: lim a-b=0 fundamental}
следует, что последовательность $A$\Hyph чисел $a_n$
является фундаментальной.
Согласно определению
\EqRef{[a]}
существует $B$\Hyph число $[a_n]$.
Согласно теореме
\ref{theorem: lim a=lim b}
и лемме
\ref{lemma: [an]=lim an}
\ShowEq{lim b=[a]}
Из равенства
\EqRef{lim b=[a]}
следует, что $\Omega$\Hyph группа $B$
является полной.
\end{proof}

\section{\texorpdfstring{$\Omega$}{Omega}-группа отображений}

\begin{theorem}
Пусть
\ShowEq{set of maps to Omega group}
- множество отображений множества $X$ в $\Omega$\Hyph группу $A$.
Мы можем определить структуру $\Omega$\Hyph группы на множестве
\ShowEq{M(X,A)}.
\end{theorem}
\begin{proof}
Пусть
\ShowEq{f g in M}
Тогда мы положим
\ShowEq{f+g=}
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Для отображений
\ShowEq{fi in M}
мы положим
\ShowEq{fi omega}
\end{proof}

Так как $X$ - произвольное множество, мы не можем определить
норму в $\Omega$\Hyph группе
\ShowEq{M(X,A)}.
Однако мы можем определить сходимость последовательности в
\ShowEq{M(X,A)};
следовательно, мы можем определить топологию в
\ShowEq{M(X,A)}

\begin{definition}
\label{definition: limit of sequence, map to Omega group}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
Отображение
\ShowEq{f M(X,A)}
называется
\AddIndex{пределом последовательности}{limit of sequence}
$f_n$, если для любого $x\in X$
\DrawEq{f(x)=lim}{}
Мы будем также говорить, что
\AddIndex{последовательность $f_n$ сходится}{sequence converges}
к отображению $f$.
\qed
\end{definition}

Из определений
\ref{definition: limit of sequence, Omega group},
\ref{definition: limit of sequence, map to Omega group}
следует, что если последовательность $f_n$ сходится к $f$,
то для любого
\ShowEq{epsilon in R}
существует $N(x)$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N(x)$.

\begin{definition}
\label{definition: sequence converges uniformly}
Пусть
\ShowEq{fn M(X,A)}
- последовательность отображений в нормированную
$\Omega$\Hyph группу $A$.
\AddIndex{Последовательность $f_n$ сходится равномерно}
{sequence converges uniformly}
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) - f(x)}
для любого $n>N$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: sequence converges uniformly}
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) in B(f(x))}
для любого $n>N$.
\end{theorem}
\begin{proof}
Следствие определений
\ref{definition: open ball},
\ref{definition: sequence converges uniformly}.
\end{proof}

\begin{theorem}
\label{theorem: sequence converges uniformly, fn-fm}
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x)-fm(x)|<e}
для любых \(n\), \(m>N\).
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: sequence converges uniformly},
для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{|fn(x) - f(x)|<e/2}
для любого $n>N$.
Для любых \(n\), \(m>N\),
из утверждения
\RefItem{|a+b|<=|a|+|b|}
и неравенства
\EqRef{|fn(x) - f(x)|<e/2}
следует, что
\ShowEq{->|fn(x)-fm(x)|<e}
Неравенство
\EqRef{|fn(x)-fm(x)|<e}
следует из неравенства
\EqRef{->|fn(x)-fm(x)|<e}.
\end{proof}

\begin{theorem}
\label{theorem: sequence converges uniformly, fn in B(fm)}
Последовательность отображений
\ShowEq{fn M(X,A)}
в нормированную
$\Omega$\Hyph группу $A$ сходится равномерно
к отображению $f$,
если для любого
\ShowEq{epsilon in R}
существует $N$ такое, что
\ShowEq{fn(x) in B(fm(x))}
для любых \(n\), \(m>N\).
\end{theorem}
\begin{proof}
Следствие определения
\ref{definition: open ball}
и теоремы
\ref{theorem: sequence converges uniformly, fn-fm}.
\end{proof}

\begin{theorem}
\label{theorem: h=f+g, converges uniformly}
Пусть последовательность отображений
\ShowEq{fn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f$.
Пусть последовательность отображений
\ShowEq{gn M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $g$.
Тогда последовательность отображений
\ShowEq{hn=fn+gn}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f+g}{converges uniformly}
\end{theorem}
\begin{proof}
Из равенства
\DrawEq{f(x)=lim}{}
и теоремы
\ref{theorem: sequence converges uniformly}
следует, что для заданного
\ShowEq{epsilon in R}
существует $N_a$ такое, что из условия
\ShowEq{n>Na}
следует
\ShowEq{fn in B_o}
Из равенства
\ShowEq{g(x)=lim}
и теоремы
\ref{theorem: sequence converges uniformly}
следует, что для заданного
\ShowEq{epsilon in R}
существует $N_b$ такое, что из условия
\ShowEq{n>Nb}
следует
\ShowEq{gn in B_o}
Пусть
\ShowEq{N Na Nb}
Из равенств
\EqRef{fn in B_o},
\EqRef{gn in B_o},
теоремы
\ref{theorem: c1+c2 in B}
и условия $n>N$
следует, что
\ShowEq{fn+gn in B_o}
Равенство
\eqRef{h=f+g}{converges uniformly}
следует из равенства
\EqRef{fn+gn in B_o}
и теоремы
\ref{theorem: sequence converges uniformly}.
\end{proof}

\begin{theorem}
\label{theorem: h=f1...fn omega, converges uniformly}
Пусть $A$ - полная $\Omega$\Hyph группа.
Пусть
\ShowEq{omega in Omega}
- $n$\Hyph арная операция.
Пусть последовательность отображений
\ShowEq{fim M(X,A)}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению $f_i$.
Пусть множество значений отображения
$f_i$
компактно.
Тогда последовательность отображений
\ShowEq{hm=f1m...fnm omega}
в полную $\Omega$\Hyph группу $A$
сходится равномерно
к отображению
\DrawEq{h=f1...fn omega}{converges uniformly}
\end{theorem}
\begin{proof}
Из равенства
\DrawEq{fi(x)=lim}{}
и теоремы
\ref{theorem: sequence converges uniformly}
следует, что для заданного
\DrawEq{delta1 in R}{f1m...fnm}
существует $M_i$ такое, что из условия
\ShowEq{m>Mi}
следует
\ShowEq{fim in B_o}
Пусть
\ShowEq{M M1 Mn}
Из равенств
\EqRef{fim in B_o},
теоремы
\ref{theorem: c1 cn omega in B}
и условия $m>M$
следует, что
\ShowEq{f1m...fnm omega in B_o 1}
\DrawEq{epsilon_1=f(delta_1)}{f1m...fnm}
где
\DrawEq{C=|f|+delta}{f1m...fnm}
Значение \(C_i\) зависит от \(x\).
Поэтому $\epsilon_1$ также зависит от \(x\).
Для оценки равномерной сходимости
нам необходимо выбрать максимальное значение $\epsilon_1$.
Для заданного \(\delta_1\), значение $\epsilon_1$
является полилинейным отображением значений \(C_i\).
Следовательно, $\epsilon_1$ имеет максимальное значение,
когда каждое \(C_i\) имеет максимальное значение.
Так как мы рассматриваем оценку значения \(\epsilon_1\)
справа,
для нас неважно одновременно ли \(C_i\) приобретают
максимальные значения.
Так как множество значений отображения
$f_i$
компактно,
то, согласно теореме
\ref{theorem: norm of compact set is bounded},
определена следующая величина
\DrawEq{F=sup|f|}{f1m...fnm}
Из равенства
\eqRef{F=sup|f|}{f1m...fnm}
и утверждения
\RefItem{|a|>=0}
следует, что
\DrawEq{F>0}{f1m...fnm}
Из равенств
\eqRef{C=|f|+delta}{f1m...fnm},
\eqRef{F=sup|f|}{f1m...fnm}
следует, что мы можем положить
\DrawEq{C=F+delta}{f1m...fnm}
Из равенства
\eqRef{C=F+delta}{f1m...fnm}
и утверждений
\eqRef{F>0}{f1m...fnm},
\eqRef{delta1 in R}{f1m...fnm}
следует, что
\DrawEq{C>0}{f1m...fnm}
Из равенств
\eqRef{epsilon_1=f(delta_1)}{f1m...fnm},
\eqRef{C=F+delta}{f1m...fnm}
и утверждения
\eqRef{C>0}{f1m...fnm}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon_1=f(delta_1)}{f1m...fnm}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $M$ зависит от значения $\delta_1$.
Мы выберем значение $M$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $M$ такое, что из условия
$m>M$
следует
\ShowEq{f1m...fnm omega in B_o 2}
Равенство
\eqRef{h=f1...fn omega}{converges uniformly}
следует из равенства
\EqRef{f1m...fnm omega in B_o 2}
и теоремы
\ref{theorem: sequence converges uniformly}.
\end{proof}




==> Omega.Representation.Russian.tex <==
%auto-ignore
\input{Omega.Representation.Eq}
\ifx\PrintBook\Defined
\chapter{Представление \texorpdfstring{$\Omega$}{Omega}-группы}
\fi

\section{Представление \texorpdfstring{$\Omega$}{Omega}-группы}

\begin{definition}
\label{definition: norm of representation}
Пусть
\ShowEq{A1->*A2}
представление\footnote{Смотри определение
\xRef{0912.3315}{definition: Tstar representation of algebra},
представления универсальной алгебры.
Согласно определению
\xRef{1211.6965}{definition: module over ring},
модуль - это представление кольца в абелевой группе.
Так как кольцо и абелева группа являются $\Omega$\Hyph группами,
то модуль - это представление $\Omega$\Hyph группы.
}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Величина
\ShowEq{norm of representation}
\ShowEq{norm of representation, definition}
называется
\AddIndex{нормой представления}{norm of representation} $f$.
\qed
\end{definition}

\begin{theorem}
\label{theorem: |fab|<|f||a||b|}
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Тогда
\ShowEq{|fab|<|f||a||b|}
\end{theorem}
\begin{proof}
Из равенства
\EqRef{norm of representation, definition}
следует, что
\ShowEq{|fab|<|f||a||b| 1}
Неравенство
\EqRef{|fab|<|f||a||b|}
следует из неравенства
\EqRef{|fab|<|f||a||b| 1}.
\end{proof}

\begin{theorem}
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Верно следующее неравенство
\ShowEq{|f(c-a)|<|f||c-a|}
где
\ShowEq{C12=max(a,c)}
\end{theorem}
\begin{proof}
Согласно определениям
\ref{definition: Omega group},
\xRef{0912.3315}{definition: Tstar representation of algebra},
\ShowEq{|f(c-a)|<|f||c-a| 1}
Из равенства
\EqRef{|f(c-a)|<|f||c-a| 1}
и утверждения
\RefItem{|a+b|<=|a|+|b|}
следует, что
\ShowEq{|f(c-a)|<|f||c-a| 2}
Из равенства
\EqRef{C12=max(a,c)}
и теоремы
\ref{theorem: |fab|<|f||a||b|}
следует, что
\ShowEq{|f(c-a)|<|f||c-a| 3}
Утверждение
\EqRef{|f(c-a)|<|f||c-a|}
следует из неравенств
\EqRef{|f(c-a)|<|f||c-a| 2},
\EqRef{|f(c-a)|<|f||c-a| 3}.
\end{proof}

\begin{theorem}
\label{theorem: f c1 c2 in B}
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Для
\ShowEq{c1 in A1}
пусть
\ShowEq{c1 in B()}
Для
\ShowEq{c2 in A2}
пусть
\ShowEq{c2 in B()}
Тогда
\ShowEq{f c1 c2 in B}
где
\ShowEq{C=|a|+R 12}
\end{theorem}
\begin{proof}
Согласно определению
\ref{definition: open ball}
\ShowEq{f c1 c2 in B 1}
Неравенство
\DrawEq{|c|<|a|+R}{12}
следует из неравенства
\EqRef{f c1 c2 in B 1}
и утверждения
\RefItem{|a+b|<=|a|+|b|}.
Неравенство
\ShowEq{C<|a|+R 12}
следует из неравенства
\eqRef{|c|<|a|+R}{12}
и равенства
\EqRef{C12=max(a,c)}.
Равенство
\EqRef{C=|a|+R 12}
следует из неравенства
\EqRef{C<|a|+R 12}.
Утверждение
\EqRef{f c1 c2 in B}
следует из неравенств
\EqRef{|f(c-a)|<|f||c-a|},
\EqRef{f c1 c2 in B 1},
равенства
\EqRef{C=|a|+R 12}
и определения
\ref{definition: open ball}.
\end{proof}

\begin{theorem}
\label{theorem: lim f c1n c2n}
Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность $A_1$\Hyph чисел
\ShowEq{a1n}
сходится и
\ShowEq{lim a1n}
Пусть последовательность $A_2$\Hyph чисел
\ShowEq{a2n}
сходится и
\ShowEq{lim a2n}
Тогда последовательность $A_2$\Hyph чисел
\ShowEq{f a1n a2n}
сходится и
\ShowEq{lim f a1n a2n}
\end{theorem}
\begin{proof}
Пусть
\DrawEq{delta1 in R}{a1m a2m}
Из равенства
\EqRef{lim a1n}
и теоремы
\ref{theorem: limit of sequence, Omega group}
следует, что для заданного
\(\delta_1\)
существует $N_1$ такое, что из условия
\ShowEq{n>N1}
следует
\ShowEq{a1n in B_o}
Из равенства
\EqRef{lim a2n}
и теоремы
\ref{theorem: limit of sequence, Omega group}
следует, что для заданного
\(\delta_1\)
существует $N_2$ такое, что из условия
\ShowEq{n>N2}
следует
\ShowEq{a2n in B_o}
Пусть
\ShowEq{N N1 N2}
Из равенств
\EqRef{a1n in B_o},
\EqRef{a2n in B_o},
теоремы
\ref{theorem: f c1 c2 in B}
и условия $n>N$
следует, что
\ShowEq{f a1n a2n in B_o 1}
\DrawEq{epsilon12=f(delta12)}{a}
где
\DrawEq{C=|a|+delta}{12}
Из равенства
\eqRef{C=|a|+delta}{12}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{a1m a2m}
следует, что
\DrawEq{C>0}{a1n a2n}
Из равенств
\eqRef{epsilon12=f(delta12)}{a},
\eqRef{C=|a|+delta}{12}
и утверждения
\eqRef{C>0}{a1n a2n}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon12=f(delta12)}{a}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $N$ зависит от значения $\delta_1$.
Мы выберем значение $N$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $N$ такое, что из условия
$N>N$
следует
\ShowEq{f a1n a2n in B_o 2}
Равенство
\EqRef{lim f a1n a2n}
следует из равенства
\EqRef{f a1n a2n in B_o 2}
и теоремы
\ref{theorem: limit of sequence, Omega group}.
\end{proof}

\begin{theorem}
Представление
\ShowEq{A1->*A2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
может быть продолжено до представления
\ShowEq{A1->*M(X,A2)}
$\Omega_1$\Hyph группы $A_1$
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где
\ShowEq{g in M(X,A2)}
\ShowEq{f*:A1->*M(X,A2)}
\end{theorem}
\begin{proof}
Чтобы доказать теорему, мы должны показать, что отображение
$f^*$ является гомоморфизмом $\Omega_1$\Hyph группы $A_1$ и
для любого $a_1\in A_1$ отображение
$f^*(a_1)$ является гомоморфизмом $\Omega_2$\Hyph группы
\ShowEq{M(X,A2)}.

Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
$f$ является гомоморфизмом $\Omega_1$\Hyph группы $A_1$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega1}
и произвольных
\ShowEq{a1...an A1}
следующее равенство верно
\DrawEq{f is homomorphism of A1}{*}
Из равенств
\EqRef{fi omega},
\eqRef{f is homomorphism of A1}{*}
следует, что
\ShowEq{f is homomorphism of A1, 1}
Из равенств
\EqRef{f*:A1->*M(X,A2)},
\EqRef{f is homomorphism of A1, 1}
следует, что
\ShowEq{f* is homomorphism of A1}
Из равенств
\EqRef{fi omega},
\EqRef{f* is homomorphism of A1}
следует, что
\ShowEq{f* is homomorphism of A1, 1}
Из равенства
\EqRef{f* is homomorphism of A1, 1}
следует, что
\ShowEq{f* is homomorphism of A1, 2}
Из равенства
\EqRef{f* is homomorphism of A1, 2}
следует, что отображение
$f^*$ является гомоморфизмом $\Omega_1$\Hyph группы $A_1$.

Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
\ShowEq{f(a1) a1 A1}
является гомоморфизмом $\Omega_2$\Hyph группы $A_2$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega2}
и произвольных
\ShowEq{a1...an A2}
следующее равенство верно
\DrawEq{f() is homomorphism of A2}{*}
Из равенств
\EqRef{f*:A1->*M(X,A2)},
следует, что
\ShowEq{f*() is homomorphism of M(X,A2)}
Из равенств
\EqRef{fi omega},
\EqRef{f*() is homomorphism of M(X,A2)}
следует, что
\ShowEq{f*() is homomorphism of M(X,A2), 1}
Из равенств
\eqRef{f() is homomorphism of A2}{*},
\EqRef{f*() is homomorphism of M(X,A2), 1}
следует, что
\ShowEq{f*() is homomorphism of M(X,A2), 2}
Из равенств
\EqRef{fi omega},
\EqRef{f*:A1->*M(X,A2)},
\EqRef{f*() is homomorphism of M(X,A2), 2}
следует, что
\ShowEq{f*() is homomorphism of M(X,A2), 3}
Из равенства
\EqRef{f*() is homomorphism of M(X,A2), 3}
следует, что
\ShowEq{f*() is homomorphism of M(X,A2), 4}
Из равенства
\EqRef{f*() is homomorphism of M(X,A2), 4}
следует, что
для любого $a_1\in A_1$ отображение
$f^*(a_1)$ является гомоморфизмом $\Omega_2$\Hyph группы
\ShowEq{M(X,A2)}.
\end{proof}

\section{Представление \texorpdfstring{$\Omega$}{Omega}-группы
отображений}

\begin{theorem}
Представление
\ShowEq{A1->*A2}
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$
порождает представление
\ShowEq{M(X,A1)->*M(X,A2)}
$\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
в $\Omega_2$\Hyph группе
\ShowEq{M(X,A2)}
где (
\ShowEq{g1 in M(X,A1)},
\ShowEq{g2 in M(X,A2)}
)
\ShowEq{f(x)g(x):X->A2}
\end{theorem}
\begin{proof}
Чтобы доказать теорему, мы должны показать, что отображение
$f_X$ является гомоморфизмом $\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}
и для любого
\ShowEq{g1 in M(X,A1)}
отображение
$f_X(g_1)$ является гомоморфизмом $\Omega_2$\Hyph группы
\ShowEq{M(X,A2)}.

Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
$f$ является гомоморфизмом $\Omega_1$\Hyph группы $A_1$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega1}
и произвольных
\ShowEq{a1...an A1}
следующее равенство верно
\DrawEq{f is homomorphism of A1}{X}
Из равенства
\EqRef{fi omega}
следует, что
\ShowEq{fi omega M(X,A1)}
Из равенств
\eqRef{f is homomorphism of A1}{X},
\EqRef{fi omega M(X,A1)}
следует, что
\ShowEq{f is homomorphism of M(X,A1)}
Из равенств
\EqRef{fi omega},
\EqRef{f is homomorphism of M(X,A1)},
следует, что
\ShowEq{f is homomorphism of M(X,A1), 1}
Из равенств
\EqRef{f(x)g(x):X->A2},
\EqRef{f is homomorphism of M(X,A1), 1}
следует, что
\ShowEq{fX is homomorphism of M(X,A1)}
Из равенств
\EqRef{fi omega},
\EqRef{fX is homomorphism of M(X,A1)}
следует, что
\ShowEq{fX is homomorphism of M(X,A1), 1}
Из равенства
\EqRef{fX is homomorphism of M(X,A1), 1}
следует, что
\ShowEq{fX is homomorphism of M(X,A1), 2}
Из равенства
\EqRef{fX is homomorphism of M(X,A1), 2}
следует, что отображение
$f_X$ является гомоморфизмом $\Omega_1$\Hyph группы
\ShowEq{M(X,A1)}.

Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
\ShowEq{f(a1) a1 A1}
является гомоморфизмом $\Omega_2$\Hyph группы $A_2$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega2}
и произвольных
\ShowEq{a1...an A2}
следующее равенство верно
\DrawEq{f() is homomorphism of A2}{X}
Из равенства
\EqRef{fi omega}
следует, что
\ShowEq{fi omega M(X,A2)}
Из равенств
\eqRef{f() is homomorphism of A2}{X},
\EqRef{fi omega M(X,A2)}
следует, что
\ShowEq{f() is homomorphism of M(X,A2)}
Из равенств
\EqRef{f(x)g(x):X->A2},
\EqRef{f() is homomorphism of M(X,A2)}
следует, что
\ShowEq{fX() is homomorphism of M(X,A2)}
Из равенств
\EqRef{fi omega},
\EqRef{fX() is homomorphism of M(X,A2)}
следует, что
\ShowEq{fX() is homomorphism of M(X,A2), 1}
Из равенств
\eqRef{f() is homomorphism of A2}{X},
\EqRef{fX() is homomorphism of M(X,A2), 1}
следует, что
\ShowEq{fX() is homomorphism of M(X,A2), 2}
Из равенства
\EqRef{fX() is homomorphism of M(X,A2), 2}
следует, что,
для любого
\ShowEq{g1 in M(X,A1)},
отображение
$f_X(g_1)$ является гомоморфизмом $\Omega_2$\Hyph группы
\ShowEq{M(X,A2)}.
\end{proof}

\begin{theorem}
\label{theorem: fX(g1)(g2), converges uniformly}
Пусть
\ShowEq{A1->*A2}
представление
полной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в полной $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть последовательность отображений
\ShowEq{g1n M(X,A1)}
сходится равномерно
к отображению $g_1$.
Пусть последовательность отображений
\ShowEq{g2n M(X,A2)}
сходится равномерно
к отображению $g_2$.
Пусть множество значений отображения $g_i$, $i=1$, $2$,
компактно.
Тогда последовательность отображений
\ShowEq{f(g1n)(g2n)}
сходится равномерно
к отображению
\ShowEq{fX(g1)(g2)}.
\end{theorem}
\begin{proof}
Из равенства
\ShowEq{gi(x)=lim}
и теоремы
\ref{theorem: sequence converges uniformly}
следует, что для заданного
\DrawEq{delta1 in R}{g1n g2n}
существует $N_i$ такое, что из условия
\ShowEq{n>Ni}
следует
\ShowEq{gin in B_o}
Пусть
\ShowEq{N N1 N2}
Из равенства
\EqRef{gin in B_o},
теоремы
\ref{theorem: f c1 c2 in B}
и условия $n>N$
следует, что
\ShowEq{f g1n g2n in B_o 1}
\DrawEq{epsilon12=f(delta12)}{g}
где
\DrawEq{C=|f|+delta}{12}
Значение \(C_i\) зависит от \(x\).
Поэтому $\epsilon_1$ также зависит от \(x\).
Для оценки равномерной сходимости
нам необходимо выбрать максимальное значение $\epsilon_1$.
Для заданного \(\delta_1\), значение $\epsilon_1$
является полилинейным отображением значений \(C_i\).
Следовательно, $\epsilon_1$ имеет максимальное значение,
когда каждое \(C_i\) имеет максимальное значение.
Так как мы рассматриваем оценку значения \(\epsilon_1\)
справа,
для нас неважно одновременно ли \(C_i\) приобретают
максимальные значения.
Так как множество значений отображения
$f_i$
компактно,
то, согласно теореме
\ref{theorem: norm of compact set is bounded},
определена следующая величина
\DrawEq{F=sup|f|}{g1n g2n}
Из равенства
\eqRef{F=sup|f|}{g1n g2n}
и утверждения
\RefItem{|a|>=0}
следует, что
\DrawEq{F>0}{g1n g2n}
Из равенств
\eqRef{C=|f|+delta}{12},
\eqRef{F=sup|f|}{g1n g2n}
следует, что мы можем положить
\DrawEq{C=F+delta}{g1n g2n}
Из равенства
\eqRef{C=F+delta}{g1n g2n}
и утверждений
\eqRef{F>0}{g1n g2n},
\eqRef{delta1 in R}{g1n g2n}
следует, что
\DrawEq{C>0}{g1n g2n}
Из равенств
\eqRef{epsilon12=f(delta12)}{g},
\eqRef{C=F+delta}{g1n g2n}
и утверждения
\eqRef{C>0}{g1n g2n}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon12=f(delta12)}{g}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $N$ зависит от значения $\delta_1$.
Мы выберем значение $N$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $N$ такое, что из условия
$n>N$
следует
\ShowEq{f g1n g2n in B_o 2}
Равенство
\ShowEq{lim f g1n g2n}
следует из равенства
\EqRef{f g1n g2n in B_o 2}
и теоремы
\ref{theorem: sequence converges uniformly}.
\end{proof}

\section{Пополнение представления
\texorpdfstring{$\Omega$}{Omega}-группы}

\begin{definition}
\label{definition: completion of representation of Omega group}
Пусть
\ShowEq{A1->*A2}
представление
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Представление
\ShowEq{B1->*B2}
полной $\Omega_1$\Hyph группы $B_1$
в полной $\Omega_2$\Hyph группе $B_2$
называется
\AddIndex{пополнением представления}
{completion of representation} $f$,
если
\StartLabelItem
\begin{enumerate}
\item
$\Omega$\Hyph группа \(B_1\) является
пополнением нормированной \(\Omega_1\)\Hyph группы \(A_1\).
\LabelItem{B1 is completion of A1}
\item
$\Omega$\Hyph группа \(B_2\) является
пополнением нормированной \(\Omega_2\)\Hyph группы \(A_2\).
\LabelItem{B2 is completion of A2}
\item
\LabelItem{g a1 a2 = f a1 a2}
Если \(a_1\in A_1\), \(a_2\in A_2\), то
\ShowEq{g a1 a2 = f a1 a2}
\end{enumerate}
\qed
\end{definition}

\begin{theorem}
\label{theorem: completion of representation of Omega group is unique}
Пусть
\ShowEq{A1->*A2}
представление
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть представления
\ShowEq{B1->*B2 12}
являются пополнениями представления $f$.
\StartLabelItem
\begin{enumerate}
\item
Для \(i=1\), \(2\),
существует изоморфизм $\Omega$\Hyph группы
\ShowEq{h:Bi1->Bi2}
такой, что
\ShowEq{h:Bi1->Bi2 A}
\ShowEq{h:Bi1->Bi2 ||}
\LabelItem{Bi1->Bi2}
\item
Пара отображений
\ShowEq{morphism of representations h1 h2}
является морфизмом представлений из $g_1$ в $g_2$.
\LabelItem{morphism of representations}
\end{enumerate}
\end{theorem}
\begin{proof}
Утверждение
\RefItem{Bi1->Bi2}
является следствием теоремы
\ref{theorem: completion of normed Omega group is unique}.

Пусть
\ShowEq{bi in Bi}
Согласно теореме
\ref{theorem: sequence in dense set}
существуют последовательности $A_i$\Hyph чисел $a_{i\cdot n}$ такая, что
\ShowEq{bi=lim ain}
Из равенства
\EqRef{bi=lim ain}
следует, что последовательность $A_I$\Hyph чисел $a_{i\cdot n}$
является фундаментальной последовательностью
в $\Omega$\Hyph группе $A_i$.
Для любого \(n\) следующее равенство очевидно
\ShowEq{f a1 a2=f a1 a2}
Так как
\ShowEq{f a1 a2 in A2}
то равенство
\ShowEq{f a1 a2 =}
является следствием равенства
\EqRef{h:Bi1->Bi2 A}.
Непрерывность отображений \(h_1\), \(h_2\)
следует из равенства
\EqRef{h:Bi1->Bi2 ||}.
Следовательно,
равенство
\ShowEq{f b1 b2 =}
следует из равенств
\EqRef{bi=lim ain},
\EqRef{f a1 a2 =}
и теоремы
\ref{theorem: lim f c1n c2n}.
Теорема следует из равенств
\EqRef{f b1 b2 =},
\xEqRef{0912.3315}{morphism of representations of F algebra, definition, 2m}
и определения
\xRef{0912.3315}{definition: morphism of representations of F algebra}.
\end{proof}

\begin{lemma}
\label{lemma: f a1n a2n is fundamental sequence}
Пусть
\ShowEq{A1->*A2}
представление
нормированной $\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в нормированную $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Пусть
\ShowEq{a1n}
является фундаментальной последовательностью \(A_1\)\Hyph чисел.
Пусть
\ShowEq{a2n}
является фундаментальной последовательностью \(A_2\)\Hyph чисел.
Тогда последовательность
\ShowEq{f a1n a2n}
является фундаментальной последовательностью \(A_2\)\Hyph чисел.
\end{lemma}
\begin{proof}
Пусть
\DrawEq{delta1 in R}{a1m a2m fundamental}
Так как последовательность
\ShowEq{a1n}
является фундаментальной последовательностью \(A_1\)\Hyph чисел,
то согласно теореме
\ref{theorem: fundamental sequence}
следует, что для заданного
\(\delta_1\)
существует, зависящее от \(\delta_1\), натуральное число $N_1$ такое, что
\ShowEq{a1q in B(a1p,d1)}
для любых $p$, $q>N_1$.
Так как последовательность
\ShowEq{a2n}
является фундаментальной последовательностью \(A_2\)\Hyph чисел,
то согласно теореме
\ref{theorem: fundamental sequence},
следует, что для заданного
\(\delta_1\)
существует, зависящее от \(\delta_1\), натуральное число $N_2$ такое, что
\ShowEq{a2q in B(a2p,d1)}
для любых $p$, $q>N_2$.
Пусть
\ShowEq{N N1 N2}
Из утверждений
\EqRef{a1q in B(a1p,d1)},
\EqRef{a2q in B(a2p,d1)}
и теоремы
\ref{theorem: f c1 c2 in B}
следует, что
\ShowEq{f a1 a2 in B 1}
\DrawEq{epsilon12=f(delta12)}{a1m a2m fundamental}
где
\DrawEq{C=|ap|+d1}{a1m a2m fundamental}
Из равенства
\eqRef{C=|ap|+d1}{a1m a2m fundamental}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{a1m a2m fundamental}
следует, что
\DrawEq{C>0}{a1p a2p}
Из равенств
\eqRef{epsilon12=f(delta12)}{a1m a2m fundamental},
\eqRef{C=|ap|+d1}{a1m a2m fundamental}
и утверждения
\eqRef{C>0}{a1p a2p}
следует, что $\epsilon_1$ является полиномиальной
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon12=f(delta12)}{a1m a2m fundamental}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $N$ зависит от значения $\delta_1$.
Мы выберем значение $N$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $N$ такое, что из условия
$n>N$
следует
\ShowEq{f a1 a2 in B 2}
Из утверждения
\EqRef{f a1 a2 in B 2}
и теоремы
\ref{theorem: fundamental sequence}
следует, что последовательность
\ShowEq{f a1n a2n}
является фундаментальной последовательностью.
\end{proof}

\begin{theorem}
Пополнение представления нормированной $\Omega$\Hyph группы существует.
\end{theorem}
\begin{proof}
Пусть $A_1$ - нормированная $\Omega_1$\Hyph группа.
Пусть $A_2$ - нормированная $\Omega_2$\Hyph группа.
Согласно теореме
\ref{theorem: completion of normed Omega group},
существует
пополнение \(B_1\) нормированной \(\Omega_1\)\Hyph группы \(A_1\)
и
пополнение \(B_2\) нормированной \(\Omega_2\)\Hyph группы \(A_2\).

Чтобы доказать существование пополнения \(g\) представления \(f\)
\ShowEq{B1->*B2}
мы будем пользоваться записью, предложенной в разделе
\ref{section: completion of normed Omega group}.
Рассмотрим отношением эквивалентности на множестве фундаментальных
последовательностей $A_i$\Hyph чисел
\ShowEq{sim lim a-b=0 i}
Пусть $B_i$ является множеством классов эквивалентных фундаментальных
последовательностей $A_i$\Hyph чисел.
Мы будем пользоваться записью
\ShowEq{[ai]}
для класса последовательностей, эквивалентных последовательности
\(a_{i\cdot n}\).

%{\hangindent=1cm
%\setlength{\parindent}{1.6cm}
\begin{lemma}
\label{lemma: f a1 a2 sim f b1 b2}
Пусть
\ShowEq{a1n b1n}
являются фундаментальными последовательностями \(A_1\)\Hyph чисел,
\ShowEq{a1n sim b1n}
Пусть
\ShowEq{a2n b2n}
являются фундаментальными последовательностями \(A_2\)\Hyph чисел,
\ShowEq{a2n sim b2n}
Тогда
\ShowEq{f a1 a2 sim f b1 b2}
\end{lemma}

{\sc Доказательство.}
Пусть
\DrawEq{delta1 in R}{f a1 a2 sim f b1 b2}
Из утверждения
\EqRef{a1n sim b1n}
и леммы
\ref{lemma: a sim b}
следует, что
для заданного
\(\delta_1\)
существует, зависящее от $\delta_1$, натуральное число $N_1$ такое, что
\ShowEq{b1n in B(a1n)}
для любого $n>N_1$.
Из утверждения
\EqRef{a2n sim b2n}
и теоремы
\ref{lemma: a sim b}
следует, что
для заданного
\(\delta_1\)
существует, зависящее от $\delta_1$, натуральное число $N_2$ такое, что
\ShowEq{b2n in B(a2n)}
для любого $n>N_2$.
Пусть
\ShowEq{N N1 N2}
Из утверждений
\EqRef{b1n in B(a1n)},
\EqRef{b2n in B(a2n)}
и теоремы
\ref{theorem: f c1 c2 in B}
следует, что
\ShowEq{f b1 b2 in B 1}
\DrawEq{epsilon12=f(delta12)}{f a1 a2 sim f b1 b2}
где
\DrawEq{C=|an|+d1}{f a1 a2 sim f b1 b2}
Из равенства
\eqRef{C=|an|+d1}{f a1 a2 sim f b1 b2}
и утверждений
\RefItem{|a|>=0},
\eqRef{delta1 in R}{f a1 a2 sim f b1 b2}
следует, что
\DrawEq{C>0}{f a1 a2 sim f b1 b2}
Из равенств
\eqRef{epsilon12=f(delta12)}{f a1 a2 sim f b1 b2},
\eqRef{C=|an|+d1}{f a1 a2 sim f b1 b2}
и утверждения
\eqRef{C>0}{f a1 a2 sim f b1 b2}
следует, что $\epsilon_1$ является
строго монотонно возрастающей функцией $\delta_1>0$.
При этом
\ShowEq{d1=0=>e1=0}
Согласно теореме
\ref{theorem: image of interval is interval, real field},
отображение
\eqRef{epsilon12=f(delta12)}{f a1 a2 sim f b1 b2}
отображает интервал
$[0,\delta_1)$
в интервал
$[0,\epsilon_1)$.
Согласно теореме
\ref{theorem: continuous map, open set},
для заданного
$\epsilon>0$
существует такое
$\delta>0$, что
\ShowEq{e(d)<e}
Согласно построению,
значение $N$ зависит от значения $\delta_1$.
Мы выберем значение $N$, соответствующее
$\delta_1=\delta$.
Следовательно,
для заданного
\ShowEq{epsilon in R}
существует $N$ такое, что из условия
$n>N$
следует
\ShowEq{f b1 b2 in B 2}
Утверждение
\EqRef{f a1 a2 sim f b1 b2}
следует из утверждения
\EqRef{f b1 b2 in B 2}
и леммы
\ref{lemma: a sim b}.
\hfill\(\odot\)

Согласно леммам
\ref{lemma: f a1n a2n is fundamental sequence},
\ref{lemma: f a1 a2 sim f b1 b2}
отображение
\ShowEq{g[a1n][a2n]=[f a1n a2n]}
определено корректно.

Пусть
\ShowEq{a12 in A12}
Согласно теореме
\ref{theorem: For any a there exists sequence},
существует последовательность \(A_i\)\Hyph чисел
\ShowEq{ain}
такая, что
\ShowEq{ai=[ain]}
Согласно теореме
\ref{theorem: lim f c1n c2n}
\ShowEq{f a1 a2=lim}
Из равенств
\EqRef{g[a1n][a2n]=[f a1n a2n]},
\EqRef{f a1 a2=lim}
следует, что отображение \(g\)
удовлетворяет утверждению
\RefItem{g a1 a2 = f a1 a2}
\ShowEq{g a1 a2 = f a1 a2 1}

\begin{lemma}
\label{lemma: f is homomorphism of A1}
Отображение
$g$ является гомоморфизмом $\Omega_1$\Hyph группы \(B_1\).
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a11...a1n}
Согласно теореме
\ref{theorem: sequence in dense set},
существует последовательность \(A_1\)\Hyph чисел
\ShowEq{a1im}
такая, что
\ShowEq{a1i=[a1im]}
Пусть
\(a_2\in B_2\).
Согласно теореме
\ref{theorem: sequence in dense set},
существует последовательность \(A_2\)\Hyph чисел
\ShowEq{a2m}
такая, что
\ShowEq{a2=[a2m]}
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
$f$ является гомоморфизмом $\Omega_1$\Hyph группы $A_1$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega1}
и любого \(m\)
следующее равенство верно
\ShowEq{fm is homomorphism of A1}
Из равенств
\EqRef{fi omega},
\EqRef{fm is homomorphism of A1},
следует, что
\ShowEq{fm is homomorphism of A1, 1}
Равенство
\ShowEq{a1i=[a1im] omega}
следует из равенства
\EqRef{a1i=[a1im]}
и теоремы
\ref{theorem: lim a1m...anm omega}.
Равенство
\ShowEq{fm is homomorphism of A1, 2}
следует из равенств
\EqRef{g[a1n][a2n]=[f a1n a2n]},
\EqRef{a2=[a2m]},
\EqRef{a1i=[a1im] omega}
и теоремы
\ref{theorem: lim f c1n c2n}.
Равенство
\ShowEq{fm is homomorphism of A1, 3}
следует из равенств
\EqRef{g[a1n][a2n]=[f a1n a2n]},
\EqRef{a1i=[a1im]},
\EqRef{a2=[a2m]}
и теоремы
\ref{theorem: lim f c1n c2n}.
Равенство
\ShowEq{fm is homomorphism of A1, 4}
следует из равенства
\EqRef{fm is homomorphism of A1, 3}
и теоремы
\ref{theorem: lim a1m...anm omega}.
Равенство
\ShowEq{fm is homomorphism of A1, 5}
следует из равенств
\EqRef{fm is homomorphism of A1, 1},
\EqRef{fm is homomorphism of A1, 2},
\EqRef{fm is homomorphism of A1, 4}.
Из равенства
\EqRef{fm is homomorphism of A1, 5}
следует, что отображение
$g$ является гомоморфизмом $\Omega_1$\Hyph группы \(B_1\).
\hfill\(\odot\)

\begin{lemma}
\label{lemma: fm() is homomorphism of A2}
Для любого
\ShowEq{a1 in B1}
отображение
\(g(a_1)\) является гомоморфизмом $\Omega_2$\Hyph группы \(B_2\).
\end{lemma}

{\sc Доказательство.}
Пусть
\ShowEq{a21...a2n}
Согласно теореме
\ref{theorem: sequence in dense set},
существует последовательность \(A_2\)\Hyph чисел
\ShowEq{a2im}
такая, что
\ShowEq{a2i=[a2im]}
Пусть
\(a_1\in B_1\).
Согласно теореме
\ref{theorem: sequence in dense set},
существует последовательность \(A_1\)\Hyph чисел
\ShowEq{a1m}
такая, что
\ShowEq{a1=[a1m]}
Согласно определению
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение
\ShowEq{f(a1m) a1m A1}
является гомоморфизмом $\Omega_2$\Hyph группы $A_2$.
Следовательно, для $n$\Hyph арной операции
\ShowEq{omega in Omega2}
и произвольного \(m\)
следующее равенство верно
\ShowEq{fm() is homomorphism of A2}
Равенство
\ShowEq{a2i=[a2im] omega}
следует из равенства
\EqRef{a2i=[a2im]}
и теоремы
\ref{theorem: lim a1m...anm omega}.
Равенство
\ShowEq{fm() is homomorphism of A2, 2}
следует из равенств
\EqRef{g[a1n][a2n]=[f a1n a2n]},
\EqRef{a1=[a1m]},
\EqRef{a2i=[a2im] omega}
и теоремы
\ref{theorem: lim f c1n c2n}.
Равенство
\ShowEq{fm() is homomorphism of A2, 3}
следует из равенств
\EqRef{g[a1n][a2n]=[f a1n a2n]},
\EqRef{a2i=[a2im]},
\EqRef{a1=[a1m]}
и теоремы
\ref{theorem: lim f c1n c2n}.
Равенство
\ShowEq{fm() is homomorphism of A2, 4}
следует из равенства
\EqRef{fm() is homomorphism of A2, 3}
и теоремы
\ref{theorem: lim a1m...anm omega}.
Равенство
\ShowEq{fm() is homomorphism of A2, 5}
следует из равенств
\EqRef{fm() is homomorphism of A2},
\EqRef{fm() is homomorphism of A2, 2},
\EqRef{fm() is homomorphism of A2, 4}.
Из равенства
\EqRef{fm() is homomorphism of A2, 5}
следует, что,
для любого
\(a_1\in B_1\),
отображение
$g(a_1)$ является гомоморфизмом $\Omega_2$\Hyph группы
\(B_2\).
\hfill\(\odot\)
%}%\hangindent

Из лемм
\ref{lemma: f is homomorphism of A1},
\ref{lemma: fm() is homomorphism of A2}
и определения
\xRef{0912.3315}{definition: Tstar representation of algebra}
следует, что
отображение \(g\),
определённое равенством
\EqRef{g[a1n][a2n]=[f a1n a2n]},
является представлением
полной $\Omega_1$\Hyph группы $B_1$
в полной $\Omega_2$\Hyph группе $B_2$.
\end{proof}





==> Omega.Ring.Russian.tex <==
%auto-ignore
\input{Omega.Ring.Eq}
%\ifx\PrintBook\Defined
%\chapter{Базис Гамеля}
%\fi

\section{\texorpdfstring{$\Omega$}{Omega}-кольцо}
%\label{Section: Module with Continues Basis}

Пусть
\ShowEq{A1->*A2}
представление
$\Omega_1$\Hyph группы $A_1$ с нормой $\|x\|_1$
в $\Omega_2$\Hyph группе $A_2$ с нормой $\|x\|_2$.
Согласно определение
\xRef{0912.3315}{definition: Tstar representation of algebra},
отображение \(f\) является гомоморфизмом $\Omega_1$\Hyph группы $A_1$.
Следовательно, если произведение определено в
$\Omega_1$\Hyph группе $A_1$,
то следующее равенство верно
\ShowEq{fab=fafb}
Однако, если произведение не определено в
$\Omega_1$\Hyph группе $A_1$,
то мы можем определить произведение в
$\Omega_1$\Hyph группе $A_1$,
пользуясь равенством
\EqRef{fab=fafb}.
Это даёт основание полагать, что в
$\Omega_1$\Hyph группе $A_1$
определено произведение.

Так как отображение \(f\) является гомоморфизмом $\Omega_1$\Hyph группы $A_1$,
то следующие равенства верны
\ShowEq{a(b+c)=ab+ac 1}
\ShowEq{a(b+c)=ab+ac 2}
Если представление \(f\) эффективно,
то равенства
\ShowEq{a(b+c)=ab+ac l}
\ShowEq{a(b+c)=ab+ac r}
являются следствием равенств
\EqRef{a(b+c)=ab+ac 1},
\EqRef{a(b+c)=ab+ac 2}.
Следовательно, умножение дистрибутивно по отношению к сложению.
Таким образом, $\Omega_1$\Hyph группа $A_1$ является
кольцом относительно сложения и умножения.

\begin{definition}
\(\Omega\)\Hyph группа, в которой определено
произведение, называется
\AddIndex{\(\Omega\)\Hyph кольцом}{Omega ring}.
\qed
\end{definition}

\begin{remark}
Бикольцо (определение
\xRef{0612.111}{definition: biring})
является примером \(\Omega\)\Hyph группы,
в которой определены две операции произведениея.
Это связано с двумя различными представлениями алгебры матриц
с элементами из некоммутативной алгебры.
Соответственно, в бикольце определены две
структуры \(\Omega\)\Hyph кольца.

В алгебре октонионов мы наблюдаем другую картину.
Так как произведение в алгебре октонионов неассоциативно,
то рассматриваемое представление алгебры октонионов
определяет иную операцию произведения.
\qed
\end{remark}

\begin{definition}
Эффективное представление \(\Omega\)\Hyph кольца \(A\)
в абелевой группе называется
\AddIndex{$A$\Hyph модулем}{module over algebra}.\footnote{Смерти
также определение
\xRef{1211.6965}{definition: module over ring}.
}
\qed
\end{definition}

Я рассматриваю представление в абелевой группе,
но не в \(\Omega\)\Hyph группе.
Это связано с тем, что произвольные операции в
универсальной алгебре усложняют условие линейной зависимости.
В тоже время, в
универсальной алгебре, порождающей представление, для нас важны только
операции сложения и умножения.


==> Preface.1305.4547.English.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\chapter{Preface}
\fi

\section{Preface}

It was first time that I drew my attention to the universal algebra
which is Abelian Group
relative to sum
in the chapter
\xRef{1003.1544}{chapter: Matrix of Mappings}.
Later I found that such universal algebra
is called $\Omega$\Hyph group.

$\Omega$\Hyph group is interesting for me, since
I think that we may consider calculus
in $\Omega$\Hyph group.
So there was a decision to study normed
$\Omega$\Hyph group.

I have devoted much attention to the topology
of normed $\Omega$\Hyph group.




==> Preface.1305.4547.Eq.tex <==
%auto-ignore





==> Preface.1305.4547.Russian.tex <==
%auto-ignore
\input{Preface.\BookNumber.Eq}

\ifx\PrintBook\Defined
\chapter{Предисловие}
\fi

\section{Предисловие}

Впервые я обратил внимание на универсальную алгебру,
которая является абелевой группой
относительно сложения,
в главе
\xRef{1003.1544}{chapter: Matrix of Mappings}.
Позже я узнал, что подобная универсальная алгебра
называется $\Omega$\Hyph группой.

$\Omega$\Hyph группа интересна для меня, так как
я полагаю, что мы можем рассмотреть математический анализ
в $\Omega$\Hyph группе.
Так возникло решение изучить нормированные
$\Omega$\Hyph группы.

Я уделил большое внимание топологии
нормированной $\Omega$\Hyph группы.



==> Symbol.Russian.tex <==
%auto-ignore
\def\indexname{Специальные символы и обозначения}
\OpenIndex

\SetIndexSpace%0%0
\Symb%
   {единичный интервал}%
   {unit interval}%

\SetIndexSpace%A%0
\Symb%
   {минорная матрица}%
   {A from b a}%
\Symb%
   {минорная матрица}%
   {A from columns T}%
\Symb%
   {минорная матрица}%
   {A from rows S}%
\Symb%
   {множество векторов, разложение которых относительно базиса $\Basis e$ сходится нормально}%
   {A plus Schauder}%
\Symb%
   {минорная матрица}%
   {A without column a}%
\Symb%
   {минорная матрица}%
   {A without columns T}%
\Symb%
   {минорная матрица}%
   {A without row b}%
\Symb%
   {минорная матрица}%
   {A without rows S}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 1}%
\Symb%
   {$A\CRcirc$\Hyph линейная комбинация}%
   {ACRcirc linear combination 2}%
\Symb%
   {активное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {active representation in basis manifold}%
\Symb%
   {активное представление группы $G(\Vector  f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {active representation in basis manifold, tower of representations}%
\Symb%
   {$A$\Hyph алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over algebra}%
\Symb%
   {алгебра многочленов над $D$\Hyph алгеброй $A$}%
   {algebra of polynomials over D algebra}%
\Symb%
   {алгебра рациональных отображений алгебры $A$}%
   {algebra of rational mappings of algebra}%
\Symb%
   {аффинное пространство}%
   {An}%
\Symb%
   {ассоциатор $D$\Hyph алгебры}%
   {associator of algebra}%
\Symb%
   {\subs строка ($c$\hyph строка) матрицы}%
   {c row}%
\Symb%
   {коммутатор $D$\Hyph алгебры}%
   {commutator of algebra}%
\Symb%
   {компонента линейного отображения}%
   {component of linear map, vector}%
\Symb%
   {компонента $p$ полилинейного отображения $\Vector A$}%
   {component of polyadditive map, D vector space}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map, vector}%
\Symb%
   {сопряжённый $D$\Hyph  модуль}%
   {conjugated D module}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {CR linear combination in A module}%
\Symb%
   {\CR степень элемента $A$ бикольца}%
   {cr power}%
\Symb%
   {\CR обратный элемент бикольца}%
   {cr-inverse element}%
\Symb%
   {\CR произведение матриц}%
   {cr-product of matrices}%
\Symb%
   {производная левого сдвига}%
   {derivative of left shift}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of left shift, 1-Parameter Group}%
\Symb%
   {производная левого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of left shift, 1-Parameter Group, algebra}%
\Symb%
   {производная правого сдвига}%
   {derivative of right shift}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической группе Ли}%
   {derivative of right shift, 1-Parameter Group}%
\Symb%
   {производная правого сдвига в $1$\Hyph параметрической D группе Ли}%
   {derivative of right shift, 1-Parameter Group, algebra}%
\Symb%
   {производная левого сдвига}%
   {derivative of Tstar shift}%
\Symb%
   {\drc вектор}%
   {drc vector}%
\Symb%
   {координаты вектора $a$ относительно базиса Гамеля}%
   {Hamel basis, coordinates}%
\Symb%
   {эрмитово сопряжение в теле}%
   {hermitian conjugation, division ring}%
\Symb%
   {тензор, обратный тензору $a$}%
   {inverse tensor}%
\Symb%
   {$(^j_i)$\hyph\CR квазидетерминант}%
   {j i CR quasideterminant definition}%
\Symb%
   {$(ji)$\hyph квазидетерминант матрицы $\bfA$}%
   {j i quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph \RC квазидетерминант}%
   {j i RC-quasideterminant definition}%
\Symb%
   {$(^j_i)$\hyph $\RCcirc$\Hyph квазидетерминант}%
   {j i RCcirc-quasideterminant definition}%
\Symb%
   {левая дробь}%
   {left fraction}%
\Symb%
   {левый главный идеал}%
   {left principal ideal}%
\Symb%
   {левый сдвиг в $D$\Hyph алгебре}%
   {left shift, D algebra}%
\Symb%
   {линейная комбинация векторов $A$\Hyph модуля}%
   {linear combination in A module}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its column}%
\Symb%
   {преобразование матрицы}%
   {matrix, replacing its row}%
\Symb%
   {$A$\Hyph модуль однородных многочленов над $D$\Hyph алгеброй $A$}%
   {module of homogeneous polynomials over algebra}%
\Symb%
   {норма в $D$\Hyph модуле}%
   {norm on D module}%
\Symb%
   {алгебра, противоположная алгебре $A$}%
   {opposite algebra}%
\Symb%
   {орбита линейного отображения}%
   {orbit of linear mapping}%
\Symb%
   {производная}%
   {overline nabla_l, definition 2}%
\Symb%
   {частное линейное отображение}%
   {partial linear map}%
\Symb%
   {главный идеал}%
   {principal ideal}%
\Symb%
   {квазидетерминант матрицы $\bfA$}%
   {quasideterminant definition}%
\Symb%
   {\sups строка ($r$\hyph строка) матрицы}%
   {r row}%
\Symb%
   {\RC степень элемента $A$ бикольца}%
   {rc power}%
\Symb%
   {\RC обратный элемент бикольца}%
   {rc-inverse element}%
\Symb%
   {\RC произведение матриц}%
   {rc-product of matrices}%
\Symb%
   {\RC квазидетерминант}%
   {RC-quasideterminant definition}%
\Symb%
   {$\RCcirc$\Hyph квазидетерминант}%
   {RCcirc-quasideterminant definition}%
\Symb%
   {\rcd вектор}%
   {rcd vector}%
\Symb%
   {правый главный идеал}%
   {right principal ideal}%
\Symb%
   {правый сдвиг в $D$\Hyph алгебре}%
   {right shift, D algebra}%
\Symb%
   {координаты вектора $a$ относительно базиса Шаудера}%
   {Schauder basis, coordinates}%
\Symb%
   {множество обратимых элементов алгебры $A$}%
   {set of invertible elements of algebra}%
\Symb%
   {множество нулей алгебры $A$}%
   {set of zeros of algebra}%
\Symb%
   {множество полилинейных отображений колец $R_1$, ..., $R_n$ в модуль $S$}%
   {set polylinear maps, ring}%
\Symb%
   {симплекс}%
   {simplex}%
\Symb%
   {косое произведение векторов $\Vector a_1$, ..., $\Vector a_m$}%
   {skew product of vectors}%
\Symb%
   {правый сдвиг}%
   {starT shift}%
\Symb%
   {\sT сдвиг}%
   {starT shift, fibered group}%
\Symb%
   {тензорная степень алгебры $A$}%
   {tensor power of algebra}%
\Symb%
   {тензорное произведение алгебр}%
   {tensor product of algebras}%
\Symb%
   {левый сдвиг}%
   {Tstar shift}%
\Symb%
   {\Ts сдвиг}%
   {Tstar shift, fibered group}%
\Symb%
   {неголономные координаты вектора}%
   {vector anholonomic coordinates}%
\Symb%
   {голономные координаты вектора}%
   {vector holonomic coordinates}%

\SetIndexSpace%B%0
\Symb%
   {многообразие базисов \rcd векторного пространства $\Vector V$}%
   {basis manifold of rcd vector space}%
\Symb%
   {многообразие базисов векторного пространства}%
   {basis manifold of vector space}%
\Symb%
   {многообразие базисов представления $f$}%
   {basis manifold representation F algebra}%
\Symb%
   {многообразие базисов башни представлений $\Vector f$}%
   {basis manifold tower of representations}%
\Symb%
   {многообразие базисов аффинного пространства}%
   {Basis Manifold, Affine Space}%
\Symb%
   {многообразие базисов \rcd аффинного пространства}%
   {Basis Manifold, rcd Affine Space, division ring}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {BCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {BEn}%
\Symb%
   {алгебра Бореля}%
   {Borel algebra}%
\Symb%
   {декартова степень $\Bundle A$ расслоения $\Bundle B$}%
   {Cartesian power A of bundle B}%
\Symb%
   {декартова степень $A$ множества $B$}%
   {Cartesian power of set}%
\Symb%
   {замкнутый шар}%
   {closed ball}%
\Symb%
   {замыкание множества}%
   {closure of set}%
\Symb%
   {многообразие базисов центро-аффинного пространства}%
   {FCAn}%
\Symb%
   {многообразие базисов евклидова пространства}%
   {FEn}%
\Symb%
   {структура всех подпредставлений представления $f$}%
   {lattice of subrepresentations}%
\Symb%
   {структура башен подпредставлений башни представлений $\Vector f$}%
   {lattice of subrepresentations, tower of representations}%
\Symb%
   {открытый шар}%
   {open ball}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, 1 n}%
\Symb%
   {правая дробь}%
   {right fraction}%
\Symb%
   {тензорная степень представления}%
   {tensor power of representation}%
\Symb%
   {тензорное произведение представлений}%
   {tensor product of representations}%

\SetIndexSpace%C%0
\Symb%
   {$\sigma$\Hyph алгебра измеримых относительно меры $\mu$ множеств}%
   {algebra of sets measurable with respect to measure}%
\Symb%
   {центро-аффинное пространство}%
   {CAn}%
\Symb%
   {центро-аффинное пространство}%
   {central affine space}%
\Symb%
   {столбцовый определитель по $j$-му столбцу  матрицы $\bfA$}%
   {column determinant}%
\Symb%
   {$\CRcirc$\Hyph произведение матриц отображений}%
   {cr product of matrices of mappings}%
\Symb%
   {левые структурные константы алгебры Ли}%
   {left structural constant of Lie algebra}%
\Symb%
   {правые структурные константы алгебры Ли}%
   {right structural constant of Lie algebra}%
\Symb%
   {множество непрерывных отображений нескольких переменных}%
   {set continuous multivariable maps}%
\Symb%
   {структурные константы}%
   {structural constants}%

\SetIndexSpace%D%0
\Symb%
   {базовый вектор представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A}%
\Symb%
   {координаты базового вектора представления группы Ли над алгеброй $A$}%
   {basis vector of representation of Lie group over algebra A, coordinates}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative of map, D vector space, short}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order}%
\Symb%
   {компонента производной Гато второго порядка отображения $f(x)$}%
   {component of Gateaux derivative of Second Order, D vector space}%
\Symb%
   {компонента производной Гато отображения $f(x)$}%
   {component of Gateaux derivative, vector space}%
\Symb%
   {сопряжение в алгебре}%
   {conjugation in algebra}%
\Symb%
   {сопряжение в кольце}%
   {conjugation in ring}%
\Symb%
   {координатное \Drc векторное расслоение}%
   {coordinate drc vector bundle}%
\Symb%
   {координатное \rcd векторное пространство}%
   {coordinate rcd vector space}%
\Symb%
   {координатная система отсчёта}%
   {coordinate reference frame, extensive definition}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in bundle, 1}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, 1 n}%
\Symb%
   {двойной определитель матрицы $\bfA$}%
   {double determinant}%
\Symb%
   {\Ds производная Фреше функции $f$ тела}%
   {Frechet Dstar derivative of map, division ring}%
\Symb%
   {\dcr производная Гато отображения $\Vector f$ $D$\Hyph векторного пространства $V$ в $D$\Hyph векторное пространство $W$}%
   {Gateaux dcr derivative of map, D vector space}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map}%
\Symb%
   {производная Гато отображения $f$}%
   {Gateaux derivative of map, fraction}%
\Symb%
   {производная Гато порядка $n$}%
   {Gateaux derivative of Order n}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, division ring}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ алгебры}%
   {Gateaux derivative of Order n, fraction, algebra}%
\Symb%
   {производная Гато порядка $n$ отображения $f$ тела}%
   {Gateaux derivative of Order n, fraction, division ring}%
\Symb%
   {производная Гато второго порядка}%
   {Gateaux derivative of Second Order}%
\Symb%
   {производная Гато второго порядка отображения $f$ алгебры}%
   {Gateaux derivative of Second Order, fraction, algebra}%
\Symb%
   {производная Гато второго порядка отображения $f$ тела}%
   {Gateaux derivative of Second Order, fraction, division ring}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, scalar}%
\Symb%
   {дифференциал Гато отображения $f$}%
   {Gateaux differential of map, vector}%
\Symb%
   {\Ds производная Гато функции $f$ тела $D$}%
   {Gateaux Dstar derivative of map, division ring}%
\Symb%
   {якобиан Гато отображения $D$\Hyph векторного пространства}%
   {Gateaux Jacobian of map, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 1, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 2, D vector space}%
\Symb%
   {частная \dcr производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial dcr derivative of map, 3, D vector space}%
\Symb%
   {частная производная Гато}%
   {Gateaux partial derivative}%
\Symb%
   {смешанная частная производная Гато}%
   {Gateaux partial derivative of Second Order}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 1, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 2, D vector space}%
\Symb%
   {частная \rcd производная Гато отображения $f^{\gi b}$ по переменной $x^{\gi a}$}%
   {Gateaux partial rcd derivative of map, 3, D vector space}%
\Symb%
   {\rcd производная Гато отображения $f$ $D$\hyph векторного пространства $V$ в $D$\hyph векторное пространство $W$}%
   {Gateaux rcd derivative of map, D vector space}%
\Symb%
   {\sD производная Гато функции $f$ тела $D$}%
   {Gateaux starD derivative of map, division ring}%
\Symb%
   {векторное пространство матриц}%
   {matrices vector space}%
\Symb%
   {производная Картана}%
   {overbrace D}%
\Symb%
   {производная}%
   {overline D}%
\Symb%
   {производная вдоль векторного поля $e_{(k)}$}%
   {partial(k)}%
\Symb%
   {произведение отображения на скаляр}%
   {product of map over scalar}%
\Symb%
   {\drc векторное пространство \subs строк}%
   {r rows drc vector space}%
\Symb%
   {скорость отклонения}%
   {speed of deviation}%
\Symb%
   {стандартная компонента производной Гато}%
   {standard component of Gateaux derivative}%
\Symb%
   {тензорное произведение тел}%
   {tensor product of division rings}%
\Symb%
   {тензорное произведение колец}%
   {tensor product of rings}%
\Symb%
   {тип векторного пространства}%
   {vector space type}%

\SetIndexSpace%E%0
\Symb%
   {$A\CRcirc$\Hyph базис модуля}%
   {A CRcirc basis, module over algebra}%
\Symb%
   {матрица Якоби левого сдвига}%
   {aE, quaternion, Jacobian matrix}%
\Symb%
   {аффинный базис}%
   {Affine Basis}%
\Symb%
   {базис векторного пространства}%
   {Basis e}%
\Symb%
   {базис в векторном пространстве $\Vector V$}%
   {basis in V}%
\Symb%
   {базис $D$\Hyph модуля $\mathcal L(D;A_1;A_2)$}%
   {basis L(A1,A2)}%
\Symb%
   {базис в векторном пространстве}%
   {basis, vector space}%
\Symb%
   {базис $(n)$\hyph векторного пространства}%
   {basis,n vector space}%
\Symb%
   {декартова степень расслоенного пространства}%
   {Cartesian power of total spaces}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 1}%
\Symb%
   {центро-аффинный базис}%
   {Central Affine Basis}%
\Symb%
   {базис в \Drc векторного расслоения}%
   {drc basis, vector bundle}%
\Symb%
   {форма системы отсчёта}%
   {dual forms, reference frame}%
\Symb%
   {евклидово пространство}%
   {Euclid space}%
\Symb%
   {евклидово пространство}%
   {Euclid space, division ring}%
\Symb%
   {базис Гамеля}%
   {Hamel basis}%
\Symb%
   {тождественное преобразование расслоения}%
   {identical transformation of bundle}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_1, quaternion}%
\Symb%
   {линейный автоморфизм алгебры кватернионов}%
   {mapping E_2, quaternion}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space}%
\Symb%
   {псевдоевклидово пространство}%
   {pseudo Euclid space, division ring}%
\Symb%
   {алгебра кватернионов над полем $F$}%
   {quaternion algebra over the field}%
\Symb%
   {алгебра кватернионов с делением над полем $F$}%
   {quaternion division algebra over the fieldL}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 1}%
\Symb%
   {$\RCcirc A$\Hyph линейная комбинация}%
   {RCcircA linear combination 2}%
\Symb%
   {\rcd аффинный базис}%
   {rcd affine basis, division ring}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 1}%
\Symb%
   {базис Шаудера}%
   {Schauder basis}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\Bundle E$}%
   {set of starT nonsingular transformations of bundle}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\Bundle E$}%
   {set of Tstar nonsingular transformations of bundle}%
\Symb%
   {стандартные координаты базиса}%
   {standard coordinates of basis}%
\Symb%
   {стандартные координаты системы отсчёта}%
   {standard coordinates of reference frame}%
\Symb%
   {векторное поле системы отсчёта}%
   {vector field of reference frame}%
\Symb%
   {вектор базиса}%
   {vector of basis}%

\SetIndexSpace%F%0
\Symb%
   {координаты базиса в \rcd векторном пространстве \sups строк}%
   {basis coordinates, c rows rcd vector space}%
\Symb%
   {координаты базиса в \drc векторном пространстве \subs строк}%
   {basis coordinates, r rows drc vector space}%
\Symb%
   {базис в \rcd векторного пространства \sups строк}%
   {basis, c rows rcd vector space}%
\Symb%
   {базис в \drc векторном пространстве \subs строк}%
   {basis, r rows drc vector space}%
\Symb%
   {центро-аффинный}%
   {Central Affine Basis, division ring}%
\Symb%
   {компонента линейного отображения $f$ тела}%
   {component of linear map, division ring}%
\Symb%
   {компонента полилинейного отображения}%
   {component of polylinear map}%
\Symb%
   {расслоенный морфизм из расслоения $\Bundle A$ в $\Bundle B$}%
   {fibered morphism from A into B}%
\Symb%
   {фильтр $\mathfrak{F}$ сходится к множеству $A$}%
   {filter converges}%
\Symb%
   {гомоморфизм расслоенных универсальных алгебр}%
   {homomorphism of fibered universal algebras}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 1}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 1}%
\Symb%
   {отображение в декартово произведение}%
   {map to Cartesian product}%
\Symb%
   {норма функционала}%
   {norm of functional}%
\Symb%
   {норма отображения}%
   {norm of map}%
\Symb%
   {норма полилинейного отображения}%
   {norm of polymap}%
\Symb%
   {норма представления}%
   {norm of representation}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of Tstar representation of group}%
\Symb%
   {ортонормированный базис}%
   {Orthonornal Basis, division ring}%
\Symb%
   {кватернионная алгебра над полем ${\rm {\mathbb{F}}}$}%
   {quaternion algebra F a b}%
\Symb%
   {система отсчёта}%
   {reference frame}%
\Symb%
   {система отсчёта, расширенное определение}%
   {reference frame, extensive definition}%
\Symb%
   {стандартная компонента биаддитивного отображения $f$ над полем $F$}%
   {standard component of biadditive map, division ring}%
\Symb%
   {стандартная компонента линейного отображения }%
   {standard component of linear map, G}%
\Symb%
   {стандартная компонента полилинейного отображения}%
   {standard component of polylinear map}%
\Symb%
   {стандартная компонента квадратичного отображения $f$ над полем $F$}%
   {standard component of quadratic map, division ring}%
\Symb%
   {стандартная компонента тензора}%
   {standard component of tensor}%
\Symb%
   {сумма линейных отображений}%
   {sum of linear maps}%

\SetIndexSpace%G%0
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {группа аффинных преобразований}%
   {affine transformation group}%
\Symb%
   {\CR матричная группа}%
   {cr-matrix group}%
\Symb%
   {расслоенная малая группа сечения $h$}%
   {fibered little group}%
\Symb%
   {расслоенная группа стабилизации сечения $h$}%
   {fibered stability group}%
\Symb%
   {алгебра Ли группы Ли}%
   {g}%
\Symb%
   {определённая слева алгебра Ли группы Ли}%
   {gl}%
\Symb%
   {определённая справа алгебра Ли группы Ли}%
   {gr}%
\Symb%
   {группа автоморфизмов представления $f$}%
   {group of automorphisms of representation}%
\Symb%
   {группа гомоморфизмов векторного пространства $\Vector V$}%
   {GV}%
\Symb%
   {группа линейных преобразований}%
   {linear transformation group}%
\Symb%
   {малая группа элемента $x$}%
   {little group}%
\Symb%
   {орбита ковариантного эффективного \sT представления расслоенной группы}%
   {orbit of effective covariant starT representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного \sT представления группы}%
   {orbit of effective covariant starT representation of group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления расслоенной группы}%
   {orbit of effective covariant Tstar representation of fibered group}%
\Symb%
   {орбита ковариантного эффективного		\Ts представления группы}%
   {orbit of effective covariant Tstar representation of group}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, 1 n}%
\Symb%
   {\RC матричная группа}%
   {rc-matrix group}%
\Symb%
   {группа стабилизации элемента $x$}%
   {stability group}%

\SetIndexSpace%H%0
\Symb%
   {обращение Адамара матрицы}%
   {Hadamard inverse of matrix}%
\Symb%
   {горизонтальная компонента вектора}%
   {horizontal component of vector}%
\Symb%
   {горизонтальное подпространство}%
   {horizontal subspace}%
\Symb%
   {кватернионная алгебра}%
   {quaternion algebra H a b}%
\Symb%
   {алгебра кватернионов над полем действительных чисел}%
   {quaternion algebra over real field}%

\SetIndexSpace%I%0
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator i of representation}%
\Symb%
   {инфинитезимальные образующие представления}%
   {infinitesimal generator of representation}%
\Symb%
   {инфинитезимальные образующие группы Ли}%
   {Lie group infinitesimal generators}%
\Symb%
   {модуль векторов алгебры $A$}%
   {vector module of algebra}%
\Symb%
   {модуль векторов кольца $D$}%
   {vector module of ring}%
\Symb%
   {вектор элемента $d$ алгебры}%
   {vector of algebra}%
\Symb%
   {вектор отображения $f$}%
   {vector of mapping}%
\Symb%
   {вектор элемента $d$ кольца}%
   {vector of ring}%

\SetIndexSpace%J%0
\Symb%
   {оператор замыкания представления $f$}%
   {closure operator, representation}%
\Symb%
   {оператор замыкания башни представлений $\Vector f$}%
   {closure operator, tower of representations}%
\Symb%
   {матрица Якоби правого сдвига}%
   {Ea, quaternion, Jacobian matrix}%
\Symb%
   {башня подпредставлений башни представлений $\Vector f$, порождённая кортежем множеств $\VX X$}%
   {subrepresentation generated by tuple of sets}%

\SetIndexSpace%K%0
\Symb%
   {ядро линейного отображения}%
   {kernel of linear map}%

\SetIndexSpace%L%0
\Symb%
   {левое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {left cofactor, matrix}%
\Symb%
   {левое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {left double cofactor}%
\Symb%
   {левый сдвиг}%
   {left shift}%
\Symb%
   {производная Ли связности}%
   {Lie derivative of connection}%
\Symb%
   {производная Ли метрики}%
   {Lie derivative of metric}%
\Symb%
   {предел соответствия $\Phi$ по фильтру $\mathfrak{F}$}%
   {limit of correspondence with respect to the filter}%
\Symb%
   {предел последовательности}%
   {limit of sequence}%
\Symb%
   {пассивное преобразование}%
   {passive transformation}%
\Symb%
   {множество \Acr линейных отображений модуля $\Vector V$ в модуль $\Vector W$}%
   {set Acr linear maps, module}%
\Symb%
   {$D$\Hyph модуль непрерывных линейных отображений нормированного $D$\Hyph модуля $A_1$ в нормированный $D$\Hyph модуль $A_2$}%
   {set continuous linear mappings, module}%
\Symb%
   {множество непрерывных линейных отображений}%
   {set continuous linear maps, vector}%
\Symb%
   {множество непрерывных полилинейных отображений}%
   {set continuous polylinear maps}%
\Symb%
   {\rcd векторное пространство линейных отображений \drc векторного пространства $ V$ в \drc векторное пространство $W$}%
   {set linear maps, drc vector space}%
\Symb%
   {\drc векторное пространство линейных отображений \rcd векторного пространства $V$ в \rcd векторное пространство $W$}%
   {set linear maps, rcd vector space}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, scalar}%
\Symb%
   {множество линейных отображений}%
   {set linear maps, vector}%
\Symb%
   {множество левосторонних невырожденных преобразований множества $M$}%
   {set of left-side nonsingular transformations}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps}%
\Symb%
   {множество $n$\hyph линейных отображений}%
   {set polylinear maps An}%
\Symb%
   {множество полилинейных отображений}%
   {set polylinear maps, D vector space}%
\Symb%
   {множество полилинейных отображений алгебр $A_1$, ..., $A_n$ в алгебру $A$}%
   {set polylinear maps, finite dimensional algebra}%
\Symb%
   {множество \sT представлений тела $S$ в аддитивной группе тела $R$}%
   {set sT representations, division ring}%
\Symb%
   {множество \Ts представлений тела $S$ в аддитивной группе тела $R$}%
   {set Ts representations, division ring}%

\SetIndexSpace%M%0
\Symb%
   {множество отображений в $\Omega$\Hyph группу $A$}%
   {set of maps to Omega group}%
\Symb%
   {множество \sT преобразований множества $M$}%
   {set of starT transformations}%
\Symb%
   {множество преобразований множества $M$}%
   {set of transformations}%
\Symb%
   {множество \Ts преобразований универсальной алгебры $M$}%
   {set of Tstar transformations}%
\Symb%
   {пространство орбит \sT ковариантного эффективного представления группы}%
   {space of orbits of effective sT representation}%
\Symb%
   {пространство орбит \Ts ковариантного эффективного представления группы}%
   {space of orbits of effective Ts representation}%
\Symb%
   {пространство орбит \Ts представления группы $G$ в множестве $M$}%
   {space of orbits of Ts representation}%

\SetIndexSpace%N%0
\Symb%
   {норма кватерниона $x$}%
   {norm, quaternion algebra}%
\Symb%
   {ядро $D$\Hyph алгебры $A$}%
   {nucleus of algebra}%

\SetIndexSpace%O%0
\Symb%
   {геометрический объект в координатном представлении, определённом в \rcd векторном пространстве}%
   {geometric object, coordinate rcd vector space}%
\Symb%
   {геометрический объект в координатном представлении}%
   {geometric object, coordinate vector space}%
\Symb%
   {геометрический объект, определённый в \rcd векторном пространстве}%
   {geometric object, rcd vector space}%
\Symb%
   {алгебра октонионов}%
   {octonion algebra}%
\Symb%
   {орбита представления расслоенной группы $\Bundle G$}%
   {orbit of representation of fibered group}%
\Symb%
   {орбита представления группы $G$}%
   {orbit of representation of group}%

\SetIndexSpace%P%0
\Symb%
   {расслоение}%
   {bundle}%
\Symb%
   {расслоение уровня $2$}%
   {bundle of level 2}%
\Symb%
   {расслоение уровня $n$}%
   {bundle of level n}%
\Symb%
   {декартова степень $n$ расслоения $\bundle{}{p}{E}{}$}%
   {Cartesian power of bundle}%
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 1}%
\Symb%
   {пассивное представление группы $G(f)$ в многообразии базисов $\mathcal B(f)$}%
   {passive representation in basis manifold}%
\Symb%
   {пассивное представление группы $G(\Vector f)$ в многообразии базисов $\mathcal B(\Vector f)$}%
   {passive representation in basis manifold, tower of representations}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 1}%
\Symb%
   {множество невырожденных \sT преобразований расслоения $\bundle{}pE{}$}%
   {set of starT nonsingular transformations of bundle, projection}%
\Symb%
   {множество невырожденных \Ts преобразований расслоения $\bundle{}pE{}$}%
   {set of Tstar nonsingular transformations of bundle, projection}%

\SetIndexSpace%R%0
\Symb%
   {активное преобразование}%
   {active transformation}%
\Symb%
   {\rcd векторное пространство \sups строк}%
   {c rows rcd vector space}%
\Symb%
   {кривизна Картана}%
   {Cartan curvature}%
\Symb%
   {\CR ранг матрицы}%
   {cr-rank of matrix}%
\Symb%
   {диагональ в расслоении $\bundle{}pA{}$}%
   {diagonal in bundle, 2}%
\Symb%
   {диагональ в расслоении $\Bundle A$}%
   {diagonal in reduced bundle, 2}%
\Symb%
   {образ $m$ при эндоморфизме $R$ эффективного представления}%
   {endomorphism image, effective representation}%
\Symb%
   {образ кортежа $\VX a$ при эндоморфизме $\VX r$ башни эффективных представлений}%
   {endomorphism image, tower of effective representations}%
\Symb%
   {кривизна}%
   {GLn curvature_overline}%
\Symb%
   {$\RCcirc$\Hyph произведение матриц отображений}%
   {rc product of matrices of mappings}%
\Symb%
   {\RC ранг матрицы}%
   {rc-rank of matrix}%
\Symb%
   {правое алгебраическое дополнение элемента  $a_{i{\kern 1pt} j} $ матрицы}%
   {right cofactor, matrix}%
\Symb%
   {правое двойное алгебраическое дополнение элемента $a_{ij}$ матрицы}%
   {right double cofactor}%
\Symb%
   {правый сдвиг}%
   {right shift}%
\Symb%
   {строчный определитель по  $i$-й строке матрицы $\bfA$}%
   {row determinant}%
\Symb%
   {алгебра скаляров алгебры $A$}%
   {scalar algebra of algebra}%
\Symb%
   {алгебра скаляров кольца $D$}%
   {scalar algebra of ring}%
\Symb%
   {скаляр элемента $d$ алгебры}%
   {scalar of algebra}%
\Symb%
   {скаляр отображения $f$}%
   {scalar of mapping}%
\Symb%
   {скаляр элемента $d$ кольца}%
   {scalar of ring}%
\Symb%
   {множество правосторонних невырожденных преобразований множества $M$}%
   {set of right-side nonsingular transformations}%

\SetIndexSpace%S%0
\Symb%
   {произведение расслоенных соответствий}%
   {composition of fibered correspondences}%
\Symb%
   {интеграл отображения \(f\)}%
   {integral of map}%
\Symb%
   {обратное расслоенное соответствие}%
   {inverse fibered correspondence, 2}%
\Symb%
   {обратное приведенное расслоенное соответствие}%
   {inverse reduced fibered correspondence, 2}%
\Symb%
   {линейная оболочка в векторном пространстве}%
   {linear span, vector space}%
\Symb%
   {образ базиса $X$ при пассивном преобразовании $S$}%
   {passive transformation of basis, representation}%
\Symb%
   {образ базиса $\VX X$ при пассивном преобразовании $\VX s$}%
   {passive transformation of basis, tower of representations}%
\Symb%
   {симметрическая группа}%
   {symmetric group}%

\SetIndexSpace%T%0
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры $A$}%
   {category of Tstar representations of Omega1 algebra}%
\Symb%
   {категория \Ts представлений $\Omega_1$\Hyph алгебры из категории $\mathcal A$}%
   {category of Tstar representations of Omega1 algebra from category}%
\Symb%
   {касательная плоскость к группе $G$}%
   {TaG}%
\Symb%
   {след кватерниона $x$}%
   {trace, quaternion algebra}%

\SetIndexSpace%V%0
\Symb%
   {аффинное пространство}%
   {affine space}%
\Symb%
   {сопряжённое аффинное пространство}%
   {conjugated affine space}%
\Symb%
   {сопряжённое векторное пространство}%
   {conjugated vector space}%
\Symb%
   {координатное векторное пространство}%
   {coordinate vector space}%
\Symb%
   {координаты в векторном пространстве}%
   {coordinates in vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, 1 n}%
\Symb%
   {дуальное пространство к \rcd векторному пространству $\Vector V$}%
   {dual space of rcd vector space}%
\Symb%
   {эрмитово сопряжённый вектор}%
   {hermitian conjugated vector}%
\Symb%
   {тензорное произведение $D$\Hyph векторных пространств}%
   {tensor product of D vector spaces}%
\Symb%
   {тензорное произведение \Ds векторных пространств}%
   {tensor product of Dstar vector spaces}%
\Symb%
   {векторное пространство}%
   {V}%
\Symb%
   {вертикальная компонента вектора}%
   {vertical component of vector}%
\Symb%
   {вертикальное подпространство}%
   {vertical subspace}%

\SetIndexSpace%W%0
\Symb%
   {множество координат представления $J(f,X)$}%
   {coordinate set of representation}%
\Symb%
   {множество кортежей координат башни представлений $\Vector J(\Vector f,\VX X)$}%
   {coordinate set of tower of representations}%
\Symb%
   {координаты базиса $X'$ относительно базиса $X$ представления}%
   {coordinates of basis relative to basis, representation}%
\Symb%
   {координаты элемента $m$ представления $f$ относительно множества $X$}%
   {coordinates of element relative to generating set, representation}%
\Symb%
   {координаты элемента $m$ относительно множества $X$}%
   {coordinates of element relative to set, representation}%
\Symb%
   {кортеж координат элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {coordinates of element, tower of representations}%
\Symb%
   {геометрический объект в координатном представлении, определённом в $\Omega_2$\Hyph алгебре $M$}%
   {geometric object, coordinate representation g}%
\Symb%
   {геометрический объект в координатном представлении, определённом в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, coordinate tower of representations g}%
\Symb%
   {геометрический объект, определённый в $\Omega_2$\Hyph алгбре $M$}%
   {geometric object, representation g}%
\Symb%
   {геометрический объект, определённый в кортеже $\VX\Omega$\Hyph алгебр $\VX A$}%
   {geometric object, tower of representations g}%
\Symb%
   {геометрический объект в векторном пространстве}%
   {geometric object, vector space}%
\Symb%
   {множество координат множества $B\subset J(f,X)$}%
   {subset of coordinates of representation}%
\Symb%
   {координаты кортежа множеств $\VX B$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations}%
\Symb%
   {координаты множества $B_k$ относительно кортежа множеств $\VX X$}%
   {subset of coordinates of tower of representations, k}%
\Symb%
   {множество $\Omega_2$\Hyph слов, представляющих множество $B\subset J(f,X)$}%
   {subset of words of representation}%
\Symb%
   {суперпозиция координат эндоморфизма представления $f$ и точки $m$}%
   {superposition of coordinates, representation}%
\Symb%
   {суперпозиция координат эндоморфизма башни представлений $\Vector f$ и элемента $\VX a$}%
   {superposition of coordinates, tower of representations}%
\Symb%
   {$\Omega_2$\Hyph слово, представляющее элемент $m\in J(f,X)$}%
   {word of element relative to generating set, representation}%
\Symb%
   {множество $\Omega_2$\Hyph слов представления $J(f,X)$}%
   {word set of representation}%
\Symb%
   {множество кортежей $\VX{\Omega}$\Hyph слов башни представлений $\Vector J(\Vector f,\VX X)$}%
   {word set of tower of representations}%
\Symb%
   {кортеж слов элемента $\Vector a$ относительно кортежа множеств $\VX X$}%
   {words of element, tower of representations}%

\SetIndexSpace%X%0
\Symb%
   {кватернион, сопряженный к кватерниону $x$}%
   {conjugate of quaternion}%
\Symb%
   {локальный базис аффинного пространства}%
   {local basis of affine space}%
\Symb%
   {неголономная координата}%
   {x(k)}%

\SetIndexSpace%Z%0
\Symb%
   {центр $D$\Hyph алгебры $A$}%
   {center of algebra}%
\Symb%
   {центр кольца $D$}%
   {center of ring}%

\SetIndexSpace%Delta%1
\Symb%
   {отклонение траекторий}%
   {deviation of trajectories}%
\Symb%
   {тождественное преобразование}%
   {identical transformation}%
\Symb%
   {образ вектора $\Vector e_k\in\Basis e$ при изоморфизме в координатное векторное пространство}%
   {image of vector e_k, coordinate vector space}%
\Symb%
   {символ Кронекерa}%
   {Kronecker symbol}%

\SetIndexSpace%Gamma%1
\Symb%
   {неголономные координаты связности}%
   {anholonomic coordinates of connection}%
\Symb%
   {символ Картана}%
   {Cartan symbol}%
\Symb%
   {связность}%
   {conection overline}%
\Symb%
   {коэффициенты связности в $D$\Hyph аффинном пространстве}%
   {connection coefficients, D affine space}%
\Symb%
   {связность в $D$\Hyph аффинном пространстве}%
   {connection, affine manifold}%
\Symb%
   {коэффициенты $D$\Hyph аффинной связности на многообразии}%
   {D affine connection coefficients, manifold}%
\Symb%
   {голономные координаты связности}%
   {holonomic coordinates of connection}%
\Symb%
   {связность Картана}%
   {overbrace Gamma i kl}%
\Symb%
   {множество сечений расслоения}%
   {set of sections of bundle}%

\SetIndexSpace%Lambda%1
\Symb%
   {обратный оператор оператора $\psi_l$}%
   {inverse operator to operator psi l}%
\Symb%
   {обратный оператор оператора $\psi_r$}%
   {inverse operator to operator psi r}%

\SetIndexSpace%M%1
\Symb%
   {декартово произведение мер}%
   {Cartesian product of measures}%
\Symb%
   {степень меры}%
   {power of measure}%
\Symb%
   {произведение мер}%
   {product of measures}%
\Symb%
   {произведение мер}%
   {product of measures, otimes}%

\SetIndexSpace%O%1
\Symb%
   {норма операции}%
   {norm of operation}%

\SetIndexSpace%Omega%1
\Symb%
   {объект неголономности}%
   {anholonomity object}%

\SetIndexSpace%Psi%1
\Symb%
   {левый базовый оператор группы Ли над алгеброй $A$}%
   {L basic operator of Lie group over algebra A}%
\Symb%
   {левый базовый оператор группы Ли}%
   {Lie Basic Operator L}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator L, 1-Parameter Group}%
\Symb%
   {левый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator L, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли}%
   {Lie Basic Operator R}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли}%
   {Lie Basic Operator R, 1-Parameter Group}%
\Symb%
   {правый базовый оператор однопараметрической группы Ли над алгеброй $A$}%
   {Lie Basic Operator R, 1-Parameter Group, algebra}%
\Symb%
   {правый базовый оператор группы Ли над алгеброй $A$}%
   {R basic operator of Lie group over algebra A}%

\SetIndexSpace%Fi%2
\Symb%
   {операция на группе Ли}%
   {Lie group composition law}%

\SetIndexSpace%Nabla%2
\Symb%
   {производная Картана}%
   {overbrace nabla_l}%
\Symb%
   {производная}%
   {overline nabla_l, definition 1}%

\SetIndexSpace%Phi%2
\Symb%
   {сужение соответсвия $\Phi$ на множество $C$}%
   {restriction of correspondence}%

\SetIndexSpace%Pi%2
\Symb%
   {декартово произведение расслоений}%
   {Cartesian product of bundles, definition 2}%
\Symb%
   {декартово произведение расслоенных пространств}%
   {Cartesian product of total spaces, definition 2}%
\Symb%
   {прямое произведение тел $D_i$, $i\in I$}%
   {direct product of division rings}%
\Symb%
   {прямое произведение тел $D_1$, ..., $D_n$}%
   {direct product of division rings, i 1 n}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_i$, $i\in I$}%
   {direct product, rcd vector space}%
\Symb%
   {прямое произведение $\RCstar D_i$\hyph векторных пространств $\Vector V_1$, ..., $\Vector V_n$}%
   {direct product, rcd vector space, i 1 n}%
\Symb%
   {произведение групп $G_i$, $i\in I$}%
   {product of groups}%
\Symb%
   {произведение групп $G_1$, ..., $G_n$}%
   {product of groups, i 1 n}%
\Symb%
   {произведением объектов $\{B_i,i\in I\}$ в категории $\mathcal A$}%
   {product of objects in category}%
\Symb%
   {произведением объектов $B_1$, ..., $B_n$ в категории $\mathcal A$}%
   {product of objects in category, i 1 n}%
\Symb%
   {приведенное декартово произведением расслоений}%
   {reduced Cartesian product of bundles, definition 2}%
\Symb%
   {приведенное декартово произведение расслоенных пространств}%
   {reduced Cartesian product of total spaces, definition 2}%

\SetIndexSpace%S%2
\Symb%
   {расслоенное подмножество}%
   {fibered subset}%
\Symb%
   {подрасслоение}%
   {subbundle}%

\CloseIndex

